Confident Learning: Estimating Uncertainty in Dataset Labels

Learning exists in the context of data, yet notions of confidence typically focus on model predictions, not label quality. Confident learning (CL) is an alternative approach which focuses instead on label quality by characterizing and identifying label errors in datasets, based on the principles of pruning noisy data, counting with probabilistic thresholds to estimate noise, and ranking examples to train with confidence. Whereas numerous studies have developed these principles independently, here, we combine them, building on the assumption of a class-conditional noise process to directly estimate the joint distribution between noisy (given) labels and uncorrupted (unknown) labels. This results in a generalized CL which is provably consistent and experimentally performant. We present sufficient conditions where CL exactly finds label errors, and show CL performance exceeding seven recent competitive approaches for learning with noisy labels on the CIFAR dataset. Uniquely, the CL framework is not coupled to a specific data modality or model (e.g., we use CL to find several label errors in the presumed error-free MNIST dataset and improve sentiment classification on text data in Amazon Reviews). We also employ CL on ImageNet to quantify ontological class overlap (e.g., estimating 645 "missile" images are mislabeled as their parent class "projectile"), and moderately increase model accuracy (e.g., for ResNet) by cleaning data prior to training. These results are replicable using the open-source cleanlab release.

==> Confident Learning (JAIR 2021) (Version 6610)/Makefile <==
DEPS := \
	algorithm.sty \
	algorithmic.sty \
	fancyhdr.sty \
	icml2019.bst \
	icml2019.sty \
	paper.bib \
	macros.tex \
	abstract.tex \
	introduction.tex \
	identifying.tex \
	case-study.tex \
	discussion.tex \
	correcting.tex \
	related-work.tex \
	conclusion.tex \
	acknowledgements.tex \
	bibliography.tex \


LATEX  := pdflatex
BIBTEX := bibtex
PANDOC := pandoc

# phony targets

all: paper.pdf abstract.txt

clean:
	rm -rf *.aux *.log *.blg *.bbl *.ent *.out *.dvi *.ps *.pdf *.tar.gz abstract.txt

arxiv: arxiv.tar.gz

.PHONY: all clean arxiv

# main targets

arxiv.tar.gz: paper.pdf # just build the paper because we want to build the .bbl
	tar czvf paper.tar.gz paper.tex paper.bbl $(DEPS)

%.txt: %.tex
	$(PANDOC) $< -o $@ -f latex -t plain --wrap=none

%.pdf: %.tex $(DEPS)
	$(eval SRC_$@ = $(patsubst %.tex, %, $<))
	$(LATEX) $(SRC_$@)
	$(BIBTEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)


==> Confident Learning (JAIR 2021) (Version 6610)/abstract.tex <==
\begin{abstract}
    
%% Old (Tuesday morning, Oct 8) abstract focused largely on results.
    
% Learning exists in the context of data, yet notions of \emph{confidence} typically focus on model predictions, not label quality. Using Angluin and Laird's classification noise process (CNP) to disambiguate prediction noise and label noise, we introduce \emph{confident learning} (CL) for characterizing, identifying, and learning with noisy labels in datasets.
%CL works by directly estimating the joint distribution between noisy (given) labels and uncorrupted (unknown) labels. We prove consistent joint estimation and show reasonable conditions when label errors can be found exactly. %, even with erroneous predicted probabilities for each example.
% Because CL only uses model outputs and noisy labels, it can be used with any model and dataset.
%CL outperforms recent approaches (e.g. MentorNet) by at least 30\% on CIFAR with non-uniform label noise and unlike prior art, CL performance does not degrade with non-uniformly random label noise.
%We use CL to identify real-world ImageNet training label errors, quantify ontological class overlap, and increase ResNet accuracy. 
%To facilitate research on noisy data, we open-source \texttt{cleanlab}\footnote{Python package link anonymized for the review process.}, a Python package for characterizing, finding, and learning with label errors.

%% Modified version of Ike's abstract below which re-frames our work as a generalization of confident learning.

Learning exists in the context of data, yet notions of \emph{confidence} typically focus on model predictions, not label quality. Confident learning (CL) is a data-centric approach which focuses instead on label quality by characterizing and identifying label errors in datasets, based on the principles of pruning noisy data, counting with probabilistic thresholds to estimate noise, and ranking examples to train with confidence. Whereas numerous studies have developed these principles independently, here, we combine them, building on the assumption of a class-conditional noise process to directly estimate the joint distribution between noisy (given) labels and uncorrupted (unknown) labels. This results in a generalized CL which is provably consistent and experimentally performant. We present sufficient conditions where CL exactly finds label errors, and show CL performance exceeding seven recent competitive approaches for learning with noisy labels on the CIFAR dataset. Uniquely, the CL framework is \emph{not} coupled to a specific data modality or model (e.g., we use CL to find several label errors in the presumed error-free MNIST dataset and improve sentiment classification on text data in Amazon Reviews). We also employ CL on ImageNet to quantify ontological class overlap (e.g., estimating 645 \emph{missile} images are mislabeled as their parent class \emph{projectile}), and moderately increase model accuracy (e.g., for ResNet) by cleaning data prior to training. These results are replicable using the open-source \href{https://github.com/cleanlab/cleanlab}{\texttt{cleanlab}} framework.


\end{abstract}

\endinput





% Confident learning works by estimating the joint distribution between noisy (given) labels and uncorrupted (unknown) labels, enabling three key advantages over prior art: (1) any model can be used, (2) we prove exact label error detection in non-trivial settings, and (3) performance does not degrade with class-conditional (non-uniformly random) label noise.

A key advantage over prior approaches is that confident learning works with any model and adds negligible computational overhead. 

We prove exact estimation of class-conditional label errors under mild assumptions and prove robustness when those assumptions are violated. 

We advance the state-of-the-art, achieving 82\% on CIFAR-10 with 40\% synthetic non-uniform label noise, improving on MentorNet's accuracy by 34\% .

We significantly out-perform recent approaches (e.g. MentorNet) by at least 30\%, achieving 82\% on CIFAR-10 with both 40\% uniform and non-uniform synthetic label noise.


Ubiquity of neural architectures widens this gap by popularizing benchmark datasets containing more labels than can be validated by hand.


cleanlab\footnote{\texttt{cleanlab} is a Python confident learning framework for characterizing, finding, and learning with label errors:
link to package has been obscured to respect the blind-review process.%\href{https://github.com/cleanlab/cleanlab/}{github.com/cleanlab/cleanlab}
} package, 


 Machine learning models exists in the context of data, yet notions of \emph{confidence} are typically with respect to model predictions, not data quality. 
    The ubiquity of neural architectures has widened this gap by popularizing large benchmark datasets with too many labels to validate by hand.
    We introduce \emph{confident learning} to fill the gap of uncertainty estimation for dataset labels. 
  %Confident learning, an interpretable, principle-driven family of theory and algorithms for robust weakly supervised learning in the presence of label errors. %Confident learning addresses the need for interpretable, principled approaches for weak and supervised learning in the presence of class-conditional label errors. 
%   Confident learning uses counting and ranking principles to avoid direct estimation with (often inexact) probabilities. Using these principles, 
    Confident learning is a family of theory and algorithms for characterizing, identifying, and learning with label errors in datasets.
    Unlike prior efforts with noisy labels, confident learning has no dependency on a particular model and adds negligible computational overhead
    
    Demonstrating the practicality of confident learning, we released the \href{https://github.com/cleanlab/cleanlab/}{cleanlab}\footnote{https://github.com/cleanlab/cleanlab/} package for characterizing, finding, and learning with label errors in datasets.
 
 
 
 
  %Using confident learning we establish the first practical solutions for multiclass learning with noisy labels with any classifier and robust estimation of the noisy channel (matrix of label flipping rates) and latent prior, while demonstrating surprisingly high accuracy on synthetic and MNIST datasets. We prove necessary conditions for multiclass learning with noisy labels including a lower bound on the number of examples needed. We use confident learning to identify previously undetected label errors in two prominent benchmark datasets: the MNIST train and test sets ($0.1\%$ label errors) and the 2012 ImageNet validation set ($10\%$ label errors) with exact indices of label errors for reproducibility (code freely available\footnote{\href{https://github.com/cgnorthcutt/confidentlearning}{https://github.com/cgnorthcutt/confidentlearning}}).


==> Confident Learning (JAIR 2021) (Version 6610)/acknowledgements.tex <==
\section*{Acknowledgements}

We thank the following colleagues: Jonas Mueller assisted with notation. Anish Athayle suggested starting the proof in claim 1 of Theorem \ref{thm:exact_label_errors} with the identity. Tailin Wu contributed to Lemma \ref{lemma:ideal_threshold}. Niranjan Subrahmanya provided feedback on baselines for confident learning. 


==> Confident Learning (JAIR 2021) (Version 6610)/bibliography.tex <==
\vskip 0.2in
\bibliography{paper}
\interlinepenalty=10000
\bibliographystyle{apalike}

==> Confident Learning (JAIR 2021) (Version 6610)/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

%%Confident learning bridges uncertainty estimation to dataset labels. 
%%% Uncertainty estimation in machine learning has historically focused on model predictions, not the quality of data %%labels. This is surprising given that machine learning models only exist in the context of data.
%%Whereas typical notions of \emph{confidence} like Bayesian confidence \citep{wasserman2000bayesian_confidence}, %%confidence intervals \citep{greenland2016statistical_confidence}, or probabilistic confidences %%\citep{Nguyen_2015_CVPR_high_confidence_predictions} refer to model predictions, confident learning is a %%principle-driven framework for uncertainty estimation in the context of dataset labels. 

%%Following the principles of confident learning, we developed both a confusion matrix approach $$\bm{C}_{\text{confusion}}$$ and a threshold-based counting approach $\cj$ to estimate the joint distribution of label noise $\joint$ and explicated both theoretical and experimental insights into the benefits of $\cj$. To our knowledge, this is the first work to benchmark the simple $$\bm{C}_{\text{confusion}}$$ approach which to our surprise, significantly outperformed prior art in our CIFAR experiments.

%%Using $\cj$, we demonstrated accurate estimation of $\joint$ in high noise and sparsity regimes. We empirically evaluated three criteria: (1) joint estimation, (2) finding label errors, and (3) learning with noisy labels on CIFAR and found CL methods significantly out-perform prior art across all three. In particular, the \emph{CL: opt} variant of finding label errors performed best, relying on the \emph{rank} principle for finding label errors.

Following the principles of confident learning, we developed a novel approach to estimate the joint distribution of label noise and explicated theoretical and experimental insights into the benefits of doing so. We demonstrated accurate uncertainty quantification in high noise and and sparsity regimes, across multiple datasets, data modalities, and model architectures. We empirically evaluated three criteria: (1) uncertainty quantification via estimation of the joint distribution of label noise, (2) finding label errors, and (3) learning with noisy labels on CIFAR-10, and found that CL methods outperform recent prior art across all three. 

These findings emphasize the practical nature of confident learning, identifying numerous pre-existing label issues in ImageNet, Amazon Reviews, MNIST, and other datasets, and improving the performance of learning models like deep neural networks by training on a cleaned dataset. Confident learning motivates the need for further understanding of dataset uncertainty estimation, methods to clean training and test sets, and approaches to identify ontological and label issues for dataset curation. Future directions include validation of CL methods on more datasets such as the OpenML Benchmark~\citep{feurer2019openml}, the multi-modal Egocentric Communications (EgoCom) benchmark \citep{northcutt2020egocom}, and the realistic noisy label benchmark CNWL~\citep{jiang2020beyond}; evaluation of CL methods using other non-neural network models, such as random forests and XGBoost; examination of other threshold function formulations; examination of label errors in test sets and they affect machine learning benchmarks at scale~\citep{northcutt2021labelerrors}; assimilation of CL label error finding with pseudo-labeling and/or curriculum learning to \emph{dynamically} provide clean data during training; and further exploration of iterative and/or regression-based extensions of CL methods.

%%Confident learning is a principled step in that direction. 


\endinput

% In this paper we explore only a few possible applications of confident learning. We conclude with a consideration of how confident learning can be used in future research. Because CL finds label errors directly, it can be used to clean test sets, necessary for accurately benchmarking state-of-the-art. Because CL estimates the joint directly, it can be used to find ontological issues in datasets as we showed in Sec. \ref{sec:experiments}. CL may also be useful for finding \emph{hard} examples for datasets without label errors, useful in the context of hard-negatives. Finally, CL may be useful for meta-learning, i.e. learning with datasets instead of examples, by modeling the joint of label noise for each dataset.

% \endinput

% %%% PERHAPS the things below this line if there is room.

% Confident learning has a number of useful properties. We discuss a few in this section.

% \paragraph{Single iteration} Unlike most methods for learning with noisy labels, confident learning comprises one-shot, single iteration algorithms. This is an intentional choice to simplify incorporation into machine learning pipelines whilst adding negligible computational overhead. The reason confident learning is non-iterative is two-fold: (1) empirically, we found little improvement by retraining a classifier on the pruned set, re-estimating the joint for the original dataset, and re-estimating the label errors with the new joint and predicted probabilities, regardless of dataset, model, or noise distribution, and (2) proving convergence criterion in these settings without numerous simplifying assumptions remains unsolved. 

% \paragraph{Alien class noise} Noisy labels added from an alien class are dealt with \emph{correctly}. For example, we added `z' letters to the MNIST dataset and found all were ignored in the construction of the joint and all were identified as label errors due to low probability of belonging to any digit class.

% \paragraph{Two-step robustness} By separating the label noise characterization from finding label errors, we eliminate the dependency on the predicted probabilities common in learning with noisy labels literature \citep{Sukhbaatar_fergus_iclr_2015, jiang2018mentornet, NIPS2013_5073, Liu:2016:CNL:2914183.2914328}. Further, label errors are identified by predicted probability ranking, not exact value, enabling robustness to imperfect model probability estimation. Finally, the confident joint does not count examples





% Like ImageNet, many benchmark are often too large to guarantee error-free training labels, and as we show, error-free \emph{validation and test} labels. This has broad implications for the machine learning community because these datasets are benchmarks for fair comparison of results, but not if the test labels are inaccurate.

% to regulate policy and fairness when comparing algorithmic performance on datasets were labels are expected to be noiseless. When machine learning competitions like Kaggle and other competitions rank the performance of algorithms based on test accuracy, label errors in the test set undermine the validity of the competition. For example, one person's algorithm might make mistakes precisely where the test set has label errors, resulting in a pseudo-win and general misconception by the machine learning community as to which method is truly more accurate -- perhaps the second place person correctly labeled all the test label errors, resulting in decreased final accuracy, but their method may be overlooked moving forward.Confident learning is yields principled approaches to address these issues. 

% The tools afforded by confident learning allow us to automatically identify label errors in massive, often crowd-sourced, datasets like MNIST and Imagenet where the number of examples is too large for human-based labeling. In a world with ever-increasing amounts of data resulting in more datasets having noisy, crowd-sourced labels, we need principles approaches to deal with label noise. Confident learning meets this challenge with generality, speed, and simplicity. 

% repeat In the past two decades, the machine learning and vision communities have increasingly used the MNIST \citep{mnist_handwritten_digits_dataset_1998} and ImageNet \citep{imagenet} datasets as benchmarks to measure state-of-the-art progress and evaluate theoretical findings. The trustworthiness of these benchmarks rely on an implicit, and as we show fallacious, assumption that these datasets have noise-free labels. In this section, we unveil the existence of numerous label errors in both datasets and thereby demonstrate the efficacy of confident learning as a general tool for automatically detecting label errors in massive, crowd-sourced datasets.




% TODO - TO ADD
% Greater emphasis on reduction of test error (trained on a train set) when errors from test set were removed without access to the train set.
% As a note of practical importance, noisy labels should be generated with a different model and data representation then the model and representation you use for confident learning. This ensures the class-conditional independence assumption is not violated.
% Although this work and binary RankPruning both involve the use of confident examples, this work is largely not an extension of binary RankPruning and distinguishes itself in four ways: (1) nearly all the algorithmic steps are new (and simpler), (2) a primary contribution of binary RankPruning was to clarify learning assumptions and prove consistent noise rate estimators and equivalent risk minimization. To avoid overlap, we do not reprove those here, and instead prove the learnability criterion  (3) we've released the confident learning python package, (4) we solve real-world problems by finding label errors in the widely-used Imagenet and MNIST benchmark datasets. The main similarity is that 
% http://www.eng.biu.ac.il/goldbej/files/2012/05/ICLR2017.pdf - page 2, equation (1). they use the method of calculating p(y) same as fergus did - not robust! - we need to compare with them on benchmarks. their model is implemented here https://github.com/udibr/noisy_labels/blob/master/mnist-simple.ipynb
% MENTORNET (icml 2018) - http://proceedings.mlr.press/v80/jiang18c/jiang18c.pdf - The ability of deep CNNs to overfit or memorize the corrupted labels can lead to very poor generalization performance (Zhang et al., 2017a). Recently, Neyshabur et al. (2017) and Arpit et al. (2017) proposed deep learning generalization theories to explain this interesting phenomenon.


==> Confident Learning (JAIR 2021) (Version 6610)/experiments.tex <==



\section{Experiments}\label{sec:experiments}
This section empirically validates CL on CIFAR \citep{cifar10} and ImageNet \citep{ILSVRC15_imagenet} benchmarks. Sec. \ref{sec:exp_synth} presents CL performance on noisy examples in CIFAR where true labels are presumed known. Sec. \ref{sec:exp_imagenet} shows real-world label errors found in the original, unperturbed MNIST, ImageNet, WebVision, and Amazon Reviews datasets, and shows performance advantages using cleaned data provided by CL to train ImageNet. Unless otherwise specified, we compute out-of-sample predicted probabilities $\bm{\hat{P}}_{k,j}$ using four-fold cross-validation and ResNet architectures.

\subsection{Asymmetric Label Noise on CIFAR-10 dataset} \label{sec:exp_synth}

We evaluate CL on three criteria: (a) joint estimation  (Fig. \ref{fig:cifar10_joint_estimation}), (b) accuracy finding label errors  (Table \ref{table:cifar10_label_error_measures}), and (c) accuracy learning with noisy labels (Table \ref{table:cifar10_benchmark}).


% Following prior work~\cite{Sukhbaatar_fergus_iclr_2015, DBLP:conf/iclr/GoldbergerB17_smodel}, we study CL performance on non-uniformly random label noise for its resemblance to real-world noise. We generate noisy data from clean data by stochastically switching some labels of training examples to different classes non-uniformly according to a randomly generated $\nm$ noise transition matrix. We generate $\nm$ matrices with different traces to run experiments for different noise levels.  The noise matrices we used in our experiments are provided in Fig. \ref{cifar10_ground_truth_noise_matrices} in the Appendix.

\paragraph{Noise Generation} Following prior work by~\cite{Sukhbaatar_fergus_iclr_2015, DBLP:conf/iclr/GoldbergerB17_smodel}, we verify CL performance on the commonly used asymmetric label noise, where the labels of error-free/clean data are randomly flipped, for its resemblance to real-world noise. We generate noisy data from clean data by randomly switching some labels of training examples to different classes non-uniformly according to a randomly generated $\nm$ noise transition matrix. We generate $\nm$ matrices with different traces to run experiments for different noise levels. The noise matrices used in our experiments are in the Appendix in Fig. \ref{cifar10_ground_truth_noise_matrices}.
We generate noise in the CIFAR-10 training dataset across varying \emph{sparsities}, the fraction of off-diagonals in $\joint$ that are zero, and the percent of incorrect labels (noise).
%We avoid symmetric label noise because its rarely occurs naturally.
We evaluate all models on the unaltered test set.



%In our experiments, we consider \emph{sparsity}, the fraction of off-diagonals in the corruption noise matrix $\nm$ that are set to zero, typical of real-world label noise, e.g. \emph{dog} is more likely mislabeled \emph{fox} than \emph{cow}. The inclusion of sparsity is notable because higher sparsity produces less uniform noise which is more challenging, e.g. the mode label combined with clustering can often easily solve uniform random noise when the number of classes is large.

\paragraph{Baselines and our method} In Table \ref{table:cifar10_benchmark}, we compare CL performance versus seven recent highly competitive approaches and a vanilla baseline for multiclass learning with noisy labels on CIFAR-10, including \emph{INCV} \citep{chen2019confusion} which finds clean data with multiple iterations of cross-validation then trains on the clean set, \emph{SCE-loss} (symmetric cross entropy) \citep{wang2019sceloss_symmetric} which adds a reverse cross entropy term for loss-correction, \emph{Mixup} \citep{icml2018mixup} which linearly combines examples and labels to augment data, \emph{MentorNet} \citep{jiang2018mentornet} which uses curriculum learning to avoid noisy data in training, \emph{Co-Teaching} \citep{han2018coteaching} which trains two models in tandem to learn from clean data, \emph{S-Model} \citep{DBLP:conf/iclr/GoldbergerB17_smodel} which uses an extra softmax layer to model noise during training, and \emph{Reed} \citep{noisy_boostrapping_google_reed_iclr_2015} which uses loss-reweighting; and a \emph{Baseline} model that denotes a vanilla training with the noisy labels.

\paragraph{Training settings} All models are trained using ResNet-50 with the common setting: learning rate 0.1 for epoch [0,150), 0.01 for epoch [150,250), 0.001 for epoch [250,350); momentum 0.9; and weight decay 0.0001, except \emph{INCV}, \emph{SCE-loss}, and \emph{Co-Teaching} which are trained using their official GitHub code. Settings are copied from the \href{https://github.com/kuangliu/pytorch-cifar/tree/5e3f99093dfe7392fcbbc0b39582e4b0d3a64511#learning-rate-adjustment}{kuangliu/pytorch-cifar} GitHub open-source code and were not tuned by hand. We report the highest score across hyper-parameters $\alpha \in \{1, 2, 4, 8\}$ for \emph{Mixup} and $p \in \{0.7, 0.8, 0.9\}$ for \emph{MentorNet}. For fair comparison with \emph{Co-Teaching}, \emph{INCV}, and \emph{MentorNet}, we also train using the \emph{co-teaching} approach with $\text{forget rate} = 0.5 \times \text{[noise fraction]}$, and report the max accuracy of the two trained models for each method.
% instead of forget rate = noise as prescribed in \citet{han2018coteaching} because CL has already removed noisy examples beforehand.
We observe that dropping the last partial batch of each epoch during training improves stability by avoiding weight updates from, in some cases, a single noisy example). Exactly the same noisy labels are used for training all models for each column of Table \ref{table:cifar10_benchmark}. For our method, we fix its hyper-parameter, \emph{i.e.} the number of folds in cross-validation across different noise levels, and do not tune it on the validation set.
% Batch size 128, 256, and 512.
% In this table, we show the max of the three \emph{prune} methods (denoted CL: OPT) to make it easier to compare CL with the other methods: see Table \ref{table:cifar10_benchmark_all} in the Appendix for benchmarks of all CL methods.
%For input augmentation, all models used random horizontal flipping and cropped all images to 32x32. For a fair comparison, all models are trained .

For each CL method, sparsity, and noise setting, we report the mean accuracy in Table \ref{table:cifar10_benchmark}, averaged over ten trials, by varying the random seed and initial weights of the neural network for training. Standard deviations are reported in Table \ref{table:cifar10_benchmark_std} to improve readability. For each column in Table \ref{table:cifar10_benchmark}, the corresponding standard deviations in in Table \ref{table:cifar10_benchmark_std} are significantly less than the performance difference between CL methods and baseline methods. Notably, all standard deviations are significantly ($\sim$10x) less than the mean performance difference between the top-performing CL method and baseline methods for each setting, averaged over random weight initialization. Standard deviations are only reported for CL methods because of difficulty reproducing consistent results for some of the other methods.


% \begin{table*}[t]

% \setlength\tabcolsep{2pt} % Makes table columns tighter
% % \renewcommand{\arraystretch}{0.9}% Makes table rows tighter
% % \caption{AISTATS rebuttal -- caption disallowed.}
% \caption{Validation accuracy (\%) of confident learning versus recent methods for learning with noisy labels in CIFAR-10. CL methods estimate label errors, remove them, then train on the cleaned data. Whereas other methods decrease in performance with high sparsity (e.g. 0.6), CL methods are robust across sparsity, as indicated by the red highlighted cells.}
% \vskip -0.1in
% \label{table:cifar10_benchmark}
% % \tiny
% \begin{center}\
% \resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

% \begin{tabular}{l|c|cccc|cccc|cccc}
% \toprule
% Noise &    &  \multicolumn{4}{c}{0.2} & \multicolumn{4}{c}{0.4} & \multicolumn{4}{c}{0.7} \\
% Sparsity &  \textbf{AVG}  &    0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 \\
% \midrule

% CL: $\bm{C}_{\text{confusion}}$    &  69.2 &  89.6 &  89.6 &  89.9 &  89.9 &  \cellcolor{highlightcolor} 84.0 &  84.1 &  83.4 &  \cellcolor{highlightcolor} 84.4 &  31.8 &  39.6 &  33.5 &  30.5 \\
% CL: PBC       &  70.5 &  90.7 &  90.4 &  90.8 &  90.8 &  \cellcolor{highlightcolor} 84.7 &  85.8 &  85.1 &  \cellcolor{highlightcolor} 86.2 &  33.7 &  40.9 &  35.0 &  31.4 \\
% CL: $\cj$  &  71.4 &  \textbf{91.4} &  \textbf{90.9} &  \textbf{91.4} &  \textbf{91.4} &  \cellcolor{highlightcolor} 86.9 &  86.7 &  86.7 &  \cellcolor{highlightcolor} 87.2 &  32.9 &  41.8 &  34.5 &  35.0 \\
% CL: C+NR      &  72.5 &  90.9 &  90.8 &  91.1 &  91.1 &  \cellcolor{highlightcolor} \textbf{87.2} &  \textbf{87.0} &  86.8 &  \cellcolor{highlightcolor} 87.3 &  \textbf{41.3} &  41.4 &  38.9 &  36.4 \\
% CL: PBNR      &  \textbf{72.6} &  90.8 &  90.5 &  91.1 &  91.0 &  \cellcolor{highlightcolor} 87.1 &  86.9 &  \textbf{86.9} &  \cellcolor{highlightcolor} \textbf{87.4} &  41.0 &  \textbf{41.9} &  \textbf{39.1} &  \textbf{37.1} \\

% \midrule

% INCV (Chen et al., 2019)  & 66.1          & 87.8 & 88.6  & 89.6  & 89.2  & \cellcolor{highlightcolor} 84.4 &  76.6 &  85.4 &  \cellcolor{highlightcolor} 73.6  & 28.3  & 25.3 &  34.8  & 29.7 \\
% Mixup (Zhang et al., 2018)  & 62.2         & 85.6 & 86.8 & 87.0 & 84.3 & \cellcolor{highlightcolor} 76.1 & 75.4 &  68.6 & \cellcolor{highlightcolor} 59.8 & 32.2 & 31.3 & 32.3 & 26.9 \\
% SCE-loss (Wang et al., 2019)  & 61.5  &  87.2  &  87.5  &  88.8  &  84.4  &  \cellcolor{highlightcolor} 76.3  &  74.1  &  64.9  & \cellcolor{highlightcolor} 58.3  &  33.0  &  28.7  &  30.9  &  24.0  \\
% MentorNet (Jiang et al., 2018) &  59.0 &  84.9 &  85.1 &  83.2 &  83.4 &  \cellcolor{highlightcolor} 64.4 &  64.2 &  62.4 &  \cellcolor{highlightcolor} 61.5 &  30.0 &  31.6 &  29.3 &  27.9 \\
% Co-Teaching (Han et al., 2018)  & 56.9   &  81.2 &  81.3 &  81.4 &  80.6 & \cellcolor{highlightcolor} 62.9 &  61.6 &  60.9 & \cellcolor{highlightcolor} 58.1 &  30.5 &  30.2 &  27.7 &  26.0 \\
% S-Model (Goldberger et al., 2017)    &  55.6 &  80.0 &  80.0 &  79.7 &  79.1 &  58.6 &  61.2 &  59.1 &  57.5 &  28.4 &  28.5 &  27.9 &  27.3 \\
% Reed (Reed et al., 2015)      &  56.0 &  78.1 &  78.9 &  80.8 &  79.3 &  60.5 &  60.4 &  61.2 &  58.6 &  29.0 &  29.4 &  29.1 &  26.8 \\
% Baseline   &  55.4 &  78.4 &  79.2 &  79.0 &  78.2 &  60.2 &  60.8 &  59.6 &  57.3 &  27.0 &  29.7 &  28.2 &  26.8 \\

% \bottomrule
% \end{tabular}
% }

% \end{center}
% % \vskip 0in
% \end{table*}


\begin{table*}[t]

\setlength\tabcolsep{2pt} % Makes table columns tighter
% \renewcommand{\arraystretch}{0.9}% Makes table rows tighter
% \caption{AISTATS rebuttal -- caption disallowed.}
\caption{Test accuracy (\%) of confident learning versus recent methods for learning with noisy labels in CIFAR-10. Scores reported for CL methods are averaged over ten trials with standard deviations shown in Table \ref{table:cifar10_benchmark_std}. CL methods estimate label errors, remove them, then train on the cleaned data. Whereas other methods decrease in performance from low sparsity (e.g., 0.0) to high sparsity (e.g. 0.6), CL methods are robust across sparsity, as indicated by comparing the two column-wise red highlighted cells. Data-centric AI methods (\textit{CL, INCV, Mixup}) outperform model-centric methods (\textit{SCE-Loss, MentorNet, Co-Teaching, S-Model}).}
\vskip -0.1in
\label{table:cifar10_benchmark}
% \tiny
\begin{center}\
\resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\begin{tabular}{l|cccc|cccc|cccc}
\toprule
Noise &  \multicolumn{4}{c}{20\%} & \multicolumn{4}{c}{40\%} & \multicolumn{4}{c}{70\%} \\
Sparsity  &    0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 \\
\midrule

CL: $\bm{C}_{\text{confusion}}$    &  89.6 &  89.4 &  90.2 &  89.9 &  \cellcolor{highlightcolor} 83.9 &  83.9 &  83.2 &  \cellcolor{highlightcolor} 84.2 &  31.5 &  39.3 &  33.7 &  30.6 \\
CL: PBC                            &  90.5 &  90.1 &  90.6 &  90.7 &  \cellcolor{highlightcolor} 84.8 &  85.5 &  85.3 &  \cellcolor{highlightcolor} 86.2 &  33.7 &  40.7 &  35.1 &  31.4 \\
CL: $\cj$                          &  \textbf{91.1} &  \textbf{90.9} &  \textbf{91.1} &  \textbf{91.3} & \cellcolor{highlightcolor}  86.7 &   86.7 &  86.6 & \cellcolor{highlightcolor} 86.9 &  32.4 &  \textbf{41.8} &  34.4 &  34.5 \\
CL: C+NR                           &  90.8 &  90.7 &  91.0 &  91.1 &  \cellcolor{highlightcolor} \textbf{87.1} &  \textbf{86.9} &  \textbf{86.7} & \cellcolor{highlightcolor} \textbf{87.2} &  \textbf{41.1} &  41.7 &  39.0 &  32.9 \\
CL: PBNR                           &  90.7 &  90.5 &  90.9 &  90.9 &  \cellcolor{highlightcolor} \textbf{87.1} &  86.8 &  86.6 &  \cellcolor{highlightcolor} \textbf{87.2} &  41.0 &  \textbf{41.8} &  \textbf{39.1} &  \textbf{36.4} \\

\midrule

INCV (Chen et al., 2019)  & 87.8 & 88.6  & 89.6  & 89.2  & \cellcolor{highlightcolor} 84.4 &  76.6 &  85.4 &  \cellcolor{highlightcolor} 73.6  & 28.3  & 25.3 &  34.8  & 29.7 \\
Mixup (Zhang et al., 2018)  & 85.6 & 86.8 & 87.0 & 84.3 & \cellcolor{highlightcolor} 76.1 & 75.4 &  68.6 & \cellcolor{highlightcolor} 59.8 & 32.2 & 31.3 & 32.3 & 26.9 \\
SCE-loss (Wang et al., 2019)  &  87.2  &  87.5  &  88.8  &  84.4  &  \cellcolor{highlightcolor} 76.3  &  74.1  &  64.9  & \cellcolor{highlightcolor} 58.3  &  33.0  &  28.7  &  30.9  &  24.0  \\
MentorNet (Jiang et al., 2018) &  84.9 &  85.1 &  83.2 &  83.4 &  \cellcolor{highlightcolor} 64.4 &  64.2 &  62.4 &  \cellcolor{highlightcolor} 61.5 &  30.0 &  31.6 &  29.3 &  27.9 \\
Co-Teaching (Han et al., 2018)  &  81.2 &  81.3 &  81.4 &  80.6 & \cellcolor{highlightcolor} 62.9 &  61.6 &  60.9 & \cellcolor{highlightcolor} 58.1 &  30.5 &  30.2 &  27.7 &  26.0 \\
S-Model (Goldberger et al., 2017)    &  80.0 &  80.0 &  79.7 &  79.1 &  58.6 &  61.2 &  59.1 &  57.5 &  28.4 &  28.5 &  27.9 &  27.3 \\
Reed (Reed et al., 2015)      &  78.1 &  78.9 &  80.8 &  79.3 &  60.5 &  60.4 &  61.2 &  58.6 &  29.0 &  29.4 &  29.1 &  26.8 \\
Baseline   &  78.4 &  79.2 &  79.0 &  78.2 &  60.2 &  60.8 &  59.6 &  57.3 &  27.0 &  29.7 &  28.2 &  26.8 \\

\bottomrule
\end{tabular}
}

\end{center}
\vskip -.2in
\end{table*}


\begin{table*}[!b]
\setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.9}% Makes table rows tighter
\caption{Standard deviations (\% units) associated with the mean score (over ten trials) for scores reported for CL methods in Table \ref{table:cifar10_benchmark}. Each trial uses a different random seed and network weight initialization. No standard deviation exceeds 2\%.}
\vskip -0.1in
\label{table:cifar10_benchmark_std}
% \tiny
\begin{center}
\resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\setlength{\tabcolsep}{6.5pt}
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
Noise &  \multicolumn{4}{c}{20\%} & \multicolumn{4}{c}{40\%} & \multicolumn{4}{c}{70\%} \\
Sparsity  &    0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 &      0 &      0.2 &      0.4 &      0.6 \\
\midrule
CL: $\bm{C}_{\text{confusion}}$  &  0.07 &  0.10 &  0.17 &  0.08 &  0.19 &  0.22 &  0.23 &  0.20 &  0.93 &  0.24 &  0.13 &  0.26 \\
CL: PBC     &  0.14 &  0.12 &  0.11 &  0.10 &  0.15 &  0.17 &  0.16 &  0.10 &  0.12 &  0.22 &  0.11 &  0.30 \\
CL: $\cj$ &  0.17 &  0.09 &  0.17 &  0.11 &  0.10 &  0.20 &  0.09 &  0.13 &  1.02 &  0.15 &  0.18 &  1.63 \\
CL: C+NR    &  0.09 &  0.10 &  0.08 &  0.08 &  0.11 &  0.14 &  0.16 &  0.10 &  0.42 &  0.33 &  0.26 &  1.90 \\
CL: PBNR    &  0.15 &  0.09 &  0.09 &  0.10 &  0.18 &  0.10 &  0.15 &  0.12 &  0.26 &  0.28 &  0.24 &  1.43 \\
\bottomrule
\end{tabular}
}

\end{center}
% \vskip 0in
\end{table*}


%The standard deviations corresponding to the mean scores in Table \ref{table:cifar10_benchmark}, are reported separately in Table \ref{table:cifar10_benchmark_std} to improve readability. For each column in Table \ref{table:cifar10_benchmark}, the corresponding standard deviations in in Table \ref{table:cifar10_benchmark_std} are significantly less than the performance difference between CL methods and baseline methods.






\begin{figure*}[!b]
    \centering
    \begin{subfigure}[b]{0.345 \textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/cifar10_true_joint_noise_4_sparsity_6.pdf}
        \caption[Network2]%
        {True $\joint$ (unknown to CL)}    
        \label{subfig:true_joint}
    \end{subfigure}
    \begin{subfigure}[b]{0.285\textwidth}  
        \centering 
        \includegraphics[width=1\textwidth]{img/cifar10_est_joint_noise_4_sparsity_6.pdf}
        \caption[]%
        {CL estimated $\estjoint$}   
        \label{subfig:est_joint}
    \end{subfigure}
    \begin{subfigure}[b]{0.349\textwidth}   
        \centering 
        \includegraphics[width=1\textwidth]{img/cifar10_abs_diff_noise_4_sparsity_6.pdf}
        \caption[]%
        {Absolute diff. $ \lvert \bm{Q}_{\tilde{y}, y^*} - \hat{\bm{Q}}_{\tilde{y}, y^*} \rvert$}
        \label{subfig:abs_diff}
    \end{subfigure}
% \vskip -0.1in
    \caption{Our estimation of the joint distribution of noisy labels and true labels for CIFAR with 40\% label noise and 60\% sparsity. Observe the similarity (RSME $=.004$) between (a) and (b) and the low absolute error in every entry in (c). Probabilities are scaled up by 100.} 
% \vskip -0.1in
    \label{fig:cifar10_joint_estimation}
\end{figure*}

We also evaluate CL's accuracy in finding label errors. In Table \ref{table:cifar10_label_error_measures}, we compare five variants of CL methods across noise and sparsity and report their precision, recall, and F1 in recovering the true label. The results show that CL is able to find the label errors with high recall and reasonable F1. 


\begin{table*}[t]

\setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{1}% Makes table rows tighter
\caption{Mean accuracy, F1, precision, and recall measures of CL methods for finding label errors in CIFAR-10, averaged  over ten trials.}
\vskip -0.1in
\label{table:cifar10_label_error_measures}
% \tiny
\begin{center}
% \begin{sc}
\resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccc|cccc|cccc|cccc}

\toprule
Measure &\multicolumn{4}{c}{Accuracy (\%) $\pm$ Std. Dev. (\%)} & \multicolumn{4}{c}{F1 (\%)} & \multicolumn{4}{c}{Precision (\%)}  & \multicolumn{4}{c}{Recall (\%)} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
Noise & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%}  & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%} \\
Sparsity &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6  &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6  &   0.0 &   0.6 &   0.0 &   0.6 \\
\midrule
CL: $\bm{C}_{\text{confusion}}$ &  $84{\pm}0.07$  &  $85{\pm}0.09$ &  $85{\pm}0.24$ &  $81{\pm}0.21$ &  71 &  72 &  84 &  79 & 56 &  58 &  74 &  70 & \textbf{98} &  \textbf{97} &  \textbf{97} &  \textbf{90} \\
CL: $\cj$ &  $89{\pm}0.15$ &  \textbf{90}${\pm}0.10$ &  $86{\pm}0.15$ &  \textbf{84}${\pm}0.12$ &  75 &  78 &  84 &  \textbf{80} &  \textbf{67} &  \textbf{70} &  78 &  77 & 86 &  88 &  91 &  84 \\
CL: PBC           &  $88{\pm}0.22$ &  $88{\pm}0.11$ &  $86{\pm}0.17$ &  $82{\pm}0.13$ &  76 &  76 &  84 &  79 &  64 &  65 &  76 &  74 &  96 &  93 &  94 &  85\\
CL: PBNR          &  $89{\pm}0.11$ &  \textbf{90}${\pm}0.08$ &  \textbf{88}${\pm}0.12$ &  \textbf{84}${\pm}0.11$ &  77 &  \textbf{79} &  \textbf{85} &  \textbf{80} &  65 &  68 &  \textbf{82} &  \textbf{79} &  93 &  94 &  88 &  82 \\
CL: C+NR          &  \textbf{90}${\pm}0.21$ &  \textbf{90}${\pm}0.10$ &  $87{\pm}0.23$ &  $83{\pm}0.14$ &  \textbf{78} &  78 &  84 &  78 &  \textbf{67} &  69 &  \textbf{82} &  \textbf{79} &  93 &  90 &  87 &  78 \\
\bottomrule
\end{tabular}
}

% \end{sc}
\end{center}
% \vskip -0.15in
\end{table*}





\paragraph{Robustness to Sparsity} Table \ref{table:cifar10_benchmark} reports CIFAR test accuracy for learning with noisy labels across noise amount and sparsity, where the first five rows report our CL approaches. As shown, CL consistently performs well compared to prior art across all noise and sparsity settings.
We observe significant improvement in high-noise and/or high-sparsity regimes.
% Table \ref{table:cifar10_benchmark} is the first to benchmark modern approaches for realistic class-conditional noise. Prior art typically benchmarks symmetric noise which does not occur normally in real datasets, CL does not decrease in accuracy for realistic, high sparsity noise.
The simplest CL method $CL: \bm{C}_{\text{confusion}}$ performs similarly to \emph{INCV} and comparably to prior art with best performance by \textbf{$\cj$} across all noise and sparsity settings. The results validate the benefit of directly modeling the joint noise distribution and show that our method is competitive compared to highly competitive, robust learning methods.


%The no-noise test accuracy for the CL models (in PyTorch) is 0.895 versus 0.935 for the other models (in TensorFlow), likely due to pipeline differences, thus the improvement of confident learning over prior art is significant as shown in Table \ref{table:cifar10_benchmark}.
% CL is the only approach with robustness to highly sparse, non-uniform label noise, modeled after real-world datasets like ImageNet.
% Among these methods, CL is the only approach that does not decrease accuracy for realistic, sparse, non-uniform label noise. 

To understand why CL performs well, we evaluate CL joint estimation across noise and sparsity with RMSE in Table \ref{table:cifar10_rmse} in the Appendix and estimated $\estjoint$ in Fig. \ref{cifar10_abs_diff_ALL} in the Appendix. For the 20\% and 40\% noise settings, on average, CL achieves an RMSE of $.004$ relative to the true joint $\joint$ across all sparsities. The simplest CL variant, $\bm{C}_{\text{confusion}}$ normalized via Eqn. (\ref{eqn_calibration}) to obtain $\hat{\bm{Q}}_{\text{confusion}}$, achieves a slightly worse RMSE of $.006$. 

In Fig. \ref{fig:cifar10_joint_estimation}, we visualize the quality of CL joint estimation in a challenging high-noise (40\%), high-sparsity (60\%) regime on CIFAR. Subfigure (a) demonstrates high sparsity in the latent true joint $\joint$, with over half the noise in just six noise rates. Yet, as can be seen in subfigures (b) and (c), CL still estimates over 80\% of the entries of $\joint$ within an absolute difference of $.005$. The results empirically substantiate the theoretical bounds of Section~\ref{sec:theory}.








In Table \ref{table:incv_stuff} (see Appendix), we report the training time required to achieve the accuracies reported in Table \ref{table:cifar10_benchmark} for INCV and confident learning. As shown in Table \ref{table:incv_stuff}, INCV training time exceeded 20 hours. In comparison, CL takes less than three hours on the same machine: an hour for cross-validation, less than a minute to find errors, and an hour to re-train.

%\lu{do you have theory or principle to explain the high-recall? If yes say it there. Curtis: good point, but requires some thought. will save this for last.}
%We observe accuracy between 84\% and 88\% finding label errors at 40\% label noise.


\subsection{Real-world Label Errors in ILSVRC12 ImageNet Train Dataset}\label{sec:exp_imagenet}

\citet{ILSVRC15_imagenet} suggest label errors exist in ImageNet due to human error, but to our knowledge, few attempts have been made to find label errors in the ILSVRC 2012 training set, characterize them, or re-train without them. Here, we consider each application. We use ResNet18 and ResNet50 architectures with standard settings: 0.1 initial learning rate, 90 training epochs with 0.9 momentum. 


\begin{table}[ht]
% \setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.8}% Makes table rows tighter
\caption{Ten largest non-diagonal entries in the confident joint $\cj$ for ImageNet train set used for ontological issue discovery. A duplicated class detected by CL is highlighted in red.}
% \vskip -0.05in
\label{table_imagenet_characterization_top10}
\begin{center}
% \tiny
% \resizebox{.8\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\begin{tabular}{rrrrrrr} 
\toprule
  $\cj$   &  $\tilde{y}$ name   &   $y^*$ name   &   $\tilde{y}$ nid   &   $y^*$ nid   &  $\bm{C}_{\text{confusion}}$  &   $\estjoint$  \\
\midrule
    645 &       projectile &       missile &       n04008634 &  n03773504 &   494  &            0.00050 \\
    539 &              tub &       bathtub &       n04493381 &  n02808440 &   400  &            0.00042 \\
    476 &      breastplate &       cuirass &       n02895154 &  n03146219 &   398  &            0.00037 \\
    437 &     green\_lizard &     chameleon &      n01693334 &  n01682714 &   369  &            0.00034 \\
    435 &        chameleon &  green\_lizard &      n01682714 &  n01693334 &   362  &            0.00034 \\
    433 &          missile &    projectile &       n03773504 &  n04008634 &   362  &            0.00034 \\
    \cellcolor{highlightcolor} 417 &         \cellcolor{highlightcolor} maillot &      \cellcolor{highlightcolor} maillot &      \cellcolor{highlightcolor} n03710637 &  \cellcolor{highlightcolor} n03710721 &  \cellcolor{highlightcolor} 338  &           \cellcolor{highlightcolor}  0.00033 \\
    416 &     horned\_viper &    sidewinder &      n01753488 &  n01756291 &   336  &            0.00033 \\
    410 &             corn &           ear &       n12144580 &  n13133613 &   333  &            0.00032 \\
    407 &        keyboard &     space\_bar &      n04505470 &  n04264628 &   293  &            0.00032 \\
\bottomrule
\end{tabular}
% }


\end{center}
% \vskip -0.1in
\end{table}


% \begin{table}[ht]
% % \vskip -0.05in
% % \setlength\tabcolsep{2pt} % Makes table columns tighter
% \renewcommand{\arraystretch}{0.8}% Makes table rows tighter
% \caption{Ten largest non-diagonal entries in the confident joint $\cj$ for ImageNet train set used for ontological issue discovery. }
% % \vskip -0.05in
% \label{table_imagenet_characterization_top10}
% \begin{center}
% % \tiny
% % \resizebox{.8\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

% \begin{tabular}{lllrr} 
% \toprule
%   $\cj$  & $\tilde{y}$ name   &   $y^*$ name  &  $\bm{C}_{\text{confusion}}$   &   $\estjoint$   \\
% \midrule
%     645 &       projectile &       missile &       494 &  0.00050   \\
%     539 &              tub &       bathtub &       400 &  0.00042   \\
%     476 &      breastplate &       cuirass &       398 &  0.00037   \\
%     437 &     green\_lizard &     chameleon &      369 &  0.00034   \\
%     435 &        chameleon &  green\_lizard &      362 &  0.00034   \\
%     433 &          missile &    projectile &       362 &  0.00034   \\
%     417 &          maillot &       maillot &       338 &  0.00033   \\
%     416 &     horned\_viper &    sidewinder &      336 &  0.00033   \\
%     410 &             corn &           ear &       333 &  0.00032   \\
%     407 &         keyboard &     space\_bar &      293 &  0.00032   \\
% \bottomrule
% \end{tabular}
% % }


% \end{center}
% % \vskip -0.2in
% \end{table}




\paragraph{Ontological discovery for dataset curation} Because ImageNet is an one-hot class dataset, the classes are required to be mutually exclusive. Using ImageNet as a case study, we observe auto-discovery of ontological issues at the class level in Table \ref{table_imagenet_characterization_top10}, operationalized by listing the 10 largest non-diagonal entries in $\cj$. For example, the class \emph{maillot} appears twice, the existence of \emph{is-a} relationships like \emph{bathtub is a tub}, misnomers like \emph{projectile} and \emph{missile}, and unanticipated issues caused by words with multiple definitions like \emph{corn} and \emph{ear}. We include the baseline $\bm{C}_{\text{confusion}}$ to show that while $\bm{C}_{\text{confusion}}$ finds fewer label errors than $\cj$, they rank ontological issues similarly.


\begin{figure*}[ht]
% \vskip -.1in
\centerline{\includegraphics[width=\textwidth]{img/imagenet_train_label_errors_32.jpg}}
% \vskip -.1in
\caption{Top 32 (ordered automatically by normalized margin) identified label issues in the 2012 ILSVRC ImageNet train set using CL: PBNR. Errors are boxed in red. Ontological issues are boxed in green. Multi-label images are boxed in blue.} 
\label{label_errors_imagenet_train_top32}
\end{figure*}

% \vskip -.1in



\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/resnet_imagenet_feb_2021/resnet18_imagenet_comparison_cl_methods_5_trials.pdf}
        \caption[Network2]%
        {Accuracy on the ILSVRC2012 validation set}    
        \label{fig_resnet18_val_acc}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{img/resnet_imagenet_feb_2021/resnet18_acc_of_20_noisiest_classes_5_trials.pdf}
        \caption[]%
        {Accuracy on the top 20 noisiest classes}   
        \label{fig_resnet18_top20_noise}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{img/resnet_imagenet_feb_2021/resnet18_acc_of_noisiest_class_foxhound_5_trials.pdf}
        \caption[]%
        {Accuracy on the noisiest class: foxhound}
        \label{fig_resnet18_foxhound}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{img/resnet_imagenet_feb_2021/resnet18_acc_of_a_noisy_class_maillot_5_trials.pdf}
        \caption[]%
        {Accuracy on known erroneous class: maillot} 
        \label{fig_resnet18_maillot}
    \end{subfigure}
    % \vskip -.1in
    \caption{ResNet-18 Validation Accuracy on ImageNet (ILSVRC2012) when 20\%, 40\%, ..., 100\% of the label issues found using confident learning are removed prior to training (blue, solid line) compared with random examples removed prior to training (orange, dash-dotted line). Each subplot is read from left-to-right as incrementally more CL-identified issues are removed prior to training (shown by the x-axis). The translucent black dotted verticals bars measure the improvement when removing examples with CL vs random examples. Each point in all subfigures represents an independent training of ResNet-18 from scratch. Each point on the graph depicts the average accuracy of 5 trials (varying random seeding and weight initialization). The capped, colored vertical bars depict the standard deviation. } 
    % \vskip .2in
    \label{fig_imagenet_resnet18_training}
\end{figure*}


\paragraph{Finding label issues}
Fig. \ref{label_errors_imagenet_train_top32} depicts the top 16 label issues found using CL: PBNR with ResNet50 ordered by the normalized margin. We use the term \emph{issue} versus \emph{error} because examples found by CL consist of a mixture of multi-label images, ontological issues, and actual label errors. Examples of each are indicated by colored borders in the figure.
% Across methods: 406k (\textbf{CL: $\bm{C}_{\text{confusion}}$}), 141k (\textbf{CL:} $\cj$), 209k (\textbf{CL: PBC}),  194k (\textbf{CL: PBNR}),  110k (\textbf{CL: C+NR}) label errors were estimated in the ImageNet train set. 
To evaluate CL in the absence of true labels, we conducted a small-scale human validation on a random sample of 500 errors (as identified using CL: PBNR) and found 58\% were either multi-label, ontological issues, or errors. ImageNet data are often presumed error-free, yet ours is the first attempt to identify label errors automatically in ImageNet training images. 








% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.235\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{img/resnet_imagenet/resnet50_imagenet_validation_acc.pdf}
%         \caption[Network2]%
%         {Acc of Validation Set}    
%         \label{fig_resnet50_val_acc}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.235\textwidth}  
%         \centering 
%         \includegraphics[width=1\textwidth]{img/resnet_imagenet/resnet50_acc_of_20_noisiest_classes.pdf}
%         \caption[]%
%         {Acc 20 noisiest classes}   
%         \label{fig_resnet50_top20_noise}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.235\textwidth}   
%         \centering 
%         \includegraphics[width=1\textwidth]{img/resnet_imagenet/resnet50_acc_of_noisiest_class:_foxhound.pdf}
%         \caption[]%
%         {Acc of noisiest class}
%         \label{fig_foxhound}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[b]{0.235\textwidth}   
%         \centering 
%         \includegraphics[width=1\textwidth]{img/resnet_imagenet/resnet50_acc_of_a_noisy_class:_bighorn.pdf}
%         \caption[]%
%         {Acc of class bighorn} 
%         \label{fig_bighorn}
%     \end{subfigure}
%     \caption{ResNet50 Val Accuracy on ImageNet when 20\%, 40\%,...,100\% of the label errors found automatically with confident learning are removed prior to training from scratch. Vertical bars depict the improvement or reduction when removing examples with confident learning vs random examples.} 
%     \label{fig_imagenet_training}
% \end{figure*}



\begin{figure*}[hbt!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/resnet_imagenet_july_2020/resnet50_imagenet_comparison_cl_methods.pdf}
        \caption[Network2]%
        {Accuracy on the ILSVRC2012 validation set}    
        \label{fig_resnet50_val_acc}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\linewidth]{img/resnet_imagenet_july_2020/resnet50_acc_of_20_noisiest_classes.pdf}
        \caption[]%
        {Accuracy on the top 20 noisiest classes}   
        \label{fig_resnet50_top20_noise}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\linewidth]{img/resnet_imagenet_july_2020/resnet50_acc_of_noisiest_class_foxhound.pdf}
        \caption[]%
        {Accuracy on the noisiest class: foxhound}
        \label{fig_resnet50_foxhound}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\linewidth]{img/resnet_imagenet_july_2020/resnet50_acc_of_a_noisy_class_maillot.pdf}
        \caption[]%
        {Accuracy on known erroneous class: maillot} 
        \label{fig_resnet50_maillot}
    \end{subfigure}
    % \vskip -.05in
    \caption{Replication of the experiments in Fig. \ref{fig_imagenet_resnet18_training} with ResNet-50. Each point in each subfigure depicts the accuracy of a single trial (due to computational limitations). Error bars, shown by the colored vertical lines, are estimated via Clopper-Pearson intervals for subfigures (a) and (b). For additional information, see the caption of Fig. \ref{fig_imagenet_resnet18_training}.} 
    % \vskip .2in
    \label{fig_imagenet_training}
\end{figure*}




\paragraph{Training ResNet on ImageNet with label issues removed}
By providing cleaned data for training, we explore how CL can be used to achieve similar or better validation accuracy on ImageNet when trained with less data.
To understand the performance differences, we train ResNet-18 (Fig. \ref{fig_imagenet_resnet18_training}) on progressively less data, removing 20\%, 40\%,..., 100\% of ImageNet train set label issues identified by CL and training from scratch each time. Fig. \ref{fig_imagenet_resnet18_training} depicts the top-1 validation accuracy when training with cleaned data from CL versus removing uniformly random examples, on each of (a) the entire ILSVRC validation set, (b) the 20 (noisiest) classes with the smallest diagonal in $\cj$, (c) the foxhound class, which has the smallest diagonal in $\cj$, and (d) the maillot class, a known erroneous class, duplicated accidentally in ImageNet, as previously published \citep{hoffman2015detector}, and verified (c.f. line 7 in Table \ref{table_imagenet_characterization_top10}). For readability, we plot the best performing CL method at each point and provide the individual performance of each CL method in the Appendix (see Fig. \ref{fig:imagenet_learning_with_noisy_labels}). For the case of a single class, as shown in Fig. \ref{fig_imagenet_resnet18_training}(c) and \ref{fig_imagenet_resnet18_training}(d), we show the recall using the model's top-1 prediction, hence the comparatively larger variance in classification accuracy reported compared to (a) and (b). We observed that CL outperforms the random removal baseline in nearly all experiments, and improves on the no-data-removal baseline accuracy, depicted by the left-most point in the subfigures, on average over the five trials for the 1,000 and 20 class settings, as shown in  Fig. \ref{fig_imagenet_resnet18_training}(a) and \ref{fig_imagenet_resnet18_training}(b). To verify the result is not model-specific, we repeat each experiment for a single trial with ResNet-50 (Fig. \ref{fig_imagenet_training}) and find that CL similarly outperforms the random removal baseline. 

% In Figure \ref{fig_imagenet_training} we demonstrate how the validation accuracy of ResNet50 improves when removing label errors estimated with confident learning versus random examples. In subfigure (a), we see the validation accuracy when random pruning is used versus confident learning. Subfigure (b) shows how that discrepancy increases as we look at the 20 noisiest classes identified by confident learning. The bottom two figures show a consistent increase in accuracy for the class identified as most noisy by confident learning (c) and a moderately noisy class (d). For subfigure (d), the spike improvement is in the middle because confident learning ranks examples and this class is not ranked as the noisiest, so the label errors in that class do not get removed until 40\%-60\% of label errors are removed. 

%For a fair comparison, we make no effort to remove label errors in the validation set: the cleaned train set may induce distributional shift, making the moderate accuracy increase notable. 
These results suggest that CL can reduce the size of a real-world noisy training dataset by 10\% while still moderately improving the validation accuracy (Figures \ref{fig_resnet18_val_acc}, \ref{fig_resnet18_top20_noise}, \ref{fig_resnet50_val_acc}, \ref{fig_resnet50_top20_noise}) and significantly improving the validation accuracy on the erroneous maillot class (Figures \ref{fig_resnet18_maillot}, \ref{fig_resnet50_maillot}). While we find CL methods may improve the standard ImageNet training on clean training data by filtering out a subset of training examples, the significance of this result lies not in the magnitude of improvement, but as a warrant of exploration in the use of cleaning methods when training with ImageNet, which is typically assumed to have correct labels. Whereas many of the label issues in ImageNet are due to multi-labeled examples \citep{yun2021relabelimagenet}, next we consider a dataset with disjoint classes.


\subsection{Amazon Reviews Dataset: CL using logistic regression on noisy text data}


The Amazon Reviews dataset is a corpus of textual reviews labeled with 1-star to 5-star ratings from Amazon customers used to benchmark sentiment analysis models~\citep{he2016ups_amazonreviews}. We study the 5-core (9.9 GB) variant of the dataset -- the subset of data in which all users and items have at least 5 reviews. 2-star and 4-star reviews are removed due to ambiguity with 1-star and 5-star reviews, respectively. Left in the dataset, 2-star and 4-star reviews could inflate error counts, making CL appear to be more effective than it is.

This subsection serves three goals. First, we use a logistic regression classifier, as opposed to a deep-learning model, for our experiments in this section to evaluate CL for non-deep-learning methods. Second, we seek to understand how CL may improve learning with noise in the label space of text data, but not noise in the text data itself (e.g. typos). Towards this goal, we consider non-empty reviews with more ``helpful'' up-votes than down-votes -- the resulting dataset consists of approximately ten million reviews. Finally, Theorem \ref{thm:robustness} shows that CL is robust to class-imbalance, but datasets like ImageNet and CIFAR-10 are balanced by construction: the Amazon Reviews dataset, however, is naturally and extremely imbalanced -- the distribution of given labels (i.e., the noisy prior), is: 9\% 1-star reviews:, 12\% 3-star reviews, and 79\% 5-star reviews.  We seek to understand if CL can find label errors and improve performance in learning with noisy labels in this class-imbalanced setting.

\paragraph{Training settings} \label{amazon_reviews_training_settings} To demonstrate that non-deep-learning methods can be effective in finding label issues under the CL framework, we use a multinomial logistic regression classifier for both finding label errors and learning with noisy labels. The built-in SGD optimizer in the open-sourced fastText library \citep{fasttext_bag_of_tricks} is used with settings: initial learning rate = 0.1, embedding dimension = 100, and n-gram = 3). Out-of-sample predicted probabilities are obtained via 5-fold cross-validation. For input during training, a review is represented as the mean of pre-trained, tri-gram, word-level fastText embeddings \citep{bojanowski2017_fasttext_word_representations}.


\paragraph{Finding label issues} Table \ref{amazon} shows examples of label issues in the Amazon Reviews dataset found automatically using the CL: C+NR variant of confident learning. We observe qualitatively that most label issues identified by CL in this context are reasonable except for sarcastic reviews, which appear to be poorly modeled by the bag-of-words approach.


\begin{table}[ht]
% \vskip -0.05in
% \setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.8}% Makes table rows tighter
\caption{Top 20 CL-identified label issues in the Amazon Reviews text dataset using CL: C+NR, ordered by normalized margin. A logistic regression classifier trained on fastText embeddings is used to obtain out-of-sample predicted probabilities. Most errors are reasonable, with the exception of sarcastic reviews, which are poorly modeled by the bag-of-words model. }
\vskip -0.15in
\label{amazon}
\begin{center}
% \tiny
\resizebox{.99\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\begin{tabular}{rcc}
\toprule
\textbf{Review} & \textbf{Given Label} & \textbf{CL Guess} \\
\midrule
                                                     A very good addition to kindle. Cleans and scans. Very easy  TO USE &        $\star$ &     $\star\star\star\star\star$ \\
                                                                                         Buy it and enjoy a great story. &        $\star\star\star$ &     $\star\star\star\star\star$ \\
               Works great! I highly recommend it to everyone that enjoys singing hymns! Love it! Love it! Love it! :) . &        $\star\star\star$ &     $\star\star\star\star\star$ \\
                Awesome it was better than all the other my weirder school books.  I love it! The best book ever.Awesome &        $\star$ &     $\star\star\star\star\star$ \\
     I gave this 5 stars under duress.  I would rather give it 3 stars.  it plays fine but it is a little boring so far. &        $\star\star\star\star\star$ &     $\star\star\star$ \\
                                                                          only six words: don't waist your money on this &        $\star\star\star\star\star$ &     $\star$ \\
                        I love it so much at first I though it would be boring but turns out its fun for all ages get it &        $\star$ &     $\star\star\star\star\star$ \\
         Excellent read, could not put it down! Keep up the great works ms. Brown. Cannot wait to download the next one. &        $\star$ &     $\star\star\star\star\star$ \\
                         This is one of the easiest to use games I have ever played. It is adaptable and fun. I love it. &        $\star$ &     $\star\star\star\star\star$ \\
                                                                               So this is what today's music has become? &        $\star$ &     $\star\star\star\star\star$ \\
           Sarah and Charlie, what a wonderful story. I loved this book and look forward to reading more of this series. &        $\star\star\star$ &     $\star\star\star\star\star$ \\
                              I've had this for over a year and it works very well.  I am very happy with this purchase. &        $\star$ &     $\star\star\star\star\star$ \\
                                               this show is insane and I love it. I will be ordering more seasons of it. &        $\star\star\star$ &     $\star\star\star\star\star$ \\
                                                                            Just what the world needs, more generic r\&b. &        $\star$ &     $\star\star\star\star\star$ \\
                                    I did like the Making Of This Is movie it  okay it not the best okay it not great  . &        $\star$ &     $\star\star\star$ \\
                                                        Tough game. But of course it has the very best sound track ever! &        $\star$ &     $\star\star\star\star\star$ \\
                                                                           unexpected kid on the way thanks to this shit &        $\star$ &     $\star\star\star\star\star$ \\
                                   The kids are fascinated by it, Plus my wife loves it.. I love it I love it we love it &        $\star\star\star$ &     $\star\star\star\star\star$ \\
 Loved this book! A great story and insight into the time period and life during those times. Highly recommend this book &        $\star\star\star$ &     $\star\star\star\star\star$ \\
     Great reading I could not put it down. Highly recommend reading this book. You will not be disappointed. Must read. &        $\star\star\star$ &     $\star\star\star\star\star$ \\
\bottomrule
\end{tabular}


}


\end{center}
% \vskip -0.2in
\end{table}



\begin{table}[ht]
% \vskip -0.05in
% \setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.8}% Makes table rows tighter
\caption{Ablation study (varying train set size, test split, and epochs) comparing test accuracy (\%) of CL methods versus a standard training baseline for classifying noisy, real-world Amazon reviews text data as either 1-star, 3-stars, or 5-stars. A simple multinomial logistic regression classifier is used. Mean top-1 accuracy and standard deviations are reported over five trials. The number of estimated label errors CL methods removed prior to training is shown in the ``Pruned'' column. Baseline training begins to overfit to noise with additional epochs trained, whereas CL test accuracy continues to increase \emph{(cf. N=1000K, Epochs: 50)}.}
\vskip -0.15in
\label{amazon_benchmarks}
\begin{center}
% \tiny
\resizebox{.99\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

\begin{tabular}{ll|llll|lll}
\toprule
  Test & \multicolumn{1}{r|}{Train set size}  & \multicolumn{4}{c|}{$N = 1000K$ } & \multicolumn{3}{c}{$N = 500K$} \\
\multicolumn{2}{l|}{}    & Epochs: 5 & Epochs: 20 & Epochs: 50 & Pruned & Epochs: 5 & Epochs: 20 & Pruned \\
\midrule
10th & CL: $\bm{C}_{\text{confusion}}$ &   85.2$\pm$0.06  &   89.2$\pm$0.02 &  90.0$\pm$0.02 & 291K &  86.6$\pm$0.03 &   86.6$\pm$0.03 &   259K \\
   & CL: C+NR                        &   86.3$\pm$0.04  &   \textbf{89.8$\pm$0.01} &  \textbf{90.2$\pm$0.01} & 250K &  \textbf{87.5$\pm$0.05} &   \textbf{87.5$\pm$0.03} &   244K \\
   & CL: $\cj$                       &   \textbf{86.4$\pm$0.01}  &   \textbf{89.8$\pm$0.02} &  90.1$\pm$0.02 & 246K &  \textbf{87.5$\pm$0.02} &   \textbf{87.5$\pm$0.02} &   243K \\
   & CL: PBC                         &   86.2$\pm$0.03  &   89.7$\pm$0.01 & \textbf{90.2$\pm$0.01} &  257K &  87.4$\pm$0.03 &   87.4$\pm$0.03 &   247K \\
   & CL: PBNR                        &   86.2$\pm$0.07  &   89.7$\pm$0.01 &  \textbf{90.2$\pm$0.01} & 257K &  87.4$\pm$0.05 &   87.4$\pm$0.05 &   247K \\
   & Baseline                        &   83.9$\pm$0.11  &   86.3$\pm$0.06 &  84.4$\pm$0.04 &  0K &  82.7$\pm$0.07 &   82.8$\pm$0.07 &     0K \\
\midrule
11th & CL: $\bm{C}_{\text{confusion}}$ &   85.3$\pm$0.05 &   89.3$\pm$0.01 &  90.0$\pm$0.0 & 294K &  86.6$\pm$0.04 &   86.6$\pm$0.06 &   261K \\
   & CL: C+NR                        &   \textbf{86.4$\pm$0.06} &   \textbf{89.8$\pm$0.01} &  90.2$\pm$0.01 & 252K &  \textbf{87.5$\pm$0.04} &   \textbf{87.5$\pm$0.03} &   247K \\
   & CL: $\cj$                       &   86.3$\pm$0.05 &   \textbf{89.8$\pm$0.01} &  90.1$\pm$0.02 & 249K &  \textbf{87.5$\pm$0.03} &   \textbf{87.5$\pm$0.02} &   246K \\
   & CL: PBC                         &   86.2$\pm$0.03 &   \textbf{89.8$\pm$0.01} &  \textbf{90.3$\pm$0.0} & 260K &  87.4$\pm$0.03 &   87.4$\pm$0.05 &   250K \\
   & CL: PBNR                        &   86.2$\pm$0.06 &   \textbf{89.8$\pm$0.01} &  90.2$\pm$0.02 & 260K &  87.4$\pm$0.05 &   87.4$\pm$0.03 &   249K \\
   & Baseline                        &   83.9$\pm$0.0  &   86.3$\pm$0.05 &   84.4$\pm$0.12 & 0K &  82.7$\pm$0.04 &   82.7$\pm$0.09 &     0K \\
\bottomrule
\end{tabular}

}

\end{center}
% \vskip -0.2in
\end{table}


\paragraph{Learning with noisy labels / weak supervision} We compare the CL methods, which prune errors from the train set and subsequently provide clean data for training, versus a standard training baseline (denoted \emph{Baseline} in Table \ref{amazon_benchmarks}), which trains on the original, uncleaned train dataset. The same training settings used to find label errors (see Subsection \ref{amazon_reviews_training_settings}) are used to obtain all scores reported in Table \ref{amazon_benchmarks} for all methods. For a fair comparison, all mean accuracies in Table \ref{amazon_benchmarks} are reported on the same held-out test set, created by splitting the Amazon reviews dataset into a train set and test set such that every tenth example is placed in a test set and the remaining data is available for training (the Amazon Reviews 5-core dataset provides no explicit train set and test set).

The Amazon Reviews dataset is naturally noisy, but the fraction of noise in the dataset is estimated to be less than 4\% \citep{northcutt2021labelerrors}, which makes studying the benefits of providing clean data for training challenging. To increase the percentage of noisy labels without adding synthetic noise, we subsample 1 million training examples from the train set by combining the label issues identified by all five CL methods from the original training data (244K examples) and a uniformly random subsample (766k examples) of the remaining ``cleaner'' training data. This process increases the percentage of label noise to 24\% (estimated) in the train set and, importantly, does \emph{not} increase the percentage of noisy labels in the test set -- large amounts of test set label noise have been shown to severely impact benchmark rankings \citep{northcutt2021labelerrors}.


To mitigate the bias induced by the choice of train set size, test set split, and the number of epochs trained, we conduct an ablation study shown in Table \ref{amazon_benchmarks}. For the train set size, we repeat each experiment with train set sizes of 1-million examples and $500,000$ examples. For the test set split, we repeat all experiments by removing every \emph{eleventh} example (instead of tenth) in our train/test split (c.f. the first column in Table \ref{amazon_benchmarks}), minimizing the overlap (9\%) between the two test sets. For each number of epochs trained, we repeat each experiment with 5, 20, and 50 epochs. We omit ($N = 500K$, Epochs: 50) because no learning occurs after 5 epochs.

Every score reported in Table \ref{amazon_benchmarks} is the mean and standard deviation of five trials: each trial varies the randomly selected subset of training data and the initial weights of the logistic regression model used for training. 

The results in Table \ref{amazon_benchmarks} reveal three notable observations. First, all CL methods outperform the baseline method by a significant margin in all cases. Second, CL methods outperform the baseline method even with nearly half of the training data pruned (Table \ref{amazon_benchmarks}, cf. N=500K). Finally, for the train set size $N = 1000K$, baseline training begins to overfit to noise with additional epochs trained, whereas CL test accuracy continues to increase \emph{(cf. N=1000K, Epochs: 50)}, suggesting CL robustness to overfitting to noise during training. The results in Table \ref{amazon_benchmarks} suggest CL's efficacy for noisy supervision with logistic regression in the context of text data.


\subsection{Real-world Label Errors in Other Datasets}

We use CL to find label errors in the purported ``error-free" MNIST dataset comprised of preprocessed black-and-white handwritten digits, and also in the noisy-labeled WebVision dataset \citep{li2017webvision} comprised of color images collected from online image repositories and using the search query as the noisy label.



\begin{figure*}[ht]
\centerline{\includegraphics[width=\textwidth]{img/mnist_training_label_errors24_prune_by_noise_rate.pdf}}
\vskip -0.1in
\caption{Label errors in the original, unperturbed MNIST train dataset identified using CL: PBNR. These are the top 24 errors found by CL, ordered left-right, top-down by increasing self-confidence, denoted \emph{conf} in teal. The predicted $\argmax \hat{p}(\tilde{y}=k ; x, \model )$ label is in green. Overt errors are in red. This dataset is assumed ``error-free'' in tens of thousands of studies.} 
\label{mnist_training_label_errors24_prune_by_noise_rate}
\vskip -.2in
\end{figure*}


\begin{figure*}[!b]
% \vskip -.1in
\centerline{\includegraphics[width=\textwidth]{img/webvision_train_label_errors.pdf}}
% \vskip -.1in
\caption{Top 32 identified label issues in the WebVision train set using CL: $\cj$. Out-of-sample predicted probabilities are obtained using a model pre-trained on ImageNet, avoiding training entirely. Errors are boxed in red. Ambiguous cases or mistakes are boxed in black. Label errors are ordered automatically by normalized margin.} 
\label{label_errors_webvision_train_top32}
\end{figure*}



To our surprise, the original, unperturbed MNIST dataset, which is predominately assumed error-free, contains blatant label errors, highlighted by the red boxes in Fig. \ref{mnist_training_label_errors24_prune_by_noise_rate}. To find label errors in MNIST, we pre-trained a simple 2-layer CNN for 50 epochs, then used cross-validation to obtain $\probmatrix$, the out-of-sample predicted probabilities for the train set. CL: PBNR was used to identify the errors. The top 24 label errors, ordered by self-confidence, are shown in Fig. \ref{mnist_training_label_errors24_prune_by_noise_rate}. For verification, the indices of the train label errors are shown in grey. 



To find label errors in WebVision, we used a pre-trained model to obtain $\probmatrix$, observing two practical advantages of CL: (1) a pre-trained model can be used to obtain $\probmatrix$ out-of-sample instead of cross-validation and (2) this makes CL fast. For example, finding label errors in WebVision, with over a million images and 1,000 classes, took three minutes on a laptop using a pre-trained ResNext model that had never seen the noisy WebVision train set before. We used the CL: $\cj$ method to find the label errors and ordered errors by normalized margins. Examples of WebVision label errors found by CL are shown in Fig. \ref{label_errors_webvision_train_top32}.






% \begin{table*}[t]

% \setlength\tabcolsep{2pt} % Makes table columns tighter
% \renewcommand{\arraystretch}{0.9}% Makes table rows tighter
% \caption{Accuracy, F1, precision, and recall measures for finding synthetic label errors in CIFAR-10.}
% \vskip -0.1in
% \label{table:cifar10_label_error_measures}
% \begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!

% \begin{tabular}{l|cccccc|cccccc|cccccc|cccccc}
% \toprule
% Measure &\multicolumn{6}{c}{\textbf{Accuracy}} & \multicolumn{6}{c}{\textbf{F1}} & \multicolumn{6}{c}{\textbf{Precision}}  & \multicolumn{6}{c}{\textbf{Recall}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} \cmidrule(lr){20-25}
% Noise & \multicolumn{2}{c}{0.2} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.7} & \multicolumn{2}{c}{0.2} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.7} & \multicolumn{2}{c}{0.2} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.7}  & \multicolumn{2}{c}{0.2} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.7} \\
% Sparsity &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6  &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6  &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6  &   0.0 &   0.6 &   0.0 &   0.6 &   0.0 &   0.6 \\
% \midrule
% \textbf{CL: baseline}      &  0.84 &  0.85 &  0.85 &  0.81 &  \textbf{0.76} &  \textbf{0.61} &  0.71 &  0.72 &  0.84 &  0.79 &  \textbf{0.83} &  \textbf{0.70} &  0.56 &  0.58 &  0.74 &  0.70 &  0.82 &  0.76 &  \textbf{0.98} &  \textbf{0.97} &  \textbf{0.97} &  \textbf{0.90} &  \textbf{0.84} &  \textbf{0.65}\\
% \textbf{CL: $\mathcal{C}$} &  0.89 &  \textbf{0.90} &  0.86 &  \textbf{0.84} &  \textbf{0.76} &  0.60 &  0.75 &  0.78 &  0.84 &  \textbf{0.80} &  \textbf{0.83} &  0.69 &  \textbf{0.67} &  \textbf{0.70} &  0.78 &  0.77 &  0.82 &  0.76 &  0.86 &  0.88 &  0.91 &  0.84 &  \textbf{0.84} &  0.63\\
% \textbf{CL: PBC}           &  0.88 &  0.88 &  0.86 &  0.82 &  0.73 &  0.59 &  0.76 &  0.76 &  0.84 &  0.79 &  0.81 &  0.67 &  0.64 &  0.65 &  0.76 &  0.74 &  0.82 &  0.76 &  0.96 &  0.93 &  0.94 &  0.85 &  0.80 &  0.61\\
% \textbf{CL: PBNR}          &  0.89 &  \textbf{0.90} &  \textbf{0.88} &  \textbf{0.84} &  0.66 &  0.54 &  0.77 &  \textbf{0.79} &  \textbf{0.85} &  \textbf{0.80} &  0.72 &  0.60 &  0.65 &  0.68 &  \textbf{0.82} &  \textbf{0.79} &  \textbf{0.84} &  \textbf{0.77} &  0.93 &  0.94 &  0.88 &  0.82 &  0.63 &  0.49\\
% \textbf{CL: C+NR}          &  \textbf{0.90} &  \textbf{0.90} &  0.87 &  0.83 &  0.64 &  0.53 &  \textbf{0.78} &  0.78 &  0.84 &  0.78 &  0.70 &  0.58 &  \textbf{0.67} &  0.69 &  \textbf{0.82} &  \textbf{0.79} &  \textbf{0.84} &  \textbf{0.77} &  0.93 &  0.90 &  0.87 &  0.78 &  0.61 &  0.47\\
% \bottomrule
% \end{tabular}
% }

% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table*}



% Confident learning does not attempt to relabel with the \emph{guessed} labels in green. It prunes (removes) these estimated errors and trains on the remaining subset. The \emph{guess} in green only serves to provide clarity in the figure, and has no algorithmic intent.

% \begin{figure*}[t]
% \vskip -.1in
% \centerline{\includegraphics[width=.8\textwidth]{img/imagenet_validation_label_errors_32_prune_by_noise_rate.pdf}}
% \vskip -.1in
% \caption{Label errors in the 2012 ImageNet validation dataset identified automatically with confident learning using a pre-trained ResNet18. Displayed are the 36 least confident labels, $\sim5000$ errors. } 
% \label{imagenet_validation_label_errors_32_prune_by_noise_rate}
% % \vskip -0.25in
% \end{figure*}


% \begin{figure}[ht]

% \begin{subfigure}[ht]{0.5\textwidth}
% \label{fig:mnist_train_removed}
% \includegraphics[width=.95\textwidth]{img/mnist_test_error_train_errors_removed.pdf}
% \vskip -.1in
% \caption{MNIST test error with estimated label errors removed from the train set.} 
% % \vskip -0.3in
% \end{subfigure}
% \begin{subfigure}[ht]{0.5\textwidth}
% \label{fig:mnist_test_removed}
% \includegraphics[width=.95\textwidth]{img/mnist_test_error_test_errors_removed.pdf}
% \vskip -.1in
% \caption{MNIST test error with estimated label errors removed from the test set.} 
% % \vskip -0.3in
% \end{subfigure}
% \caption{MNIST test error with errors removed from the (a) train set, and (b) test set.}
% \label{fig:mnist_test_error_removing_errors}
% \end{figure}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=.95\textwidth]{img/mnist_test_error_test_errors_removed.pdf}}
% \vskip -.1in
% \caption{MNIST test error with estimated label errors removed from the test set.} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{figure*}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=.5\textwidth]{img/mnist_test_error_train_errors_removed.pdf}}
% \vskip -.1in
% \caption{MNIST test error with estimated label errors removed from the train set.} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{figure*}


% MAYBE DONT DELTE THIS
% \textbf{2012 ImageNet validation set} 

% The top-left image in Fig. \ref{imagenet_validation_label_errors_32_prune_by_noise_rate} is a multi-label image valid for both labels `baseball' and `bucket'. This is problematic as we may count this example twice and overestimate the number of label errors. This is not an inconsistency in our theory, but instead reflects our assumption that all inputs belong to a single class. Consequently, it is possible confident learning overestimated the number of errors in this dataset.



% \textbf{Computation time} All figures in this section were generated end-to-end on a single i7 CPU processor in a few hours. The majority of compute time comes from the forward pass to compute the softmax output (predicted probabilities) for all 50,000 ImageNet validation examples using the \href{https://github.com/pytorch/vision/blob/master/torchvision/models/resnet.py}{PyTorch pre-trained resnet18} (1 hour), computing the 250x250 ImageNet noise matrices (30 minutes), and to pre-train the  \href{https://github.com/pytorch/examples/blob/master/mnist/main.py}{PyTorch MNIST CNN} for 50 epochs (30 minutes). Computation was distributed over 4 threads. The compute time added by the other confident learning steps was negligible (<60s). 



==> Confident Learning (JAIR 2021) (Version 6610)/framework.tex <==


%% In this section, we define the notation, assumptions, and principles underlying confident learning.
%%
%% \subsection{Framework}




\section{CL Framework and Problem Set-up}
\label{sec:setup}


% Confident learning is built on a common language of variables, definitions, and assumptions. 
In the context of multiclass data with possibly noisy labels, let $[m]$ denote $\{1, 2, ..., m\}$, the set of $m$ unique class labels, and $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ denote the dataset of $n$ examples $\bm{x} \in \mathbb{R}^d$ with associated observed noisy labels $\tilde{y} \in [m]$. $\bm{x}$ and $\tilde{y}$ are coupled in $\bm{X}$ to signify that \emph{cleaning} removes data and label. While a number of relevant works address the setting where annotator labels are available \citep{chi2021data, bouguelia2018agreeing, tanno2019learning, Tanno_2019_CVPR, khetan2018learning}, this paper addresses the general setting where no annotation information is available except the observed noisy labels.

\paragraph{Assumptions} We assume there exists, for every example, a latent, true label $y^*$. Prior to observing $\tilde{y}$, a class-conditional classification noise process \citep{angluin1988learning} maps $y^* {\scriptstyle \rightarrow} \; \tilde{y}$ such that every label in class $j \in [m]$ may be independently mislabeled as class $i \in [m]$ with probability $p(\tilde{y} \smalleq i \vert y^* \smalleq j)$. This assumption is reasonable and has been used in prior work~\citep{DBLP:conf/iclr/GoldbergerB17_smodel,Sukhbaatar_fergus_iclr_2015}.

\paragraph{Notation} Notation is summarized in Table \ref{t:notation}. The discrete random variable $\tilde{y} $ takes an observed, noisy label (potentially flipped to an incorrect class), and $y^* $ takes a latent, uncorrupted label. The subset of examples in $\bm{X}$ with noisy class label $i$ is denoted $\bm{X}_{\tilde{y}\smalleq i}$, \emph{i.e.} $\bm{X}_{\tilde{y}\smalleq \text{cow}}$ is read, ``examples with class label \emph{cow}.'' The notation $p(\tilde{y} ; \bm{x})$, as opposed to $p(\tilde{y} \vert \bm{x})$, expresses our assumption that input $\bm{x}$ is observed and error-free. We denote the discrete joint probability of the noisy and latent labels as $p(\tilde{y},y^*)$, where conditionals $p(\tilde{y} \vert y^*)$ and $p(y^* \vert \tilde{y})$ denote probabilities of label flipping. We use $\hat{p}$ for predicted probabilities. In matrix notation, the $n \times m$ matrix of out-of-sample predicted probabilities is $\bm{\hat{P}}_{k,i} \coloneqq \hat{p}(\tilde{y} = i; \bm{x}_k, \bm{\theta})$, the prior of the latent labels is $\prior \coloneqq p(y^* \smalleq i)$; the $m \times m$ joint distribution matrix is $\joint \coloneqq p(\tilde{y} \smalleq i,y^* \smalleq j)$; the $m \times m$ noise transition matrix (noisy channel) of flipping rates is $\nm \coloneqq p(\tilde{y} \smalleq i \vert y^* \smalleq j)$; and the $m \times m$ mixing matrix is $\inv \coloneqq p(y^* \smalleq i \vert \tilde{y} \smalleq j)$. At times, we abbreviate $\hat{p}(\tilde{y} = i ; \bm{x}, \bm{\theta})$ as $\predprobshorti$, where $\model$ denotes the model parameters. CL assumes no specific loss function associated with $\model$: the CL framework is model-agnostic.
% We denote the confident joint as $\cj$ and the joint as $\joint$. From $\estjoint$, all latent distributions are derived: $\estprior, \estnm, \estinv$. 

\begin{table*}[hbt!] 
% \renewcommand{\arraystretch}{.9}% Makes table rows tighter
\caption{Notation used in confident learning.}
% \vskip -.2in
\label{t:notation}
\begin{center}
% \begin{small}
% \begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{rl} 
\toprule

\textbf{Notation} & \textbf{Definition} \\
\midrule
$m$ & The number of unique class labels \\
$[m]$ & The set of $m$ unique class labels \\
$\tilde{y}$  & Discrete random variable $\tilde{y} \in [m]$ takes an observed, noisy label \\
$y^*$  & Discrete random variable  $y^* \in [m]$  takes the unknown, true, uncorrupted label \\
$\bm{X}$ & The dataset $(\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ of $n$ examples $\bm{x} \in \mathbb{R}^d$ with noisy labels \\
$\bm{x}_k$ & The $k^{th}$ training data example \\
$\tilde{y}_k$ & The observed, noisy label corresponding to $\bm{x}_k$ \\
$y_k^*$ & The unknown, true label corresponding to $\bm{x}_k$ \\
$n$ & The cardinality of $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n$, i.e. the number of examples in the dataset \\
$\bm{\theta}$ & Model parameters \\
$\bm{X}_{\tilde{y}\smalleq i}$ & Subset of examples in $\bm{X}$ with noisy label $i$, \emph{i.e.} $\bm{X}_{\tilde{y}\smalleq \text{cat}}$ is ``examples labeled cat'' \\
$\bm{X}_{\tilde{y}\smalleq i, y^*\smalleq j}$ & Subset of examples in $\bm{X}$ with noisy label $i$ and true label $j$ \\
$\hat{\bm{X}}_{\tilde{y}\smalleq i, y^*\smalleq j}$ & Estimate of subset of examples in $\bm{X}$ with noisy label $i$ and true label $j$ \\
$p(\tilde{y} \smalleq i, y^* \smalleq j)$ & Discrete joint probability of noisy label $i$ and true label $j$. \\
$p(\tilde{y} \smalleq i \vert y^* \smalleq j)$ & Discrete conditional probability of true label flipping, called the noise rate \\
$p( y^* \smalleq j \vert \tilde{y} \smalleq i )$ & Discrete conditional probability of noisy label flipping, called the inverse noise rate \\
$\hat{p}(\cdot)$ & Estimated or predicted probability (may replace $p(\cdot)$ in any context) \\
$\prior$ & The prior of the latent labels \\
$\estprior$ & Estimate of the prior of the latent labels \\
$\joint$ & The $m \times m$ joint distribution matrix for $p(\tilde{y},y^*)$ \\
$\estjoint$ & Estimate of the $m \times m$ joint distribution matrix for $p(\tilde{y},y^*)$ \\
$\nm$ & The $m \times m$ noise transition matrix (noisy channel) of flipping rates for $p(\tilde{y} \vert y^*)$ \\
$\estnm$ & Estimate of the $m \times m$ noise transition matrix of flipping rates for $p(\tilde{y} \vert y^*)$ \\
$\inv$ & The inverse noise matrix for $p(y^* \vert \tilde{y})$ \\
$\estinv$ & Estimate of the inverse noise matrix for $p(y^* \vert \tilde{y})$ \\
$\hat{p}(\tilde{y} = i ; \bm{x}, \bm{\theta})$ & Predicted probability of label $\tilde{y} = i$ for example $\bm{x}$ and model parameters $\bm{\theta}$ \\
$\predprobshorti$ & Shorthand abbreviation for predicted probability $\hat{p}(\tilde{y} = i ; \bm{x}, \bm{\theta})$ \\
$\hat{p}(\tilde{y}\smalleq i ; \bm{x} \smallin \bm{X}_{\tilde{y}=i}, \bm{\theta} )$ & The \emph{self-confidence} of example $\bm{x}$ belonging to its given label $\tilde{y}\smalleq i$ \\
$\bm{\hat{P}}_{k,i}$ & $n \times m$ matrix of out-of-sample predicted probabilities $\hat{p}(\tilde{y} = i; \bm{x}_k, \bm{\theta})$ \\
$\cj$ & The \emph{confident joint} ${\cj \in \mathbb{N}_{\geq 0}}^{m \times m}$, an unnormalized estimate of $\joint$ \\
$\bm{C}_{\text{confusion}}$ & Confusion matrix of given labels $\tilde{y}_k$ and predictions $\argmax_{i \in [m]} \hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta}) $ \\
$t_j$ & The expected (average) self-confidence for class $j$ used as a threshold in $\cj$ \\
$p^*(\tilde{y} \smalleq i \vert y^* \smalleq y_k^*)$ & \emph{Ideal} probability for some example $\bm{x}_k$, equivalent to noise rate $p^*(\tilde{y} \smalleq i \vert y^* \smalleq j)$ \\
$\perfprobshorti$ & Shorthand abbreviation for ideal probability $p^*(\tilde{y} \smalleq i \vert y^* \smalleq y_k^*)$ \\


\bottomrule
\end{tabular}
}
% \end{sc}
% \end{small}
\end{center}
%  \vskip -0.25in
\end{table*}

\paragraph{Goal} Our assumption of a class-conditional noise process implies the label noise transitions are data-independent, i.e., 
$p(\tilde{y} \vert y^* ; \bm{x}) = p(\tilde{y} \vert y^*)$. To characterize class-conditional label uncertainty, one must estimate $p(\tilde{y} \vert y^*)$ and $p(y^*)$, the latent prior distribution of uncorrupted labels. Unlike prior works which estimate $p(\tilde{y} \vert y^*)$ and $p(y^*)$ independently, we estimate both jointly by directly estimating the joint distribution of label noise, $p(\tilde{y} , y^*)$. \textbf{Our goal} is to estimate every $p(\tilde{y} , y^*)$ as a matrix $\joint$ and use $\joint$ to find all mislabeled examples $\bm{x}$ in dataset $\bm{X}$ where $y^* \neq \tilde{y}$. This is hard because it requires disambiguation of model error (epistemic uncertainty) from the intrinsic label noise (aleatoric uncertainty), while simultaneously estimating the joint distribution of label noise ($\joint$) without prior knowledge of the latent noise transition matrix ($\nm$), the latent prior distribution of true labels ($\prior$), or any latent, true labels ($y*$).

\begin{definition} [Sparsity]
    A statistic to quantify the characteristic shape of the label noise defined by fraction of zeros in the off-diagonals of $\joint$. \emph{High sparsity quantifies non-uniformity of label noise, common to real-world datasets. For example, in ImageNet, \emph{missile} may have high probability of being mislabeled as \emph{projectile}, but near-zero probability of being mislabeled as most other classes like \emph{wool} or \emph{wine}. Zero sparsity implies every noise rate in $\joint$ is non-zero. A sparsity of 1 implies no label noise because the off-diagonals of $\joint$, which encapsulate the class-conditional noise rates, must all be zero if sparsity = 1.}
\end{definition}

\begin{definition}[Self-Confidence]
    The predicted probability for some model $\bm{\theta}$ that an example $\bm{x}$ belongs to its given label $\tilde{y} $, expressed as $\hat{p}(\tilde{y}\smalleq i ; \bm{x} \smallin \bm{X}_{\tilde{y}=i}, \bm{\theta} )$. \emph{Low self-confidence is a heuristic-likelihood of being a label error.}
\end{definition}


\endinput


\textbf{Assumptions.} \;
% We assume that prior to observing $\tilde{y} $, a class-conditional Classification Noise Process (CNP) \citep{angluin1988learning} randomly mapped latent labels $y^* $ to noisy labels $\tilde{y} $ such that each label in class $i \smallin M$ is mislabeled independently as class $j \smallin M$ with probability $p(\tilde{y}\smalleq i \vert y^* = j)$. Thus, $\forall \bm{x} \in X,  p(\tilde{y} \vert y^* ; \bm{x}) = p(\tilde{y} \vert y^*)$. Throughout, we assume there is at least one example belonging to every class, the number of examples is finite, and the data $\bm{X}$ is error-free.
Prior to observing $\tilde{y}$, we assume a class-conditional classification noise process (CNP) \citep{angluin1988learning} maps $y^* {\scriptstyle \rightarrow} \; \tilde{y}$ such that every label in class $j \in [m]$ may be independently mislabeled as class $i \in [m]$ with probability $p(\tilde{y} \smalleq i \vert y^* \smalleq j)$. 
This assumption is reasonable and has been used in prior work~\citep{DBLP:conf/iclr/GoldbergerB17_smodel,Sukhbaatar_fergus_iclr_2015}. CNP implies a data-independent noise transition probability, namely, 
$p(\tilde{y} \vert y^* ; \bm{x}) = p(\tilde{y} \vert y^*)$.

% or in Amazon Reviews natural language dataset \citep{he2016ups_amazonreviews}, a \emph{4-star} rating is more likely to be mislabeled \emph{5-stars}, than \emph{1-star}. 
%CNP implies a data-independent noise transition probability $p(\tilde{y} \vert y^*)$:
%% \vskip -0.2in
%\begin{equation} \label{eqn:cnp}
%    p(\tilde{y} \vert y^* ; \bm{x}) = p(\tilde{y} \vert y^*)
%\end{equation}














% The asymmetric noise rates $p(\tilde{y} \vert y)$ form what is known in information theory as the noisy channel, an $n {\times} n$ noise rate matrix.

% \begin{definition}{Noise Rate Matrix, $\nm$.}\label{noise_matrix}
% % In multiclass learning with observed noisy labels $\tilde{y}$ and hidden true labels $y^* $, 
% $\nm$ is a $n {\times} n$, class-conditional probability matrix with entries $\nm_{\tilde{k},k} = p(\tilde{y}=\tilde{k} \vert y^*=k)$ and $\sum_{\tilde{n}=1}^M \small{p(\tilde{y}=\tilde{k} \vert y^*=k)} = 1$. $\nm$ captures the noise corruption process that maps $y \rightarrow \tilde{y}$. The $n$ diagonal entries $p(\tilde{y}=\tilde{k} \vert y^*=k) \in [0,1]$ measure \emph{class label consistency} and the $n^2 {-} n$ non-diagonal entries $p(\tilde{y}=\tilde{k} \vert y^*=k) \in [0,1), \tilde{k} \neq k $, are the \emph{asymmetric noise rates}.
% \end{definition}

% % From Def. (\ref{noise_matrix}), when $\frac{1}{n}\Tr(\nm) = 1$, then $\nm=\mathbf{I}$ and all noise rates (non-diagonal entries) are zero. Given a set $\mathbb{S}$ of candidate noisy label vectors $\textbf{s} = [s_1, s_2, ..., s_N]$ and an estimate of $\nm$ for each, the \emph{least noisy} $\textbf{s} \in \mathbb{S}$ is $\textbf{s}^* =  \argmax_{\textbf{s} \in \mathbb{S}}  \Tr(\nm)$. 

% From Def. (\ref{noise_matrix}), when $\frac{1}{n}\Tr(\nm) = 1$, then $\nm=\mathbf{I}$ and all noise rates (non-diagonal entries) are zero. Thus, the \emph{average class label consistency} is $\frac{1}{M}\Tr(\nm)$ and the \emph{average noise per class} is $1 - \frac{1}{M}\Tr(\nm)$. The two goals of multiclass Rank Pruning for multiclass learning with noisy labels are (1) perfect estimation of $\nm$ when the hidden class distributions are separable and an exact expression otherwise and (2) uncover the mapping $x \to y$ given only observed ($x,\tilde{y}$) pairs, where $y^* $ and $\nm$ are hidden.



To this end, we introduce \emph{confident learning}, a family of theory and algorithms for learning in the presence of label errors. For input examples $\bm{x}$ and their latent labels $y^* \in [m]$, we consider the dataset $\bm{X}$ of pairs $(\bm{x}, \tilde{y})$, where the observed given label $\tilde{y} \in Y$ is noisy. The noisy label distribution can be described by a $K \times K$ noise matrix $P_{\tilde{y}\mid y^*}$, where entry $(i,j)$ of the noise matrix is the probability that an example with latent label $y^*$ is given label $\tilde{y}$. This model assumes that label flips \todo{clarify? or is this term obvious} are independent of the input example $\bm{x}$, but some given labels may more likely than others for a particular latent label $y^*$. For example, a cat is more likely to be mislabeled as a dog than a tree. We are interested in discovering \emph{label errors}, where $\tilde{y} \neq y^*$ \todo{this isn't exactly right, fix}.

Because the noise matrix is unknown, we introduce the \emph{confident joint $\bm{C}$}, an unnormalized estimate of the joint distribution matrix $P_{\tilde{y}, y^*}$, computed with a particular classification model $\bm{\theta}$. The confident joint is a $K \times K$ matrix of counts where $\bm{C}_{i,j}$ is the number of examples labeled $\tilde{y} = i$ that the model confidently labels as $y^* = j$. The diagonal entries of $\bm{C}$ count the number of examples that are confidently predicted as their given label, while the off-diagonal elements $\bm{C_{i,j}}, i\neq j$ are interpreted as label error counts. The intuition is that an example that is confidently labeled as $i \neq \tilde{y}=j$ is likely to be a label error.

For a prediction $\hat{p}(y^*=k; \bm{x}, \bm{\theta})$ to be considered a confident prediction, we define a threshold $t_k$ for each class $k \in Y$:
$$ t_k = \frac{1}{|\bm{X}_{\tilde{y}=k}|} \sum_{\bm{x} \in \bm{X}_{\tilde{y}=k}} \hat{p}(y^*=k; \bm{x}, \bm{\theta})$$
where $\bm{X}_{\tilde{y}=k}$ is the set of examples with given label $k$. The threshold expresses the intuition that if an example has a higher predicted probability of belonging to a class $k$ than the average predicted probability of examples with that class label, then the model is confident that it belongs to that class.

==> Confident Learning (JAIR 2021) (Version 6610)/introduction.tex <==
\section{Introduction}

% \emph{PAR 1: Brief context. Many datasets nowadays are crow-sourced and include noisy labels. THe problem in dealing wtih noisy labels means two things: find label errors and learn in spite of them.}


Advances in learning with noisy labels and weak supervision usually introduce a new model or loss function. Often this model-centric approach band-aids the real question: which data is mislabeled? Yet, large datasets with noisy labels have become increasingly common. Examples span prominent benchmark datasets like ImageNet \citep{ILSVRC15_imagenet} and MS-COCO \citep{MS-COCO-IMAGE-DATASET} to human-centric datasets like electronic health records \citep{yoni_sontag_anchors_2016} and educational data \citep{NORTHCUTT_cameo_2016}. The presence of noisy labels in these datasets introduces two problems. How can we identify examples with label errors and how can we learn well despite noisy labels, irrespective of the data modality or model employed? Here, we follow a data-centric approach to theoretically and experimentally investigate the premise that the key to learning with noisy labels lies in accurately and directly characterizing the uncertainty of label noise in the data.

% Large datasets with noisy labels have become increasingly common. Examples span prominent benchmark datasets like ImageNet \citep{ILSVRC15_imagenet} and MS-COCO \citep{MS-COCO-IMAGE-DATASET} to human-centric datasets like electronic health records \citep{yoni_sontag_anchors_2016} and educational data \citep{NORTHCUTT_cameo_2016}.

% 

% Weak super\citep{fair_laurens_van_der_maaten_limits_weak_supervision_2018}

% crowd-sourced datasets labeled with Mechanical Turk \citep{mech_turk_quality}


% The last decade has witnessed a paradigm shift in supervised learning from training with curated, accurately-labeled datasets to using noisy, crowd-sourced datasets with thousands to billions of examples, potentially with erroneous labels. 
% Examples include prominent image datasets like ImageNet \citep{ILSVRC15_imagenet} and MS-COCO \citep{MS-COCO-IMAGE-DATASET} large, crowd-sourced datasets labeled with Mechanical Turk \citep{mech_turk_quality}; large-scale, rule-based labeling systems like Snorkel \citep{ratner_chris_re_large_training_sets_NIPS2016_6523, paroma_rule_baed_NIPS2017_6628}; medical applications like electronic health record phenotype prediction \citep{yoni_sontag_anchors_2016}; cheating detection in massive open online courses, where error-free non-cheating labels do not exist \citep{NORTHCUTT_cameo_2016}. To adapt to these changes, we have seen a proliferation of contributions in weakly-supervised learning or learning with noisy labels.
%\citep{weak_supervision_confidence_networks_nips2017_workshop, scott17_mutual_decontamination, ratner_chris_re_large_training_sets_NIPS2016_6523, fair_laurens_van_der_maaten_limits_weak_supervision_2018, Blanchard:2010:SND:1756006.1953028}, semi-supervised learning \citep{hendrycks2018using}, and learning with noisy labels \citep{NIPS2013_5073, Claesen201573, Menon2015, Liu:2016:CNL:2914183.2914328}.

% \emph{PAR 2: To find label errors, we model the noise using the joint. Estimating the joint is very valuable because (1) ontological issues, (2) from it you can estimate all the statistics of previous work. To our knowledge, no prior work is dedicated to a thorough analysis of estimating the joint of label noise. We estimate the joint, we can and can prove it.}

A large body of work, which may be termed ``confident learning,'' has arisen to address the uncertainty in dataset labels, from which two aspects stand out.  First, \possessivecite{angluin1988learning} classification noise process (CNP) provides a starting assumption that label noise is class-conditional, depending only on the latent true class, not the data. While there are exceptions, this assumption is commonly used \citep{DBLP:conf/iclr/GoldbergerB17_smodel,Sukhbaatar_fergus_iclr_2015} because it is reasonable for many datasets. For example, in ImageNet, a \emph{leopard} is more likely to be mislabeled \emph{jaguar} than \emph{bathtub}.  Second, direct estimation of the joint distribution between noisy (given) labels and true (unknown) labels (see Fig. \ref{fig_flow_examples}) can be pursued effectively based on three principled approaches used in many related studies: (a) {\bf Prune}, to search for label errors, e.g. following the example of \cite{chen2019confusion, patrini2017making, rooyen_menon_unhinged_nips15}, using \emph{soft-pruning} via loss-reweighting, to avoid the convergence pitfalls of iterative re-labeling -- (b) {\bf Count}, to train on clean data, avoiding error-propagation in learned model weights from reweighting the loss \citep{natarajan2017cost} with imperfect predicted probabilities, generalizing seminal work \cite{forman2005counting, forman2008quantifying, icml_lipton_label_shift_confusion_matrix} -- and (c) {\bf Rank} which examples to use during training, to allow learning with unnormalized probabilities or decision boundary distances, building on well-known robustness findings \citep{page1997pagerank} and ideas of curriculum learning \citep{jiang2018mentornet}.

% To address these problems, we directly estimate the joint distribution between noisy (given) labels and true (unknown) labels under the assumption of \possessivecite{angluin1988learning} classification noise process (CNP). CNP assumes label noise is class-conditional, depending only on the latent true class, not the data. While there are exceptions, this assumption is commonly used \citep{DBLP:conf/iclr/GoldbergerB17_smodel,Sukhbaatar_fergus_iclr_2015} because it is reasonable. For example, in ImageNet, a \emph{leopard} is more likely to be mislabeled \emph{jaguar} than \emph{bathtub}. 

% To our knowledge, no prior work has dedicated to direct estimation of the joint distribution of label noise. Estimating the joint is challenging, but useful because its marginals yield the important statistics used in the literature, including latent noise transition rates \citep{Sukhbaatar_fergus_iclr_2015, DBLP:conf/iclr/GoldbergerB17_smodel, noisy_boostrapping_google_reed_iclr_2015}, latent prior of uncorrupted labels \citep{lawrence_bayesian_prior_py_noisy_2001, graepel_kernel_gibbs_sampler_prior_py_bayesian_nips_2001}, and inverse noise rates \citep{scott17_mutual_decontamination}. While the noise rates are useful for loss-reweighting \citep{NIPS2013_5073} in learning with noisy labels, only the joint can directly estimate estimate the number of label errors for each pair of true and noisy classes. The joint is also useful to auto-discover ontological issues in datasets, e.g. ImageNet includes two classes for the same \emph{maillot} class (Table \ref{table_imagenet_characterization_top10} in Sec. \ref{sec:experiments}). Whereas prior approaches for joint estimation \citep{northcutt2017rankpruning} matrix-multiply noise rates and latent priors thereby summing error from two estimates, we estimate the joint directly and prove consistent estimation in Sec. \ref{sec:theory} with experimental evidence of accurate estimation on real datasets in Sec. \ref{sec:experiments}.

% \emph{PAR 3: What is confident learning and what has been done in the past. metnion angluin and laird's CNP. (abbreviated of first par in related works)  (leave some for related works). One sentence why prior works don't estimate the joint accurately.}


% \emph{Confident learning} (CL) is a principle-driven family of theory and algorithms for characterizing, finding, and learning with label errors. It uses the outputs of any model: this is important because state-of-the-art models frequently change \citep{jordan2015machine}. Shown in Fig. \ref{fig_flow_examples}, CL uses predicted probabilities and noisy labels to \emph{count} examples in the unnormalized \emph{confident joint} which is normalized to estimate the joint, then used to \emph{prune} noisy data. \cite{forman2008quantifying, forman2005counting} pioneered the \emph{count} principle to robustly estimate false positive and false negative rates and grand incites by \cite{NIPS2013_5073, rooyen_menon_unhinged_nips15, scott17_mutual_decontamination} pioneered the \emph{prune} principle with loss re-weighting as soft-pruning. 


To our knowledge, no prior work has thoroughly analyzed the direct estimation of the joint distribution between noisy and uncorrupted labels. Here, we assemble these principled approaches to generalize confident learning (CL) for this purpose. Estimating the joint distribution is challenging as it requires disambiguation of epistemic uncertainty (model predicted probabilities) from aleatoric uncertainty (noisy labels) \citep{aleatoric_epistemic_uncertainty_2013}, but useful because its marginals yield important statistics used in the literature, including latent noise transition rates \citep{Sukhbaatar_fergus_iclr_2015, noisy_boostrapping_google_reed_iclr_2015}, latent prior of uncorrupted labels \citep{lawrence_bayesian_prior_py_noisy_2001, graepel_kernel_gibbs_sampler_prior_py_bayesian_nips_2001}, and inverse noise rates \citep{scott19_jmlr_mutual_decontamination}. While noise rates are useful for loss-reweighting \citep{NIPS2013_5073}, only the joint can directly estimate the number of label errors for each pair of true and noisy classes. Removal of these errors prior to training is an effective approach for learning with noisy labels \citep{chen2019confusion}. The joint is also useful to discover ontological issues in datasets for dataset curation, e.g. ImageNet includes two classes for the same \emph{maillot} class (c.f. Table \ref{table_imagenet_characterization_top10} in Sec. \ref{sec:experiments}). 

% Whereas prior approaches for joint estimation \citep{northcutt2017rankpruning} matrix-multiply noise rates and latent priors thereby summing error from two estimates.

The generalized CL assembled in this paper upon the principles of pruning, counting, and ranking, is a model-agnostic family of theories and algorithms for characterizing, finding, and learning with label errors. It uses predicted probabilities and noisy labels to count examples in the unnormalized \emph{confident joint}, estimate the joint distribution, and prune noisy data, producing clean data as output.

This paper makes two key contributions to prior work on finding, understanding, and learning with noisy labels. First, a proof is presented giving realistic sufficient conditions under which CL exactly finds label errors and exactly estimates the joint distribution of noisy and true labels. Second, experimental data are shared, showing that this CL algorithm is empirically performant on three tasks (a) label noise estimation, (b) label error finding, and (c) learning with noisy labels, increasing ResNet accuracy on a cleaned-ImageNet and outperforming seven recent highly competitive methods for learning with noisy labels on the CIFAR dataset. The results presented are reproducible with the implementation of CL algorithms, open-sourced as the \textbf{\texttt{\href{https://github.com/cleanlab/cleanlab/?utm_source=arxiv&utm_medium=publication&utm_campaign=cleanlab}{cleanlab}}}\footnote{To foster future research in data cleaning and learning with noisy labels and to improve accessibility for newcomers, \textbf{\texttt{\href{https://github.com/cleanlab/cleanlab/?utm_source=arxiv&utm_medium=publication&utm_campaign=cleanlab}{cleanlab}}} is open-source and well-documented: \href{https://github.com/cleanlab/cleanlab/?utm_source=arxiv&utm_medium=publication&utm_campaign=cleanlab}{https://github.com/cleanlab/cleanlab/}} Python package.  

These contributions are presented beginning with the formal problem specification and notation (Section~\ref{sec:setup}), then defining the algorithmic methods employed for CL (Section~\ref{sec:methods}) and theoretically bounding expected behavior under ideal and noisy conditions (Section~\ref{sec:theory}). Experimental benchmarks on the CIFAR, ImageNet, WebVision, and MNIST datasets, cross-comparing CL performance with that from a wide range of highly competitive approaches, including
\emph{INCV} \citep{chen2019confusion}, \emph{Mixup} \citep{icml2018mixup}, \emph{MentorNet} \citep{jiang2018mentornet}, and \emph{Co-Teaching} \citep{han2018coteaching}, are then presented in Section~\ref{sec:experiments}. Related work (Section~\ref{sec:related}) and concluding observations (Section~\ref{sec:conclusion}) wrap up the presentation. Extended proofs of the main theorems, algorithm details, and comprehensive performance comparison data are presented in the appendices.

% CL is the only approach with robustness to highly sparse, non-uniform label noise, modeled after real-world datasets like ImageNet.
% Among these methods, CL is the only approach that does not decrease accuracy for realistic, sparse, non-uniform label noise. 

% % Lu suggested last paragraph
% We make three contributions in this paper. First we propose a novel CL framework based that allows for direct estimation of the joint distribution of label noise. We show in theory our model can produce consistent joint estimation and exact identification of label errors under realistic sufficient conditions. Second, We empirically evaluate CL on three tasks (a) label noise joint estimation, (b) label error finding, and (c) learning with noisy labels. These experiments validate the performance benefits of estimating the joint distribution. Finally, we release our code.... The code can be imported as standard python library.


% % Ike suggested last paragraph
% This new CL generalization provides three key advantages over prior art: (1) direct estimation of the joint distribution of noisy labels and true labels, (2) robust performance against non-uniformly random label noise, and (3) consistent joint estimation and exact identification of label errors under realistic sufficient conditions. We empirically evaluate CL on (a) accuracy of joint estimation, (b) label error finding, and (c) learning with noisy labels on CIFAR and ImageNet for both synthetic and real-world noise. These experiments validate the performance benefits of estimating the joint distribution. The new CL code, which reproduces all results described here, is fully open-sourced as the \texttt{cleanlab}\footnote{\ifarxiv \texttt{cleanlab} for finding and learning with noisy labels is open-source: \href{https://github.com/cleanlab/cleanlab/?utm_source=arxiv&utm_medium=publication&utm_campaign=cleanlab}{https://github.com/cleanlab/cleanlab/} \else Link to Python package anonymized for blind review. \fi} Python package.


% While we improve CL with direct joint estimation, CL's principles were establisihed by a number of pioneering works In pioneering work, \cite{forman2008quantifying, forman2005counting} introduced The \emph{count} principle to robustly estimate false positive and false negative rates. \cite{Elkan:2008:LCO:1401890.1401920} improved Forman's approach using thresholds to improve robustness, but requires uncorrupted positive labels. CL generalizes this use of thresholds to noise in every class. A number of formative works \citep{NIPS2013_5073, rooyen_menon_unhinged_nips15, scott17_mutual_decontamination} use loss re-weighting to prove empirical risk minimization motivating CL loss re-weighting when learning with noisy labels. CL combines these insights into a data-agnostic, model-agnostic framework supported by  sufficient conditions for robust, consistent estimation of the joint exact identification of label errors.

% \emph{PAR 4: How we improve confident learning to estimate the joint. Major techniques and benefits and contributions. We show this with both theoretical analysis under realistic settings and experiments. (try to summarize the method in one sentence) (reference fig 1). (this should answer last sentence in par three).}

% unlike prior art, CL performance does not degrade with non-uniformly random label noise



% Based on the theory, we implement \texttt{cleanlab}, a Python framework for characterizing, finding, and learning with label errors.

% State-of-the-art models change increasingly frequently \cite{jordan2015machine}, prompting the need for a model-agnostic framework that works with model outputs (e.g. probabilities) regardless of which model generated them.


% \emph{PAR 5: in this work, we Evaluate confident learning based on three criterion: joint estimation, label error finding, and learning with noisy labels. Result in Sec 1., shows this about joint estimation. result in sec \#, shows this about label error, ... Align our claims with our experimental results. Explain that while prior works in confident learning have made considerable contributions, there is no code base for researchers to use to build off and facilitate future researcher working with noisy label.}


\endinput

% Our contributions can be summarized as follows: 

% \quad \phantom{} 1. Proposed confident learning for characterizing, finding, \& learning with label errors in datasets. \\
% \phantom{\quad} 2. Proved non-trivial conditions for consistent joint estimation and exactly finding label errors. \\
% \phantom{\quad} 3. Verified the efficacy of CL on CIFAR (added label noise) and ImageNet (real label noise).\\
% \phantom{\quad} 4. Released the \texttt{cleanlab} Python package for accessibility and reproducibility. \\





% emphasize sparsity
% c\_confusion is basically incv w/ one iteration


% Because few code bases exist for researchers to facilitate future researchers working with noisy labels, we open-source \texttt{cleanlab}, a Python package using for characterizing, finding, and learning with label errors.


% To expand our understanding of machine learning models and their predictions, we must understand the data these models rely on.





% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.36\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/confident_learning_flow_figure.pdf}
%         \caption[]%
%         {The confident learning process. It is non-iterative. The red `X' shows model-agnosticism: only outputs are used.}    
%         \label{fig_flow_examples_a}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.29\textwidth}  
%         \centering 
%         \includegraphics[width=\textwidth]{img/confident_learning_confident_joint.pdf}
%         \caption[]%
%         {Example confident joint comprised of unnormalized counts. \\The matrix is asymmetric. Typically, similar classes (\emph{dog, fox}) have larger count than (\emph{cow, fox}).}
%         \label{fig_flow_examples_b}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.29\textwidth}  
%         \centering 
%         \includegraphics[width=\textwidth]{img/confident_learning_joint_example.pdf}
%         \caption[]%
%         {Example joint distribution of (b), fully characterizing class-conditional label noise. Rows sum to the distribution of observed labels. Matrix sum is 1.}   
%         \label{fig_flow_examples_c}
%     \end{subfigure}
% \label{fig_flow_examples}
% \caption{The confident learning process and examples of the confident joint $\cj$ and joint $\joint$, where $\tilde{y}$ indicates an observed noisy label and $y^*$ indicates a latent uncorrupted label.}
% \vskip -.2in
% \end{figure*}










% Perpetuated by a prolific increase in machine learning research \cite{jordan2015machine}, state-of-the-art models change increasingly frequently. In response, the theory and algorithms comprising confident learning are model-agnostic.  Confident learning works with model outputs (e.g. probabilities) regardless of which model generated them (Fig. \ref{fig_flow_examples_a}). For example, confident learning can use outputs from Bayesian models, deep learning models, and the state-of-the-art model that hasn't been invented yet.




%link to package has been obscured to respect the blind-review process.%\href{https://github.com/cleanlab/cleanlab/}{github.com/cleanlab/cleanlab}

%\phantom{\quad} 4. Out-performed commonly benchmarked methods by 30\% on CIFAR-10 with 40\% label noise. \\
%\phantom{\quad} 5. Improved ResNet test accuracy on ImageNet by removing train errors via confident learning. 


% Paramount to our ability to make progress in supervised learning with big data is efficient, accurate methods for estimating the amount of noise in training labels, identifying the label errors, and uncovering the same classifier we would have had if the training data was not mislabeled. We provided a fast, classifier-independent, robust solution to these three problems in this paper. Obtaining perfectly-labeled datasets is often impractical, but procuring erroneous, often crowd-sourced, labels may be more accessible, motivating the need for a robust, general solution to the problem of multiclass learning with noisy labels. Until now, no practical algorithm for robust multiclass learning with noisy labels exists. To our knowledge, multiclass Rank Pruning is the first practical solution for multiclass learning with noisy labels and fast estimation of the latent noisy channel.

% State-of-the-art supervised learning often requires thousands to millions of training examples, but obtaining accurate labels for large datasets is difficult. Most large-scale labeling approaches fall into two categories: (1) crowd-sourced, nonspecialist workers like in Mechanical Turk \citep{mech_turk_quality} or (2) rule-based systems like Snorkel \citep{ratner_chris_re_large_training_sets_NIPS2016_6523, paroma_rule_baed_NIPS2017_6628}. Both of these processes are inherently noisy. 



==> Confident Learning (JAIR 2021) (Version 6610)/macros.tex <==
% usage: \todo{message} or \todo[person]{message}
\newcommand*{\todo}[2][]{\textcolor{red}{[\textbf{\ifthenelse{\equal{#1}{}}{TODO}{TODO(#1)}}: #2]}}

% usage: \note{message}
\newcommand*{\note}[1]{\textcolor{blue}{[#1]}}

% Theory commands
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}

\newcommand*\estimates{\mathrel{\widehat=}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\indicator}[1]{\mathbbm{1}[[#1]]}
\newcommand{\datak}{X_{\tilde{y}{\scriptscriptstyle =}k}}
\newcommand{\dataj}{X_{\tilde{y}{\scriptscriptstyle =}j}}
\newcommand{\smalleq}{{\scriptstyle =}}
\newcommand{\smallplus}{{\scriptstyle +}}
\newcommand{\smallminus}{{\scriptstyle -}}
\newcommand{\smallcoloneq}{{\scriptstyle \coloneqq}}
\newcommand{\smallra}{{\scriptstyle \rightarrow}}
\newcommand{\tinyeq}{{\scriptscriptstyle =}}
\newcommand{\smallin}{{\scriptstyle \in}}
\newcommand{\tinyin}{{\scriptscriptstyle \in}}

\newcommand{\nm}{\bm{Q}_{\tilde{y} \vert y^*}}
\newcommand{\inv}{\bm{Q}_{y^* \vert \tilde{y}}}
\newcommand{\joint}{\bm{Q}_{\tilde{y}, y^*}}
\newcommand{\prior}{\bm{Q}_{y^*}}
\newcommand{\noisyprior}{\bm{Q}_{\tilde{y}}}

\newcommand{\estnm}{\hat{\bm{Q}}_{\tilde{y} \vert y^*}}
\newcommand{\estinv}{\hat{\bm{Q}}_{y^* \vert \tilde{y}}}
\newcommand{\estjoint}{\hat{\bm{Q}}_{\tilde{y}, y^*}}
\newcommand{\estprior}{\hat{\bm{Q}}_{y^*}}

\newcommand{\nmlong}{\bm{Q}_{\tilde{y} = i \vert y^* = j}}
\newcommand{\invlong}{\bm{Q}_{y^* = j \vert \tilde{y} = i}}
\newcommand{\jointlong}{\bm{Q}_{\tilde{y} = i, y^* = j}}
\newcommand{\priorlong}{\bm{Q}_{y^* = j}}
\newcommand{\noisypriorlong}{\bm{Q}_{\tilde{y} = i}}

\newcommand{\estnmlong}{\hat{\bm{Q}}_{\tilde{y} = i \vert y^* = j}}
\newcommand{\estinvlong}{\hat{\bm{Q}}_{y^* = j \vert \tilde{y} = i}}
\newcommand{\estjointlong}{\hat{\bm{Q}}_{\tilde{y} = i, y^* = j}}
\newcommand{\estpriorlong}{\hat{\bm{Q}}_{y^* = j}}


\newcommand{\model}{\bm{\theta}} 
\newcommand{\pyx}{\hat{p}(\tilde{y} ; \bm{x}, \bm{\theta})} 
\newcommand{\probmatrix}{\bm{\hat{P}}_{k,i}}
\newcommand{\predprobshorti}{\hat{p}_{\bm{x}, \tilde{y} \smalleq i}}
\newcommand{\predprobshortj}{\hat{p}_{\bm{x}, \tilde{y} \smalleq j}}
\newcommand{\predprobshortk}{\hat{p}_{\bm{x}, \tilde{y} \smalleq k}}
\newcommand{\predprobshortl}{\hat{p}_{\bm{x}, \tilde{y} \smalleq l}}
\newcommand{\perfprobshorti}{p^*_{\bm{x}, \tilde{y} \smalleq i}}
\newcommand{\perfprobshortj}{p^*_{\bm{x}, \tilde{y} \smalleq j}}
\newcommand{\perfprobshortk}{p^*_{\bm{x}, \tilde{y} \smalleq k}} 
\newcommand{\perfprobshortl}{p^*_{\bm{x}, \tilde{y} \smalleq l}}
\newcommand{\errorxi}{\epsilon_{\bm{x}, \tilde{y} \smalleq i}}
\newcommand{\errorxj}{\epsilon_{\bm{x}, \tilde{y} \smalleq j}}
\newcommand{\cj}{\bm{C}_{\tilde{y}, y^*}}
\newcommand{\cjlong}{\bm{C}_{\tilde{y} \smalleq i, y^* \smalleq j}}
\newcommand{\estpartition}{\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}
\newcommand{\partition}{\bm{X}_{ \tilde{y} \smalleq i,y^* \smalleq j}}

\newcommand\req[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\tiny #1}}}{=}}}
\DeclareMathOperator*{\EXlimits}{\mathbb{E}}% expected value
\DeclareMathOperator{\EX}{\mathbb{E}}% expected value

% Taken from ICLR template
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}


\newcommand{\beginsupplement}{ % use to mark beginning of supplementary section.
\setcounter{section}{0}
\renewcommand{\thesection}{S\arabic{section}} %
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\setcounter{table}{0}
\renewcommand{\thetable}{S\arabic{table}} %
\setcounter{figure}{0}
\renewcommand{\thefigure}{S\arabic{figure}} %
}

% allows you to create Northcutt & Athalye's (2020) work on... (note the apostrophe occurs in the name, not appeneded to the year).
\newcommand{\possessivecite}[1]{\citeauthor{#1}'s (\citeyear{#1})}

==> Confident Learning (JAIR 2021) (Version 6610)/methods.tex <==
\section{CL Methods}
\label{sec:methods}

Confident learning (CL) estimates the joint distribution between the (noisy) observed labels and the (true) latent labels. CL requires two inputs: (1) the out-of-sample predicted probabilities $\bm{\hat{P}}_{k,i}$ and (2) the vector of noisy labels $\tilde{y}_k$. The two inputs are linked via index $k$ for all $\bm{x}_k \in \bm{X}$. None of the true labels $y^*$ are available, except when $\tilde{y} = y^*$, and we do not know when that is the case.

The out-of-sample predicted probabilities $\bm{\hat{P}}_{k,i}$ used as input to CL are computed beforehand (e.g. cross-validation) using a model $\model$: so, how does $\model$ fit into the CL framework? Prior works typically learn with noisy labels by directly modifying the model or training loss function, restricting the class of models. Instead, CL decouples the model and data cleaning procedure by working with model outputs $\bm{\hat{P}}_{k,i}$, so that any model that produces a mapping $\model: \bm{x} \rightarrow \hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta})$ can be used (e.g. neural nets with a softmax output, naive Bayes, logistic regression, etc.). However, $\model$ affects the predicted probabilities $\hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta})$ which in turn affect the performance of CL. Hence, in Section \ref{sec:theory}, we examine sufficient conditions where CL finds label errors exactly, even when $\hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta})$ is erroneous. Any model $\model$ may be used for final training on clean data provided by CL.

% Estimating the joint distribution of noisy and true labels $\joint$ requires no hyperparameters and we examine five methods for finding label errors (Sec. \ref{sec:rank_prune_find_errors}) each of which requires no hyperparameters beyond the selection of the method itself.

CL identifies noisy labels in existing datasets to improve learning with noisy labels. The main procedure (see Fig. \ref{fig_flow_examples}) comprises three steps: (1) estimate $\estjoint$ to characterize class-conditional label noise (Sec. \ref{sec:label_noise_characterization}), (2) filter out noisy examples (Sec. \ref{sec:rank_prune_find_errors}), and (3) train with errors removed, reweighting the examples by class weights $\frac{\estprior[i]}{\estjoint[i][i]}$ for each class $i \in [m]$. In this section, we define these three steps and discuss their expected outcomes.

\begin{figure*}[t]
\centerline{\includegraphics[width=.7\linewidth]{img/confident_learning_digram_final.pdf}}
\caption{An example of the confident learning (CL) process. CL uses the confident joint, $\cj$, and $\estjoint$, an estimate of $\joint$, the joint distribution of noisy observed labels $\tilde{y}$ and unknown true labels $y^*$, to find examples with label errors and produce clean data for training.}
    \label{fig_flow_examples}
% \vskip -0.3in
\end{figure*}

% \subsection{Label Noise Characterization: Estimate \texorpdfstring{$\estjoint$}{the joint} via the confident joint \texorpdfstring{$\cj$}{}}
\subsection{Count: Characterize and Find Label Errors using the Confident Joint}
\label{sec:label_noise_characterization}

To estimate the joint distribution of noisy labels $\tilde{y}$ and true labels, $\joint$, we count examples that are likely to belong to another class and calibrate those counts so that they sum to the given count of noisy labels in each class, $|\bm{X}_{\tilde{y}=i}|$. Counts are captured in the \emph{confident joint} ${\cj \in \mathbb{Z}_{\geq 0}}^{m \times m}$, a statistical data structure in CL to directly find label errors. Diagonal entries of $\cj$ count correct labels and non-diagonals capture asymmetric label error counts. As an example, $C_{\tilde{y}\smalleq 3,y^* \smalleq 1} \smalleq 10$ is read, ``Ten examples are labeled \emph{3} but should be labeled \emph{1}.''

In this section, we first introduce the \emph{confident joint} $\cj$ to partition and count label errors. Second, we show how $\cj$ is used to estimate $\joint$ and characterize label noise in a dataset $\bm{X}$. Finally, we provide a related baseline $\bm{C}_{\text{confusion}}$ and consider its assumptions and short-comings (e.g. class-imbalance) in comparison with $\cj$ and CL. CL overcomes these shortcomings using thresholding and collision handling to enable robustness to class imbalance and heterogeneity in predicted probability distributions across classes.

\paragraph{The confident joint $\cj$}

$\cj$ estimates $\partition$, the set of examples with noisy label $i$ that actually have true label $j$, by partitioning $\bm{X}$ into estimate bins $\estpartition$. When $\estpartition = \partition$, then $\cj$ exactly finds label errors (proof in Sec. \ref{sec:theory}). $\estpartition$ (note the hat above $\hat{\bm{X}}$ to indicate $\estpartition$ is an estimate of $\partition$) is the set of examples $\bm{x}$ labeled $\tilde{y}\smalleq i$ with \emph{large enough} $\hat{p} (\tilde{y} = j ;\bm{x}, \bm{\theta})$ to likely belong to class $y^*\smalleq j$, determined by a per-class threshold, $t_j$. Formally, the definition of the \emph{confident joint} is

\begin{equation} \label{eqn_paper_confident_joint}
\begin{split}
    \cj[i][j] \coloneqq & \lvert \estpartition  \rvert  \quad \text{where} \\
    \estpartition \coloneqq & \left\{ \bm{x} \in \bm{X}_{\tilde{y} = i} : \; \hat{p} (\tilde{y} = j ;\bm{x}, \bm{\theta})  \ge t_j, \,\, j = \hspace{-18pt} \argmax_{l \in [m] : \hat{p} (\tilde{y} = l ;\bm{x}, \bm{\theta})  \ge t_l}  \hat{p} (\tilde{y} = l ;\bm{x}, \bm{\theta})  \right\}
\end{split}
\end{equation}

and the threshold $t_j$ is the expected (average) self-confidence for each class
\vspace{-2pt}
\begin{equation} \label{eqn_paper_threshold}
     t_j = \frac{1}{|\bm{X}_{\tilde{y}=j}|} \sum_{\bm{x} \in \bm{X}_{\tilde{y}=j}} \hat{p}(\tilde{y}=j; \bm{x}, \bm{\theta})
\end{equation}


Unlike prior art, which estimates label errors under the assumption that the true labels are $\tilde{y}^*_k = \argmax_{i \in [m]} \hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta})$~\citep{chen2019confusion}, the thresholds in this formulation improve CL uncertainty quantification robustness to (1) heterogeneous class probability distributions and (2) class-imbalance. For example, if examples labeled $i$ tend to have higher probabilities because the model is over-confident about class $i$, then $t_i$ will be proportionally larger; if some other class $j$ tends toward low probabilities, $t_j$ will be smaller. These thresholds allow us to guess $y^*$ in spite of class-imbalance, unlike prior art which may guess over-confident classes for $y^*$ because $\argmax$ is used \citep{kilian_weinberger_calibration_Guo2017_icml}. We examine ``how good'' the probabilities produced by model $\model$ need to be for this approach to work in Section \ref{sec:theory}.

To disentangle Eqn. \ref{eqn_paper_confident_joint}, consider a simplified formulation:
\begin{align}
    \hat{\bm{X}}^{\text{(simple)}}_{ \tilde{y} \smalleq i,y^* \smalleq j} &  = \{\bm{x} \in \bm{X}_{\tilde{y} = i} : \,\, \hat{p} (\tilde{y} = j ;\bm{x}, \bm{\theta})  \ge t_j \} \nonumber
\end{align}


The simplified formulation, however, introduces \emph{label collisions} when an example $\bm{x}$ is confidently counted into more than one $\estpartition$ bin. Collisions only occur along the $y^*$ dimension of $\cj$ because $\tilde{y}$ is given. We handle collisions in the right-hand side of Eqn. \ref{eqn_paper_confident_joint} by selecting $\hat{y}^* \gets \argmax_{j \in [m]} \; \hat{p} (\tilde{y} = j ;\bm{x}, \bm{\theta})$ whenever $\lvert \left\{ k \smallin [m] : \hat{p} (\tilde{y} \smalleq k ;\bm{x} \smallin \bm{X}_{\tilde{y} = i}, \bm{\theta})  \ge t_k \right\} \rvert > 1$ (collision). In practice with softmax, collisions sometimes occur for softmax outputs with higher temperature (more uniform probabilities), few collisions occur with lower temperature, and no collisions occur with a temperature of zero (one-hot prediction probabilities).

% T --> ∞, softmax --> uniform
% T --> 0, softmax --> argmax


The definition of $\cj$ in Eqn. \ref{eqn_paper_confident_joint} has some nice properties in certain circumstances.
First, if an example has low (near-uniform) predicted probabilities across classes, then it will not be counted for any class in $\cj$ so that $\cj$ may be robust to pure noise or examples from an alien class not in the dataset.
Second, $\cj$ is intuitive -- $t_j$ embodies the intuition that examples with higher probability of belonging to class $j$ than the expected probability of examples in class $j$ probably belong to class $j$.
Third, thresholding allows flexibility -- for example, the $90^{th}$ percentile may be used in $t_j$ instead of the mean to find errors with higher confidence; despite the flexibility, we use the mean because we show (in Sec. \ref{sec:theory}) that this formulation exactly finds label errors in various settings, and we leave the study of other formulations, like a percentile-based threshold, as future work.


\paragraph{Complexity} We provide algorithmic implementations of Eqns. \ref{eqn_paper_threshold}, \ref{eqn_paper_confident_joint}, and \ref{eqn_calibration} in the Appendix. Given predicted probabilities $\bm{\hat{P}}_{k,i}$ and noisy labels $\tilde{y}$, these require $\mathcal{O}(m^2 + nm)$ storage and arithmetic operations to compute $\cj$, for $n$ training examples over $m$ classes.


\paragraph{Estimate the joint $\estjoint$.} Given the confident joint $\cj$, we estimate $\joint$ as
% \vskip -0.15in
\begin{equation} \label{eqn_calibration}
    \estjointlong = \frac{\frac{\bm{C}_{\tilde{y}=i, y^*=j}}{\sum_{j \in [m]} \bm{C}_{\tilde{y}=i, y^*=j}} \cdot \lvert \bm{X}_{\tilde{y}=i} \rvert}{\sum\limits_{i \in [m], j \in [m]} \left( \frac{\bm{C}_{\tilde{y}=i, y^*=j}}{\sum_{j^\prime \in [m]} \bm{C}_{\tilde{y}=i, y^*=j^\prime}} \cdot \lvert \bm{X}_{\tilde{y}=i} \rvert \right)}
\end{equation}
% \vskip -0.1in
The numerator calibrates $\sum_j \estjointlong = \lvert \bm{X}_i \rvert / \sum_{i \in [m]}  \lvert \bm{X}_i \rvert, \forall i \smallin [m]$ so that row-sums match the observed marginals. The denominator calibrates $\sum_{i,j} \estjointlong = 1$ so that the distribution sums to 1.


\paragraph{Label noise characterization} Using the observed prior $\noisypriorlong = \lvert \bm{X}_i \rvert \, / \, \sum_{i \in [m]}  \lvert \bm{X}_i \rvert $ and marginals of $\joint$, we estimate the latent prior as $\estpriorlong  \coloneqq  \sum_i \estjointlong, \forall j \smallin [m]$; the noise transition matrix (noisy channel) as $\estnmlong \coloneqq \estjointlong / \estpriorlong, \forall i \smallin [m]$; and the mixing matrix \citep{scott19_jmlr_mutual_decontamination} as $\estinvlong \coloneqq \hat{\bm{Q}}^\top_{\tilde{y} \smalleq j,y^* = i} / \noisypriorlong, \forall i \smallin [m]$. As long as $\estjoint \approxeq \joint$, each of these estimators is similarly consistent (we prove this is the case under practical conditions in Sec. \ref{sec:theory}).  Whereas prior approaches compute the noise transition matrices by directly averaging error-prone predicted probabilities \citep{noisy_boostrapping_google_reed_iclr_2015, DBLP:conf/iclr/GoldbergerB17_smodel}, CL is one step removed from the predicted probabilities by estimating noise rates based on counts from $\cj$ -- these counts are computed based on whether the predicted probability is greater than a threshold, relying only on the \emph{relative ranking} of the predicted probability, not its exact value. This feature lends itself to the robustness of confident learning to imperfect probability estimation.


\paragraph{Baseline approach $\bm{C}_{\text{confusion}}$}
To situate our understanding of $\cj$ performance in the context of prior work, we compare $\cj$ with $\bm{C}_{\text{confusion}}$, a baseline based on a single-iteration of the performant INCV method \citep{chen2019confusion}. $\bm{C}_{\text{confusion}}$ forms an $m \times m$ confusion matrix of counts $\lvert \tilde{y}_k = i, y^*_k = j \rvert$ across all examples $\bm{x}_k$, assuming that model predictions, trained from noisy labels, uncover the true labels, i.e. $\bm{C}_{\text{confusion}}$ simply assumes $y^*_k = \argmax_{i \in [m]} \hat{p}(\tilde{y}\smalleq i;\bm{x}_k, \bm{\theta})$. This baseline approach performs reasonably empirically (Sec. \ref{sec:experiments}) and is a consistent estimator for noiseless predicted probabilities (Thm. \ref{thm:exact_label_errors}), but fails when the distributions of probabilities are not similar for each class (Thm. \ref{thm:robustness}), e.g. class-imbalance, or when predicted probabilities are overconfident \citep{kilian_weinberger_calibration_Guo2017_icml}.
%, i.e. if a model struggles with a particular class and yields small probabilities, that class may be under-counted.


\paragraph{Comparison of $\cj$ (confident joint) with $\bm{C}_{\text{confusion}}$ (baseline)}
To overcome the sensitivity of $\bm{C}_{\text{confusion}}$ to class-imbalance and distribution heterogeneity, the \emph{confident joint}, $\cj$, uses per-class thresholding \citep{richard1991neural_thresholding, elkan_cost_sensitive_learning_thresholding} as a form of calibration \citep{hendrycks17baseline}. Moreover, we prove that unlike $\bm{C}_{\text{confusion}}$, the confident joint (Eqn. \ref{eqn_paper_confident_joint}) exactly finds label errors and consistently estimates $\joint$ in more realistic settings with noisy predicted probabilities (see Sec. \ref{sec:theory}, Thm. \ref{thm:robustness}).


\subsection{Rank and Prune: Data Cleaning} \label{sec:rank_prune_find_errors}

Following the estimation of $\cj$ and $\joint$ (Section \ref{sec:label_noise_characterization}), any rank and prune approach can be used to clean data. This \emph{modularity} property allows CL to find label errors using interpretable and explainable ranking methods, whereas prior works typically couple estimation of the noise transition matrix with training loss \citep{DBLP:conf/iclr/GoldbergerB17_smodel} or couple the label confidence of each example with the training loss using loss reweighting \citep{NIPS2013_5073, jiang2018mentornet}. In this paper, we investigate and evaluate five rank and prune methods for finding label errors, grouped into two approaches. We provide a theoretical analysis for Method 2: $\cj$ in Sec. \ref{sec:theory} and evaluate all methods empirically in Sec. \ref{sec:experiments}.

\paragraph{Approach 1: Use off-diagonals of $\cj$ to estimate $\estpartition$} We directly use the sets of examples counted in the off-diagonals of $\cj$ to estimate label errors. %, as discussed in Sec. \ref{sec:label_noise_characterization}.

\textbf{\emph{CL baseline 1: $\bm{C}_{\text{confusion}}$.}} \;\; Estimate label errors as the Boolean vector ${\tilde{y}}_{k} \neq \argmax_{j \in [m]} \hat{p}(\tilde{y} = j; \bm{x}_k, \bm{\theta})$, for all $\bm{x}_k \smallin \bm{X}$, where \emph{true} implies label error and \emph{false} implies clean data. This is identical to using the off-diagonals of $\bm{C}_{\text{confusion}}$ and similar to a single iteration of INCV \citep{chen2019confusion}.

\textbf{\emph{CL method 2: $\cj$.}} \;\; Estimate label errors as $\{\bm{x} \in \estpartition : i \neq j \}$ from the off-diagonals of $\cj$.

\paragraph{Approach 2: Use $n \cdot \estjoint$ to estimate $\lvert \estpartition \rvert$, prune by probability ranking} These approaches calculate $n \cdot \estjoint$ to estimate $\lvert \estpartition \rvert$, the count of label errors in each partition. They either sum over the $y^*$ dimension of $\lvert \estpartition \rvert$ to estimate and remove the number of errors in each class (prune by class), or prune for every off-diagonal partition (\emph{prune by noise rate}). The choice of which examples to remove is made by ranking the examples based on predicted probabilities.

\textbf{\emph{CL method 3: Prune by Class (PBC).}} \;\; For each class $i \in [m]$, select the \\ $n \cdot\sum_{j \in [m] : j \neq i} \left( \hat{\bm{Q}}_{\tilde{y} = i, y^* = j}[i] \right)$ examples with lowest self-confidence $\hat{p}(\tilde{y}=i;\bm{x} \in \bm{X}_i)$ .

\textbf{\emph{CL method 4: Prune by Noise Rate (PBNR).}} \;\; For each off-diagonal entry in $\estjointlong, i \neq j$, select the $n \cdot \estjointlong$ examples $\bm{x} \smallin \bm{X}_{\tilde{y}\smalleq i}$ with max margin $\predprobshortj - \predprobshorti$.
This margin is adapted from \possessivecite{wei2018nomralizedmaxmargin} normalized margin.

\textbf{\emph{CL method 5: C+NR.}} \;\; Combine the previous two methods via element-wise `\emph{and}', i.e. set intersection. Prune an example if both methods PBC and PBNR prune that example.


\paragraph{Learning with Noisy Labels} To train with errors removed, we account for missing data by reweighting the loss by $\frac{1}{\hat{p}(\tilde{y}=i \vert y^* = i)} \smalleq \frac{\estprior[i]}{\estjoint[i][i]}$ for each class $i \smallin [m]$, where dividing by $\estjoint[i][i]$ normalizes out the count of clean training data and $\estprior[i]$ re-normalizes to the latent number of examples in class $i$. CL finds errors, but does not prescribe a specific training procedure using the clean data. Theoretically, CL requires no hyper-parameters to find label errors. In practice, cross-validation might introduce a hyper-parameter: $k$-fold. However, in our paper $k=4$ is fixed in the experiments using cross-validation.

\paragraph{Which CL method to use?} Five methods are presented to clean data. By default we use CL: $\cj$ because it matches the conditions of Thm. \ref{thm:robustness} exactly and is experimentally performant (see Table \ref{table:cifar10_label_error_measures}). Once label errors are found, we observe ordering label errors by the normalized margin: $\hat{p}(\tilde{y} \smalleq i; \bm{x}, \bm{\theta}) - \max_{j \neq i} \hat{p}(\tilde{y} \smalleq j; \bm{x}, \bm{\theta})$ \citep{wei2018nomralizedmaxmargin} works well. %Another option is ordering by self-confidence.






% The latent prior, noise matrix, and mixing noise matrix are given by marginalizing $\estjoint$ estimated in Alg. \ref{alg:calibration}.

% \emph{latent prior}:
% $\estpriorlong  {\scriptstyle \coloneqq }  \sum_i \estjointlong, \forall j \smallin M$

% \emph{noisy channel / noise transition matrix}:
% $\estnmlong {\scriptstyle \coloneqq } \estjointlong / \estpriorlong, \forall i \smallin M$

% \emph{inverse noise matrix}:
% $\estinvlong  {\scriptstyle \coloneqq } \hat{\bm{Q}}^\top_{\tilde{y} \smalleq j,y^* = i} / \noisypriorlong, \forall i \smallin M$, where $\noisypriorlong = \lvert \bm{X}_i \rvert / \sum_{i \in M}  \lvert \bm{X}_i \rvert $

% Note $\noisyprior$ is the prior of the known noisy labels. It is not estimated.



% We typically use cross-validation to compute $\bm{\hat{P}}_{k,i}$ for train sets and a model trained on the train set and fine-tuned with cross-validation on the test set to compute $\bm{\hat{P}}_{k,i}$ for a test set. Any method works as long  $\hat{p}(\tilde{y}=j; \bm{x}, \bm{\theta})$ are out-of-sample, holdout, predicted probabilities.


%Building on the principles of confident learning, the Confident learning algorithm (Alg. \ref{alg:rp} becomes straightforward. Ignoring notional overhead,






% The joint algorithm, Alg.  (\ref{alg:calibration}), extends the confident joint algorithm by calibrating $\cj$ to be a valid joint distribution estimate of $\estjoint$. The calibration steps in Alg. (\ref{alg:calibration}) guarantee $\noisypriorlong = \sum_j \estjointlong$, $\forall i \smallin M$ and $\sum_{i,j} \estjointlong = 1$.






% We conclude this section with two comments. Firstly, our choice to prune instead of relabeling is intentional. Consider an image of the letter `M' mixed into the handwritten digits MNIST dataset with label '8'. The image is detected as an error, but if we relabel, we will still detect an error. Nothing can be done. By pruning labels, we can handle both class-conditional label noise and injected examples from other distributions. Secondly, Confident learning is \emph{not} a convergence algorithm. It runs in a single iteration. There is no benefit to repeatedly running Confident learning because the probabilities in step 1 must be out-of-sample to avoid over-fitting, so there is no reason to re-train the classifier, \emph{clf}, further.


% NOTES ----
% Although Confident learning is inductive, i.e. the learning classifier is intended for prediction on unseen test examples, $t_{k} \smalleq \frac{1}{\vert \datak \vert} \sum_{x \smallin \datak} \hat{p}(\tilde{y} = k ; \bm{x})$


% Clarify that it is two steps. We dont use joint_counts directly because those are counts of examples we are confident in (just so we can get the ratio's correct) -- that number isn't necessarily the right number of examples to remove. this is important to understand and can be tricky for people. By computing inverse noise rate, we can compute the number of examples to remove in terms of counts(s) which is known and the inverse noise rate which is estimated, instead of just in terms of the estimated joint counts. This helps increase robustness in our estimate by directly including known count(s).

% \begin{minipage}[t]{0.49\textwidth}
% \begin{algorithm}[H]
%     \centering
% \caption*{\textbf{The Confident Joint Algorithm}\\for class-conditional label noise characterization}
% \label{alg:cj}
% \begin{algorithmic}
% \Statex \textbf{input} $\bm{\hat{P}}_{k,i}$ an $n \times m$ matrix of out-of-sample predicted probabilities $\bm{\hat{P}}_{k,j}[i][k] \coloneqq \hat{p}(\tilde{y} = k; \bm{x}_i, \bm{\theta})$
% \Statex \textbf{input} $\bm{\tilde{y}}$ an $n \times 1$ array of noisy integer labels
% % \Procedure {ConfidentJoint}{$\bm{\hat{P}}_{k,i}$, $\bm{\tilde{y}}$}
% % \Algphase{Part 1 - Compute thresholds}
% \State $\bm{t} \gets$ $m \times 1$ array of zeros
% \For {$k \gets 1,m$}  \Comment{1. compute thresholds}
% % \State  $t[k] \gets \frac{1}{\vert \datak \vert} \sum_{x \smallin \datak} \hat{p}(\tilde{y} = k ; \bm{x})$
% \For {$i \gets 1,n$}
% \State $S \gets \emptyset$
% \If {$\bm{\tilde{y}}[i] = k$}
% \State $S \gets S \cup \{\bm{\hat{P}}_{k,j}[i][k]\}$
% \EndIf
% \EndFor
% \State $\bm{t}[k] \gets average(S)$
% \EndFor

% % \Algphase{Part 2 - Compute Confident Joint}
% \State $\bm{C} \gets$ $m \times m$ matrix of zeros
% \For {$i \gets 1,n$} \Comment{2. compute confident joint}
% \State $cnt \gets 0$
% \For {$k \gets 1,m$}
% \If {$\bm{\hat{P}}_{k,j}[i][k] \geq t[k] $}
% \State $cnt \gets cnt + 1$
% \State $y^* \gets k$   \Comment{guess of true label}
% \EndIf
% \EndFor
% \State $\tilde{y} \gets \bm{\tilde{y}}[i]$
% \If {$cnt > 1$}  \Comment{if label collision}
% \State $ y^* \gets \argmax{\bm{\hat{P}}_{k,j}[i] }$ \Comment{use max prob}
% \EndIf
% \If {$cnt > 0$}
% \State $\bm{C}[\tilde{y}][y^*] \gets \bm{C}[\tilde{y}][y^*] + 1$
% \EndIf
% \Statex \textbf{output} $\bm{C}$ an {$\scriptsize m \times m$} unnormalized counts matrix
% \EndFor
% % \EndProcedure
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.49\textwidth}
% \begin{algorithm}[H]
%     \centering
% \caption*{\textbf{The Joint Algorithm} calibrates the confident joint to estimate the true distribution of label noise}
% \label{alg:calibration}
% \begin{algorithmic}
% \Statex \textbf{input} $\bm{C}$ the confident joint
% \Statex \textbf{input} $\bm{\tilde{y}}$ an $n \times 1$ array of noisy integer labels
% \State $x = y$
%     \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% [4]{L}[0pt]{0pt}


% \begin{algorithm}
% \caption{(\textbf{Label Noise Characterization})}
% \label{alg:cj}
% \begin{algorithmic}
% % \STATE \hspace{-.15in} {\sc notation}: $M$: \textit{set of unique class labels, $\bm{X}$: set of input examples, $s$: noisy label, $y$: actual (latent)}
% % \STATE \hspace{.55in} \emph{label}. $s$ and $y$ are discrete random variables. They take any value in set $M$, e.g. $\tilde{y} = \text{`cat.'}$

% \STATE \hspace{-.1in} {\sc \textbf{input}:} noisy labels, $\tilde{y})$; \emph{any} classifier, \emph{clf}
% \STATE \hspace{-.1in} {\sc \textbf{output}:} $C_{s,y}$, $P_{s,y}$, \emph{clf} trained on error-free subset of labels, and the label errors, $s(\mathbf{X}_{err})$

% \STATE 1.  {\small\textsc{\textbf{transductive probs}:}} {\small Compute} $\hat{p}(\tilde{y} = j ; \bm{x} \in X) \, \forall j \smallin M, x \smallin X$ {\small using cross validation.}

% \STATE 2.  {\small\textbf{\textsc{c-joint:}}} $C_{s,y} = \vert  \{x \smallin \dataj \, \vert \,  \hat{p}(\tilde{y} = k ; \bm{x}) \geq t_k \} \vert, {\scriptstyle \forall j, k \smallin M}$, {\tiny where} $t_{k} \smalleq \frac{1}{\vert \datak \vert} \sum_{x \smallin \datak} \hat{p}(\tilde{y} = k ; \bm{x})$

% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
% \caption{(\textbf{Confident learning}): A general solution for multiclass learning with noisy labels}
% \label{alg:rp}
% \begin{algorithmic}
% \STATE \hspace{-.15in} {\sc notation}: $M$: \textit{set of unique class labels, $\bm{X}$: set of input examples, $s$: noisy label, $y$: actual (latent)}
% \STATE \hspace{.55in} \emph{label}. $s$ and $y$ are discrete random variables. They take any value in set $M$, e.g. $\tilde{y} = \text{`cat.'}$

% \STATE \hspace{-.1in} {\sc \textbf{input}:} feature matrix, $\mathbf{X}$; associated noisy labels, $s(\mathbf{X})$; \emph{any} classifier, \emph{clf}
% \STATE \hspace{-.1in} {\sc \textbf{output}:} $C_{s,y}$, $P_{s,y}$, \emph{clf} trained on error-free subset of labels, and the label errors, $s(\mathbf{X}_{err})$

% \STATE 1.  {\small\textsc{\textbf{transductive probs}:}} {\small Compute} $\hat{p}(\tilde{y} = j ; \bm{x} \in X) \, \forall j \smallin M, x \smallin X$ {\small using cross validation.}

% \STATE 2.  {\small\textbf{\textsc{c-joint:}}} $C_{s,y} = \vert  \{x \smallin \dataj \, \vert \,  \hat{p}(\tilde{y} = k ; \bm{x}) \geq t_k \} \vert, {\scriptstyle \forall j, k \smallin M}$, {\tiny where} $t_{k} \smalleq \frac{1}{\vert \datak \vert} \sum_{x \smallin \datak} \hat{p}(\tilde{y} = k ; \bm{x})$

% \STATE 3. {\small\textsc{\textbf{calibration}:}} $n \Hat{P}_{s,y} =  \frac{n}{\sum_j \sum_k C_{\tilde{y} = j , y^* = k}} \cdot C_{s,y} $ $\qquad\triangleright$ {\small $n \Hat{P}_{s,y}$ is just unnormalized $\Hat{P}_{s,y}$, as counts}.

% %\STATE 4.  {\small\textsc{\textbf{find errors}:}} $X_{err} = \{x \smallin \dataj \, \vert \,  \hat{p}(\tilde{y} = k \vert \bm{x}) > t_{j,k}, {\scriptstyle \forall j \in M, k } \}$, {\tiny where} $t_{j,k}$ {\small is the} $C_{s \tinyeq j,y \tinyeq k}^{th}$ {\small largest} $ \hat{p}(\tilde{y} = k \vert \bm{x} \smallin \dataj)$

% \STATE 4.  {\small\textsc{\textbf{find errors}:}} $X_{{\scriptstyle err}} = \{x \smallin \dataj$ {\small with} $n \Hat{P}_{s \tinyeq j,y \tinyeq k}$ {\small largest} $ \hat{p}(\tilde{y} \smalleq k ; \bm{x}), \, {\scriptstyle \forall j, k \smallin M,\color{red}{j \neq k} } \}$ $ \triangleright$ {\tiny use BFPRT (1973).}

% \STATE 5. {\small\textsc{\textbf{prune}:}} $X_{{\scriptscriptstyle conf}} = X \setminus X_{{\scriptstyle err}} \quad \triangleright$ {\small`$\setminus$' means `set difference,' i.e. $X_{{\scriptscriptstyle conf}}$ is the subset of $\bm{X}$ without $X_{{\scriptscriptstyle err}}$ }

% \STATE 6.  {\small\textsc{\textbf{re-train}:}} Train \emph{clf} with ${X}_{{\scriptscriptstyle conf}}, s(\mathbf{X}_{{\scriptscriptstyle conf}})$, {\small and class weights} $\frac{1}{\hat{p}(\tilde{y} \smalleq k \vert y^* \smalleq k)} \forall k \smallin M  \triangleright$ {\tiny $\hat{p}(\tilde{y} \smalleq k \vert y^* \smalleq k)$ via Alg. \ref{alg:latent}}

% %\geq \text{the} C_{s,y}^{th} \text{largest}  \hat{p}(\tilde{y} = j ; \bm{x}) \}$

% % Prune $\hat{\pi}_{k}s_{k}$ examples in each set $\{x|\tilde{y} = \tilde{k}\}$ that has the smallest $g_{k}(x)$. Refit the pruned set with reweighting coefficient $\frac{1}{p(\tilde{y}=k^*|y^* =k^*)}$

% \end{algorithmic}
% \end{algorithm}


% $\hat{p}(\tilde{y} = k ; \bm{x}) \leftarrow$
% \begin{algorithm}
%   \caption{: \textbf{Multiclass Learning with Noisy Labels}}
%   \label{alg:rp}
% \begin{algorithmic}
%   \INPUTS{Feature matrix $\bm{X}$, noisy labels $s$, classifier \emph{clf}}
%   \STATE 1. $\hat{p}(\tilde{y} = j | \bm{x}) \leftarrow$ \emph{clf}.cross\_val\_predict($\bm{X}$,$s$)  \ \ $\triangleright \; k$ classes
%   \textbf{Estimate noise matrix $\nm_{kl}$}:
%   \STATE 2. $\hat{\nm}_{kl} =  \frac{count(\tilde{y} = \tilde{k}, g_{l}(x) \geq p(\hat{s}=l \vert \tilde{y} = l)}{count(g_{l}(x) \geq p(\hat{s}=l \vert \tilde{y} = l)}$
%   \STATE 3. Obtain the inverse noise rates:
%   \STATE \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $\hat{\pi}_{k} = 1 - \frac{\hat{N}_{kk}}{s_{k}} (\hat{\nm}^{-1}\mathbf{s})_{k}$
%   \STATE where $\mathbf{s} = (s_{1}, s_{2}, ... s_{k})^{T}$ and $s_{k} = |\{x|\tilde{y} = \tilde{k}\}|, k = 1,2, ... M$
%   \STATE 4. Prune $\hat{\pi}_{k}s_{k}$ examples in each set $\{x|\tilde{y} = \tilde{k}\}$ that has the smallest $g_{k}(x)$. Refit the pruned set with reweighting coefficient $\frac{1}{p(\tilde{y}=j|y^* =k)}$
%   \STATE {\bfseries Output:} clf with trained weights/parameters, and estimated noise matrix $\nm$
% \end{algorithmic}
% \end{algorithm}


% Although MRP may seem similar to RP, the pruning step is fundamentally different. Pruning is done based on the estimated $\hat{p}(y^* =k \vert \bm{x})$, not the noisy, observable $\hat{p}(\tilde{y}=j)$.


% By construction, MRP for two classes ($m = 2$) is equivalent to binary Rank Pruning and similarly by construction, the guarantees \citep{northcutt2017Confident learning} are the same. Thus, noise rate estimation is provably consistent (exact) consistency when probability estimation is perfect and the class distributions do not overlap. When these conditions are relaxed, the closed-form solutions from binary Rank Pruning are applicable to MRP. MRP has equivalent expected risk as learning with uncorrupted labels for both perfect probability estimation and imperfect probability estimation in the range-seperable case \citep{northcutt2017Confident learning}. The only assumption underlying these proofs is we assume $N \rightarrow \infty$ such that the true hidden distributions contain infinite examples.

% \begin{algorithm}
% \caption{(\textbf{robust latent estimation}): A solution for latent noisy channel and prior estimation}
% \label{alg:latent}
% \begin{algorithmic}
% \STATE \hspace{-.1in} {\sc \textbf{input}:} $C_{s,y}$, the confident joint, $p(s)$, prior of given labels.
% \STATE \hspace{-.1in} {\sc \textbf{output}:} Returns estimates for $\hat{p}(y), \hat{P}_{s \vert y}, \hat{P}_{y \vert s}$

% \STATE 0.  {\small\textsc{\textbf{prior counts}:}} $C_{\tilde{y} \smalleq j} = \sum_{k \smallin M} C_{\tilde{y} \smalleq j,y^* \smalleq k}, \forall j \smallin M, \quad C_{y^* \smalleq k} = \sum_{j \in M} C_{\tilde{y} \smalleq j,y^* \smalleq k}, \forall k \smallin M$

% \STATE 1.  {\small\textsc{\textbf{estimate latent prior}:}} $\hat{p}(y^* \smalleq k) = C_{y^* \smalleq k} / C_{\tilde{y} \smalleq k} \cdot p(\tilde{y} \smalleq k), \forall k \smallin M$

% \STATE 2.  {\small\textsc{\textbf{estimate latent noisy channel}:}} $\hat{P}_{s \vert y^* \smalleq k} = C_{s,y^* \smalleq k} / C_{y^* \smalleq k}, \forall k \smallin M$

% \STATE 3.  {\small\textsc{\textbf{estimate latent inverse noise matrix}:}} $\hat{P}_{y \vert \tilde{y} \smalleq j} = C^\top_{\tilde{y} \smalleq j,y} / C_{\tilde{y} \smalleq j}, \forall j \smallin M$


% \end{algorithmic}
% \vskip -0.05in
% \end{algorithm}








==> Confident Learning (JAIR 2021) (Version 6610)/related-work.tex <==
\section{Related work}
\label{sec:related}

% 1. confident learning can estimate joint label distribution
% 2. confident learning can estimate multi-class labels
% 3. confident learning is effective for non-uniform noise (differ from most robust learning methods that deal with uniform noise). Compared to prior work on non-uniform noise, confident learning is model agnostic, and has theoretical justification.

We first discuss prior work on confident learning, then review how CL relates to noise estimation and robust learning.

\paragraph{Confident learning} \; Our results build on a large body of work termed ``confident learning''. \citet{elkan_cost_sensitive_learning_thresholding} and \citet{forman2005counting} pioneered counting approaches to estimate false positive and false negative rates for binary classification. We extend counting principles to multi-class setting. To increase robustness against epistemic error in predicted probabilities and class imbalance, \citet{Elkan:2008:LCO:1401890.1401920} introduced thresholding, but required uncorrupted positive labels. CL generalizes the use of thresholds to multi-class noisy labels. CL also reweights the loss during training to adjust priors for the data removed. This choice builds on formative works \citep{NIPS2013_5073, rooyen_menon_unhinged_nips15} which used loss reweighting to prove equivalent empirical risk minimization for learning with noisy labels. 
More recently, \citet{deep_self_learning_arxiv_2019} proposed an empirical deep self-supervised learning approach to avoid probabilities by using embedding layers of a neural network. In comparison, CL is non-iterative and theoretically grounded. \citet{icml_lipton_label_shift_confusion_matrix} estimate label noise using approaches based on confusion matrices and cross-validation. However, unlike CL, the former assumes a less general form of label shift than class-conditional noise. \cite{o2unet_iccv} demonstrate the empirical efficacy of first finding label errors, then training on clean data, but the study evaluates only uniform (symmetric) and pair label noise -- CL augments these empirical findings with theoretical justification for the broader class of asymmetric and class-conditional label noise.
% Like CL, \citet{icml_lipton_label_shift_confusion_matrix} and \citet{chen2019confusion} estimate label noise using approaches based on confusion matrices and cross-validation. However, unlike CL the former assumes a specific form of label shift and the latter, \emph{INCV}, uses an iterative pruning approach comparable to the $\bm{C}_{\text{confusion}}$ baseline. An extensive comparison of \emph{INCV} and CL is available in the Appendix (see Sec. \ref{sec:compare_incv_and_cl}).

% \textbf{Label noise estimation (binary).} \;
% % Early work in learning with noisy labels is often restricted to binary classification. %To our knowledge, the only model-agnostic, time-efficient solution for noise rate estimation is binary rankpruning \citep{northcutt2017rankpruning}. 
% % For example, 
% \citet{scott2015rate} developed a theoretical and practical convergence criterion in the binary setting. With the simplifying assumption that all positive labels are error-free, \citet{Elkan:2008:LCO:1401890.1401920} introduced a formative time-efficient probabilistic approach that directly estimates the probability of label flipping using a holdout set. \citet{northcutt2017rankpruning} introduced learning with confident examples for binary classification by a calibration technique. Assuming the noise rates are given (which in practice is rarely true), a variety of algorithms achieved equivalent expected risk as learning with binary uncorrupted labels. In contrast to these studies, CL can estimate the label noise for multi-class classification.

\paragraph{Theory: a model-free, data-free approach} Theoretical analysis with noisy labels often assumes a restricted class of models or data to disambiguate model noise from label noise. For example, \cite{ICML_iterative_trimmed_loss} provide theoretical guarantees for learning with noisy labels in a more general setting than CL that includes adversarial examples and noisy data, but limit their findings to generalized linear models. CL theory is model and dataset agnostic, instead restricting the magnitude of example-level noise. In a formative related approach, \cite{neurips2019novelinformationtheory} prove that using the loss function $-\log \left(\vert \det (\joint) \right) \rvert$ enables noise robust training for any model and dataset, further justified by performant empirical results. Similar to confident learning, their approach hinges on the use of $\joint$, however, they require that $\nm$ is invertible and estimate $\joint$ using $\bm{C}_{\text{confusion}}$, which is sensitive to class-imbalance and heterogeneous class probability distributions (see Sec. \ref{sec:label_noise_characterization}). In Sec. \ref{sec:theory}, we show sufficient conditions in Thm. \ref{thm:robustness} where $\cj$ exactly finds label errors, regardless of each class's probability distribution.

\paragraph{Uncertainty quantification and label noise estimation} \; A number of formative works developed solutions to estimate noise rates using convergence criterion \citep{scott2015rate}, positive-unlabeled learning \citep{Elkan:2008:LCO:1401890.1401920}, and predicted probability ratios \citep{northcutt2017rankpruning}, but are limited to binary classification. Others prove equivalent empirical risk for \emph{binary} learning with noisy labels \citep{NIPS2013_5073,Liu:2016:CNL:2914183.2914328,Sugiyama:2012:DRE:2181148} assuming noise rates are known, which is rarely true in practice. Unlike these binary approaches, CL estimates label uncertainty in the multiclass setting, where prior work often falls into five categories: (1) theoretical contributions \citep{scott19_jmlr_mutual_decontamination}, (2) loss modification for label noise robustness \citep{DBLP:conf/icml/PatriniNNC16, patrini2017making, Sukhbaatar_fergus_iclr_2015, rooyen_menon_unhinged_nips15}, (3) deep learning and model-specific approaches \citep{Sukhbaatar_fergus_iclr_2015, DBLP:conf/icml/PatriniNNC16, 7837934_multiclass_learning_with_noise_using_dropout}, (4) crowd-sourced labels via multiple workers \citep{zhang2017improving, dawid1979maximum, ratner_chris_re_large_training_sets_NIPS2016_6523}, (5) factorization, distillation \citep{Li_distillation2017}, and imputation \citep{amjad_devavrat_svd_imputation_2017} methods, among other \citep{Saez2014_multiclass_learning_by_binary_subproblem}. 
%All of these methods are either model specific, computationally expensive, require a correctly labeled (anchor) data, or assume the noisy channel (flipping rates) are given, which is rarely the case.
Unlike these approaches, CL provides a consistent estimator for exact estimation of the joint distribution of noisy and true labels directly, under practical conditions.

\paragraph{Label-noise robust learning} \; Beyond the above noise estimation approaches, extensive studies have investigated training models on noisy datasets, e.g. \citep{beigman2009learning,brodley1999identifying}. Noise-robust learning is important for deep learning because modern neural networks trained on noisy labels generalize poorly on clean validation data~\citep{zhang2017understanding}. A notable recent rend in noise robust learning is benchmarking with symmetric label noise in which labels are uniformly flipped, e.g.~\citep{DBLP:conf/iclr/GoldbergerB17_smodel,arazo2019unsupervised}. However, noise in real-world datasets is highly non-uniform and often sparse. For example, in ImageNet \citep{ILSVRC15_imagenet}, \emph{missile} is likely to be mislabeled as \emph{projectile}, but has a near-zero probability of being mislabeled as most other classes like \emph{wool}, \emph{ox}, or \emph{wine}. To approximate real-world noise, an increasing number of studies examined asymmetric noise using, e.g. loss or label correction~\citep{patrini2017making,noisy_boostrapping_google_reed_iclr_2015,DBLP:conf/iclr/GoldbergerB17_smodel}, per-example loss reweighting~\citep{jiang2020beyond,jiang2018mentornet,shu2019meta}, Co-Teaching~\citep{han2018coteaching}, semi-supervised learning~\citep{hendrycks2018using,Li_distillation2017,vahdat2017toward}, symmetric cross entropy~\citep{wang2019sceloss_symmetric}, and semi-supervised learning~\citep{iclr_li2020dividemix}, among others. These approaches work by introducing novel new models or insightful modifications to the loss function during training. CL takes a loss-agnostic approach, instead focusing on generating clean data for training by directly estimating of the joint distribution of noisy and true labels.

\paragraph {Comparison of the INCV Method and Confident Learning} \label{sec:compare_incv_and_cl}

The INCV algorithm \citep{chen2019confusion} and confident learning both estimate clean data, use cross-validation, and use aspects of confusion matrices to deal with label errors in ML workflows. Due to these similarities, we discuss four key differences between confident learning and INCV.

First, INCV errors are found using an iterative version of the $\bm{C}_{\text{confusion}}$ confident learning baseline: any example with a different given label than its argmax prediction is considered a label error. This approach, while effective (see Table \ref{table:cifar10_benchmark}), fails to properly count errors for class imbalance or when a model is more confident (larger or smaller probabilities on average) for certain class than others, as discussed in Section \ref{sec:theory}. To account for this class-level bias in predicted probabilities and enable robustness, confident learning uses theoretically-supported (see Section \ref{sec:theory}) thresholds \citep{elkan_cost_sensitive_learning_thresholding, richard1991neural_thresholding} while estimating the confident joint. Second, a major contribution of CL is finding the label errors in the presumed error-free benchmarks such as ImageNet and MNIST, whereas INCV emphasizes empirical results for learning with noisy labels. Third, in each INCV training iteration, 2-fold cross-validation is performed. The iterative nature of INCV makes training slow (see Appendix Table \ref{table:incv_stuff}) and uses fewer data during training. Unlike INCV, confident learning is not iterative. In confident learning, cross-validated probabilities are computed only once beforehand from which the joint distribution of noisy and true labels is directly estimated which is used to identify clean data to be used by a single pass re-training. We demonstrate this approach is experimentally performant without iteration (see Table \ref{table:cifar10_benchmark}). Finally, confident learning is modular. CL approaches for training, finding label errors, and ordering label errors for removal are independent. In INCV, the procedure is iterative, and all three steps are tied together in a single looping process. A single iteration of INCV equates to the $\bm{C}_{\text{confusion}}$ baseline benchmarked in this paper.


% These works take a model-centric approach, creating a new model or modifying the loss function for the purpose of \emph{ learning in spite of noise}. CL instead takes a data-centric approach, directly estimating the joint distribution of noisy and true labels and cleaning the dataset before re-training, with the purpose of \emph{learning without noise}. 


%Common approaches to learning with noisy labels include iterative co-training \citep{Blum:1998:CLU:279943.279962}, modifying the loss \citep{DBLP:conf/icml/PatriniNNC16, patrini2017making, Sukhbaatar_fergus_iclr_2015}, imputation \citep{Li_distillation2017, amjad_devavrat_svd_imputation_2017},  crowd-based approaches \citep{zhang2017improving, dawid1979maximum, ratner_chris_re_large_training_sets_NIPS2016_6523}, error removal \citep{pmlr-icml2018-Kamalika-Chaudhuri, northcutt2017rankpruning}, or fixing labels \citep{deep_self_learning_arxiv_2019}. Works in these areas introduced a number of grand insights used in CL, discussed in the next subsection. 

%Unlike prior works, confident learning offers an unsupervised, model-agnostic way to overcome, as well as estimate, noise of provable theoretical properties. Our experiments verify its competitive performance on CIFAR and its effectiveness in identifying noise in ImageNet.


% In the rest of this section, we consider related works as they relate to eight features of confident learning. We summarize a comparison of commonly benchmarked prior art across six of these features in Table \ref{t:related_works}, limiting our focus to \emph{model-agnostic} approaches that \emph{do not require true labels}.

% \textbf{Model agnostic} \; model specific approaches are \citep{DBLP:conf/icml/PatriniNNC16, 7837934_multiclass_learning_with_noise_using_dropout}

% \textbf{Doesn't need true labels} \; requires a subset of true labels \citep{}

% \begin{table*}[ht] 
% \renewcommand{\arraystretch}{.5}% Makes table rows tighter
% \caption{Comparison of commonly benchmarked approaches for learning with noisy labels. Comparison is limited to model-agnostic approaches that do not require a subset of true labels.  \todo{Lu, please check these checkmarks -- thanks!}}
% \vskip -.1in
% \label{t:related_works}
% % \begin{center}
% % \begin{small}
% % \begin{sc}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccc} 
% \toprule

% \textbf{Related Work} & \textbf{Est. Noise} & \textbf{Multi-} & \textbf{Find/Estim.} &  \textbf{Non}  & \textbf{Theory} & \textbf{Doesn't Assume} \\
%                       & \textbf{Transition} &  \textbf{class}   & \textbf{Label Errors} & \textbf{Iterative} & \textbf{Support} & \textbf{Uniform Noise} \\
% \midrule
% \cite{NIPS2013_5073} &            &   &   & \checkmark  & \checkmark & \checkmark\\
% \midrule
% \cite{noisy_boostrapping_google_reed_iclr_2015} &  \checkmark  & \checkmark &   & \checkmark  & & \checkmark\\
% \midrule % \href{DBLP:conf/iclr/GoldbergerB17_smodel}{S-Model (ICLR, 2017)}
% \cite{DBLP:conf/iclr/GoldbergerB17_smodel} & \checkmark &  \checkmark &            & \checkmark &  & \checkmark\\
% % \midrule
% % \cite{lee2018cleannet} &            & \checkmark & \checkmark & \checkmark &            & \checkmark & \checkmark &\\
% \midrule
% \cite{jiang2018mentornet} &  & \checkmark & \checkmark & &  & \\

% \toprule
% \textbf{Confident Learning (2019)} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

% \bottomrule
% \end{tabular}
% }
% % \end{sc}
% % \end{small}
% % \end{center}
% %  \vskip -0.25in
% \end{table*}


% \textbf{Estimation noise transition matrix} \; \citep{Sukhbaatar_fergus_iclr_2015, DBLP:conf/iclr/GoldbergerB17_smodel, noisy_boostrapping_google_reed_iclr_2015}

% \textbf{Multi-class Label estimation in noisy data} \;  

% \textbf{Find/estimate label errors} \; \citep{forman2005counting}

% \textbf{Non-iterative} \; example of non-iterative approach is \citep{Sukhbaatar_fergus_iclr_2015}

% \textbf{Theoretical support} \; theoretical contributions \citep{scott17_mutual_decontamination, Blanchard_scott_aistats2014}



\endinput

TONS OF RELATED WORKS I still haven't cited !!!!!!!!!!!!

	1. Particle competition and cooperation for semi-supervised learning with label noise
		a. https://www.sciencedirect.com/science/article/pii/S0925231215001277?via%3Dihub
	2. Deep self-learning from noisy labels
		a. https://arxiv.org/pdf/1908.02160.pdf
	3. On the Impacts of Noise from Group-Based Label Collection for Visual Classification
		a. https://ieeexplore.ieee.org/document/8260618
	4. AUTO-encoder for data cleaning and classification with label noise
		a. https://link.springer.com/article/10.1007/s11063-018-9963-9
	5. SOSELETO: A Unified Approach to Transfer Learning and Training with Noisy Labels
		a. https://openreview.net/forum?id=r1lqA-OSvV
	6. AUXILIARY IMAGE REGULARIZATION FOR DEEP CNNS WITH NOISY LABELS
		a. https://arxiv.org/pdf/1511.07069.pdf
	7. WEBVISION DATASET 1.0
		a. https://www.vision.ee.ethz.ch/webvision/2017/index.html
	8. LLD ICLR 2019 workshop - https://lld-workshop.github.io/
	9. Disentagling Factors of Vraitions Using Few Labels
		a. https://openreview.net/forum?id=SkGy6hjvPE
	10. Learning Graph Neural Networks with Noisy Labels
		a. https://openreview.net/forum?id=r1xOmNmxuN
	11. SOSELETO: A Unified Approach to Transfer Learning and Training with Noisy Labels
		a. https://openreview.net/forum?id=r1lqA-OSvV
	12. Why ReLU networks yield high-confidence predictions far away from the training data and how to mitigate the problem
		a. http://www.gatsby.ucl.ac.uk/~balaji/udl2019/accepted-papers/UDL2019-paper-01.pdf
		b. http://openaccess.thecvf.com/content_CVPRW_2019/papers/Uncertainty%20and%20Robustness%20in%20Deep%20Visual%20Learning/Hein_Why_ReLU_networks_yield_high-confidence_predictions_far_away_from_the_CVPRW_2019_paper.pdf
	13. Pumpout: A Meta Approach to Robust Deep Learning with Noisy Labels
		a. http://www.gatsby.ucl.ac.uk/~balaji/udl2019/accepted-papers/UDL2019-paper-14.pdf
	14. Robust conditional GANs under missing or uncertain labels
		a. http://www.gatsby.ucl.ac.uk/~balaji/udl2019/accepted-papers/UDL2019-paper-40.pdf
	15. Incremental Learning with Unlabeled Data in the Wild
		a. http://openaccess.thecvf.com/content_CVPRW_2019/papers/Uncertainty%20and%20Robustness%20in%20Deep%20Visual%20Learning/Lee_Incremental_Learning_with_Unlabeled_Data_in_the_Wild_CVPRW_2019_paper.pdf
	16. Uncertainty Based Detection and Relabeling of Noisy Image Labels
		a. http://openaccess.thecvf.com/content_CVPRW_2019/papers/Uncertainty%20and%20Robustness%20in%20Deep%20Visual%20Learning/Kohler_Uncertainty_Based_Detection_and_Relabeling_of_Noisy_Image_Labels_CVPRW_2019_paper.pdf
	17. Learn To Be Uncertain: Leveraging Uncertain Labels In Chest X-rays With Bayesian Neural Networks
		a. http://openaccess.thecvf.com/content_CVPRW_2019/papers/Uncertainty%20and%20Robustness%20in%20Deep%20Visual%20Learning/Yang_Learn_To_Be_Uncertain_Leveraging_Uncertain_Labels_In_Chest_X-rays_CVPRW_2019_paper.pdf
	18. Automated Label Noise Identification for Facial Attribute Recognition
		a. http://openaccess.thecvf.com/content_CVPRW_2019/papers/Uncertainty%20and%20Robustness%20in%20Deep%20Visual%20Learning/Speth_Automated_Label_Noise_Identification_for_Facial_Attribute_Recognition_CVPRW_2019_paper.pdf
	19. Are Anchor Points Really Indispensable in Label-Noise Learning
		a. https://arxiv.org/abs/1906.00189
	20. Cvpr ROBUSTNESS WORKSHOP -- http://openaccess.thecvf.com/CVPR2019_workshops/CVPR2019_Uncertainty_and_Robustness_in_Deep_Visual_Learning.py
	21. Learning to learn from noisy labeled data
        a. https://arxiv.org/pdf/1812.05214.pdf




Imperfectly labeled datasets are becoming increasingly common \citep{Frenay2014}. We consider milestones in learning with noisy labels, broken into subsections requiring consecutively fewer assumptions. In all cases, and throughout this manuscript, we assume class-conditional noise \citep{angluin1988learning}. Because state-of-the-art model performance changes over time, we focus on approaches that are not limited to a specific classifier or model.

Most prior work in learning with noisy labels assumes is restricted to binary classification. %To our knowledge, the only model-agnostic, time-efficient solution for noise rate estimation is binary rankpruning \citep{northcutt2017rankpruning}. 
For noise estimation, Scott et al. (2013, 2015) \cite{ScottBH13, scott2015rate} developed a theoretical and practical convergence criterion in the binary setting. With the simplifying assumption that all positive labels are error-free, Elkan et al. (2008) \cite{Elkan:2008:LCO:1401890.1401920} introduce a formative time-efficient probabilistic approach that directly estimates the probability of label flipping by averaging predicted probabilities of a holdout set. Assuming the noise rates are given (which in practice is rarely true), a variety of algorithms \cite{NIPS2013_5073}, \cite{Liu:2016:CNL:2914183.2914328}, and \cite{Sugiyama:2012:DRE:2181148} achieve equivalent expected risk as learning with uncorrupted labels, but like Elkan et al. (2008) \cite{Elkan:2008:LCO:1401890.1401920} assume perfect class separability (all predicted probabilities are 0 and 1). %class separability $p(y=k ; x) \in \{0,1\}$ and perfect predicted probabilities $p(\hat{s}=k;x)$. 
Northcutt et al. (2017) \citep{northcutt2017rankpruning} introduced \emph{learning with confident examples}, motivating the development of confident learning more broadly. They re-purposed a calibration technique \citep{Elkan:2008:LCO:1401890.1401920} as a threshold for robust estimation of asymmetric noise rates and learning with noisy labels in the binary setting. In all of these cases, the latent noise rates \cite{NIPS2013_5073}, the mixing rates \cite{scott17_mutual_decontamination}, and the latent prior of the actual labels \cite{lawrence_bayesian_prior_py_noisy_2001, graepel_kernel_gibbs_sampler_prior_py_bayesian_nips_2001} are essential to characterizing label noise. The advantage of confident learning is we estimate the joint noise distribution directly, from which all of the above can be computed.

% Binary Rank Pruning \citep{northcutt2017rankpruning} takes as input training examples $\bm{X}$, noisy labels $s$, and a probabilistic classifier and finds a subset of $X, s$ that is likely to be correctly labeled, i.e. a subset of $X, y$. To do this, two thresholds, $p(\hat{s}=1|s=1)$ and $(\hat{s}=1|s=0)$, are used to \emph{confidently} guess the correctly and incorrectly labeled examples in each of class $s=1$ and $s=0$, forming four sets, then use the set sizes to estimate the noise rates $p(s = 0 | y = 1)$ and $p(s = 1 | y = 0)$. The noise rates are used to estimate and remove the number of examples with observed label $s = 1$ and hidden label $y = 0$ from each class $k$ by removing those with lowest predicted probability $p(s=j;x)$. The classifier is trained using the pruned set, which is intended to represent a subset of the correctly labeled data.



==> Confident Learning (JAIR 2021) (Version 6610)/theory.tex <==
\section{Theory} \label{sec:theory}


In this section, we examine sufficient conditions when (1) the confident joint exactly finds label errors and (2) $\estjoint$ is a consistent estimator for $\joint$. We first analyze CL for noiseless $\predprobshortj$, then evaluate more realistic conditions, culminating in Thm. \ref{thm:robustness} where we prove (1) and (2) with noise in the predicted probabilities for every example. Proofs are in the Appendix (see Sec. \ref{sec:proofs}). As a notation reminder, $\predprobshorti$ is shorthand for $\hat{p}(\tilde{y} \smalleq i; \bm{x}, \bm{\theta})$. 

In the statement of each theorem, we use $\estjoint \approxeq \joint$, i.e. \emph{approximately equals}, to account for precision error of using discrete count-based $\cj$ to estimate real-valued $\joint$. For example, if a noise rate is $0.39$, but the dataset has only 5 examples in that class, the nearest possible estimate by removing errors is $2/5 = 0.4  \approxeq 0.39$. So, $\estjoint$ is technically a \emph{consistent estimator} for $\joint$ only because of discretization error, otherwise all equalities are exact. Throughout, we assume $\bm{X}$ includes at least one example from every class. 


% In Lemma \ref{lemma:ideal_threshold} and Thm. \ref{thm:robustness}, we assume $\lvert \bm{X} \rverte \rightarrow \infty$; however, these results apply to finite-sized $\bm{X}$ omitting the precision error of estimating a real-valued $\joint$ from discrete count-based $\cj$. 



% \textbf{Per-Class Diffracted Condition} \;
% $\predprobshorti$ is \emph{per-class diffracted} if there exist linear combinations of class-conditional error in the predicted probabilities s.t. $\predprobshorti = \epsilon_i^{(1)} \perfprobshorti + \epsilon_i^{(2)}$ where $\epsilon_i^{(1)}, \epsilon_i^{(2)} \sim \mathcal{N}(0,\sigma^{2})), \sigma \smallin \mathbb{R}^+$. This relaxes the ideal condition with a noise model relevant for neural networks, known to be class-conditionally overly confident \citep{kilian_weinberger_calibration_Guo2017_icml}. 

% \textbf{Per-Example Diffracted Condition} \;
% $\predprobshorti$ is \emph{per-example diffracted} if there exist linear combinations of error in the predicted probabilities s.t. $ \forall l \smallin [m], i \smallin [m], j \smallin [m], \forall \bm{x} \smallin \bm{X}_{\tilde{y}=i, y^*=j}, \; \predprobshortl = \epsilon_{i,j,l}^{(1)} \cdot \perfprobshortl + \epsilon_{i,j,l}^{(2)}$ where $\epsilon_{i,j,l}^{(1)}, \epsilon_{i,j,l}^{(2)} \sim \mathcal{N}(\epsilon_i,\sigma^{2})), \epsilon_i \smalleq \mathop{\mathbb{E}}_{\bm{x} \in \bm{X}} \epsilon_{\bm{x}, i}, \sigma \smallin \mathbb{R}^+$. \todo{figure out $\epsilon_i$ expectation, currently this is wrong} This is our least-assuming condition with Gaussian noise for each $\bm{x} \smallin \bm{X}_{\tilde{y}=i, y^*=j}$ set, for each class $l \smallin [m]$.






 

\subsection{Noiseless Predicted Probabilities}

We start with the \emph{ideal} condition and a non-obvious lemma that yields a closed-form expression for threshold $t_i$ when $\predprobshorti$ is ideal. Without some condition on $\predprobshorti$, one cannot disambiguate label noise from model noise. 

% \textbf{Ideal Condition} \;
\begin{condition}[Ideal]
The predicted probabilities $\pyx$ for a model $\theta$ are \emph{ideal} if $\forall \bm{x}_k \smallin \bm{X}_{y^* \tinyeq j}, i \smallin [m], j \smallin [m]$,
we have that
$\hat{p}(\tilde{y} \smalleq i ; \bm{x}_k \in \bm{X}_{y^* \tinyeq j}, \bm{\theta}) = p^*(\tilde{y} \smalleq i \vert y^* \smalleq y_k^*) = p^*(\tilde{y} \smalleq i \vert y^* \smalleq j)$. \emph{The final equality follows from the class-conditional noise process assumption. The \emph{ideal} condition implies error-free predicted probabilities: they match the noise rates corresponding to the $y^*$ label of $\bm{x}$. We use $\perfprobshorti$ as a shorthand.}
\end{condition}

\begin{lemma}[Ideal Thresholds] \label{lemma:ideal_threshold} %Proof \ref{proof:ideal_threshold}.4 in Supp. Mats. \\
For a noisy dataset $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ and model $\model$, 
if $\hat{p}(\tilde{y}; \bm{x}, \model)$ is \emph{ideal}, then 
$\forall i \smallin [m], t_i = \sum_{j \smallin [m]} p(\tilde{y} = i \vert y^* \smalleq j) p(y^* \smalleq j \vert \tilde{y} = i)$.
\end{lemma}

This form of the threshold is intuitively reasonable: the contributions to the sum when $i=j$ represents the probabilities of correct labeling, whereas when $i\neq j$, the terms give the probabilities of mislabeling $p(\tilde{y} = i \vert y^* = j)$, weighted by the probability $p(y^* = j \vert \tilde{y} = i)$ that the mislabeling is corrected. Using Lemma \ref{lemma:ideal_threshold} under the ideal condition, we prove in Thm. \ref{thm:exact_label_errors} confident learning exactly finds label errors and $\estjoint$ is a consistent estimator for $\joint$ when each diagonal entry of $\nm$ maximizes its row and column. The proof hinges on the fact that the construction of $\cj$ eliminates collisions.

\begin{theorem}[Exact Label Errors] \label{thm:exact_label_errors} %Proof \ref{proof:exact_label_errors}.4 in Supp. Mats. \\
For a noisy dataset, $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \smallin {(\mathbb{R}^d, [m])}^n$ and model $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$, 
if $\hat{p}(\tilde{y} ; \bm{x}, \bm{\theta})$ is \emph{ideal} and each diagonal entry of $\nm$ maximizes its row and column, 
then $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} = \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$ and $\estjoint \approxeq \joint$ (consistent estimator for $\joint$).
\end{theorem}

% Thm. \ref{thm:exact_label_errors} guarantees Corollary \ref{cor:consistent_estimation} and shows that the confident joint exactly estimates true joint distribution of label noise when input predicted probabilities are ideal and the there are more. 

% \todo{Consider proving the following observation: When assumptions are relaxed, confident learning over-estimates label noise. The addition examples estimated as label errors are an artifact of the }

% \begin{corollary}[Consistent Estimation] \label{cor:consistent_estimation} %Proof \ref{proof:consistent_estimation}.4 in Supp. Mats. \\
% For $(\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ and $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$, 
% if $\hat{p}(\tilde{y} ; \bm{x}, \bm{\theta})$ is ideal and each diagonal entry of $\nm$ maximizes its row and column, 
% then as $n \rightarrow \infty$, $\bm{C}_{\tilde{y}, y^*} \smalleq n \joint$.
% \end{corollary}




While Thm. \ref{thm:exact_label_errors} is a reasonable sanity check, observe that $ y^* \gets \argmax_j \; \hat{p}(\tilde{y} \smalleq i \vert \tilde{y}^* \smalleq i; \bm{x}) $, used by $\bm{C}_{\text{confusion}}$, trivially satisfies Thm. \ref{thm:exact_label_errors} if the diagonal of $\nm$ maximizes its row and column. We highlight this because $\bm{C}_{\text{confusion}}$ is the variant of CL most-related to prior work (e.g., \citet{chen2019confusion}). We next consider relaxed conditions \emph{motivated by real-world settings}~(e.g., \citet{jiang2020beyond}) where $\cj$ exactly finds label errors ($\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} = \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$) and consistently estimates the joint distribution of noisy and true labels ($\estjoint \approxeq \joint$), but $\bm{C}_{\text{confusion}}$ does not.



\subsection{Noisy Predicted Probabilities}

 
% While $\bm{C}_{\text{confusion}}$ assumes the similar distributions of probabilities for each class. 
Motivated by the importance of addressing class imbalance and heterogeneous class probability distributions, we consider linear combinations of noise per-class. Here, we index $\predprobshortj$ by $j$ to match the comparison $\hat{p} (\tilde{y} \smalleq j ;\bm{x}, \bm{\theta}) \ge t_j$ from the construction of $\cj$ (see Eqn. \ref{eqn_paper_confident_joint}).

\begin{condition} [Per-Class Diffracted]
    $\predprobshortj$ is \emph{per-class diffracted} if there exist linear combinations of class-conditional error in the predicted probabilities s.t. $\predprobshortj = \epsilon_j^{(1)} \perfprobshortj + \epsilon_j^{(2)}$ where $\epsilon_j^{(1)}, \epsilon_j^{(2)} \in \mathbb{R}$ and $\epsilon_j$ can be any distribution. \emph{This relaxes the \emph{ideal} condition with noise that is relevant for neural networks, which are known to be class-conditionally overly confident \citep{kilian_weinberger_calibration_Guo2017_icml}.}
\end{condition}




% In Cor. \ref{cor:per_class_robustness} we relax this assumption so that the diagonal of $\nm$ no longer maximizes its column. %We show this in case 1 of the proof in Thm. \ref{thm:exact_label_errors}.

% When you combine maxcol with ideal probs, np.argmax is sufficient to completely unveil every hidden, true label. in practice this is a ridiculous algorithm because it hinges on the ideal probabilities. Confident learning avoids dealing with probabilities directly except to handle collisions, instead manipulating ratios of counts based on rankings. An example of how this makes confident learning more powerful is shown in Corollary \ref{cor:per_class_robustness}. 

\begin{corollary}[Per-Class Robustness] \label{cor:per_class_robustness} %Proof \ref{proof:robustness}.4 in Supp. Mats.
For a noisy dataset, $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \smallin {(\mathbb{R}^d, [m])}^n$ and model $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$, 
if $\predprobshortj$ is \textbf{per-class diffracted} without label collisions and each diagonal entry of $\nm$ maximizes its row, then $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} = \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$ and $\estjoint \approxeq \joint$.
\end{corollary}

Cor. \ref{cor:per_class_robustness} shows us that $\cj$ in confident learning (which counts $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}$) is robust to any linear combination of per-class error in probabilities. This is not the case for $\bm{C}_{\text{confusion}}$ because Cor. \ref{cor:per_class_robustness} no longer requires that the diagonal of $\nm$ maximize its column as before in Thm. \ref{thm:exact_label_errors}: for intuition, consider an extreme case of per-class diffraction where the probabilities of only one class are all dramatically increased. Then $\bm{C}_{\text{confusion}}$, which relies on $\tilde{y}^*_k \gets \argmax_{i \in [m]} \; \hat{p}(\tilde{y} \smalleq i \vert y^* \smalleq j; \bm{x}_k) $, will count only that one class for all $y^*$ such that all entries in the $\bm{C}_{\text{confusion}}$ will be zero except for one column, i.e. $\bm{C}_{\text{confusion}}$ cannot count entries in any other column, so $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} \neq \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$. In comparison, for $\cj$, the increased probabilities of the one class would be subtracted by the class-threshold, re-normalizing the columns of the matrix, such that, $\cj$ satisfies Cor. \ref{cor:per_class_robustness} using thresholds for robustness to distributional shift and class-imbalance.

Cor. \ref{cor:per_class_robustness} only allows for $m$ alterations in the probabilities and there are only $m^2$ unique probabilities under the ideal condition, whereas in real-world conditions, an error-prone model could potentially output $n \times m$ unique probabilities. Next, in Thm. \ref{thm:robustness}, we examine a reasonable sufficient condition where CL is robust to erroneous probabilities for every example and class.

% \textbf{Per-Example Diffracted Condition} \;
\begin{condition}[Per-Example Diffracted]
$\predprobshortj$ is \emph{per-example diffracted} if $ \forall j \smallin [m], \forall \bm{x} \smallin \bm{X}$, we have error as $\predprobshortj = \perfprobshortj + \errorxj$ where 
\begin{equation} \label{eqn:piecewise_error}
    \errorxj \sim \begin{cases} 
      \mathcal{U}(\epsilon_j \smallplus t_j \smallminus \perfprobshortj \, , \, \epsilon_j \smallminus t_j \smallplus \perfprobshortj] & \perfprobshortj \geq t_j \\
      \mathcal{U}[\epsilon_j \smallminus t_j \smallplus \perfprobshortj \, , \, \epsilon_j \smallplus t_j \smallminus \perfprobshortj) & \perfprobshortj < t_j
  \end{cases}
\end{equation}
where $\epsilon_j = \mathop{\mathbb{E}}_{\bm{x} \in \bm{X}} \big[\errorxj\big]$ and $\mathcal{U}$ denotes a uniform distribution (we discuss a more general case in the Appendix).
\end{condition}

% This is our least-assuming condition allowing model output noise for every example and every class. We analyze the intuition of the distribution bounds in Sec. \ref{sec:theory}.

% When we relax the assumptions of Thm. \ref{thm:exact_label_errors} (no longer requiring that $\nm$ maximizes its column, an important assumption to remove because it enables a trivial solution: $ y^* \gets \underset{j}{\argmax} \; \hat{p}(\tilde{y} = j \vert \tilde{y}^* \smalleq i; x)  $)  and also allow predicting probabilities to be imperfect (\emph{per-class diffracted}), we find that the estimation of the confident joint remains unaffected for examples without label collisions. While we assume Gaussian error (because it is necessary for Thm. \ref{thm:robustness} later on, for Cor. \ref{cor:per_class_robustness} it is not necessary and any $\epsilon_j \smallin \mathbb{R}$ works. This underlies the robustness we find on real datasets in Section~\ref{sec:experiments}.

\begin{theorem}[Per-Example Robustness] \label{thm:robustness} % Proof \ref{proof:robustness}.4 in Supp. Mats. \\
For a noisy dataset, $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ and model $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$, 
if $\predprobshortj$ is \textbf{per-example diffracted} without label collisions and each diagonal entry of $\nm$ maximizes its row, then $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} \approxeq  \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$ and $\estjoint \approxeq \joint$.
\end{theorem}

 

In Thm. \ref{thm:robustness}, we observe that if each example's predicted probability resides within the residual range of the ideal probability and the threshold, then CL exactly identifies the label errors and consistently estimates $\joint$. Intuitively, if $\predprobshortj \geq t_j$ whenever $\perfprobshortj \geq t_j$ and $\predprobshortj < t_j$ whenever $\perfprobshortj < t_j$, then regardless of error in $\predprobshortj$, CL exactly finds label errors. As an example, consider an image $\bm{x}_k$ that is mislabeled as \emph{fox}, but is actually a \emph{dog} where $t_{fox} =0.6$, $p^*(\tilde{y} \smalleq fox; \bm{x} \in \bm{X}_{y^* \smalleq dog}, \bm{\theta}) = 0.2 $, $t_{dog} =0.8$, and  $p^*(\tilde{y} \smalleq dog; \bm{x} \in \bm{X}_{y^* \smalleq dog}, \bm{\theta}) = 0.9 $. Then as long as $-0.4 \leq \epsilon_{\bm{x}, fox} < 0.4$ and $-0.1 < \epsilon_{\bm{x}, dog} \le 0.1$, CL will surmise $y_k^* = dog$, not $fox$, even though $\tilde{y}_k = fox$ is given. We empirically substantiate this theoretical result in Section \ref{sec:exp_imagenet}.

% While $\joint$ is a statistic to characterize aleatoric uncertainty from latent label noise, Thm. \ref{thm:robustness} addresses the epistemic uncertainty in the case of erroneous predicted probabilities.

Thm. \ref{thm:robustness} addresses the \emph{epistemic} uncertainty of latent label noise, via the statistic, $\joint$, while accounting for the \emph{aleatoric} uncertainty of inherently erroneous predicted probabilities.

% $p^*(\tilde{y} \smalleq dog; \bm{x}, \bm{\theta}) = 0.9 $, then CL allows error $-0.3 < \epsilon_{\bm{x}, j} \le 0.3$. If the example had been mislabeled \emph{fox}, but is actually a \emph{dog}, and $p^*(\tilde{y} \smalleq fox; \bm{x} \in \bm{X}_{y^* \smalleq dog}, \bm{\theta}) = 0.2 $, then CL allows error $-0.4 \geq \epsilon_{\bm{x}, j} < 0.4$, i.e. $\hat{p}(\tilde{y} \smalleq fox; \bm{x}, \bm{\theta}) < 0.6 $.
% The insight is that an example's probability need only be greater than or equal to a threshold, not an exact value. 
% Thm. \ref{thm:robustness} generalizes Corollary \ref{cor:per_class_robustness} to the per-example diffracted condition. Thm. \ref{thm:robustness} shows us that with confident learning, $\estjoint$ is still a consistent estimator for $\joint$ even with error in model outputs for every example and class. 

%%% Move following to the Appendix
%%While we use a uniform distribution in Eqn. \ref{eqn:piecewise_error}, any bounded symmetric distribution with mode $\epsilon_j = \mathop{\mathbb{E}}_{\bm{x} \in \bm{X}} \epsilon_{\bm{x}, j}$ is sufficient. Observe that the bounds of the distribution are non-vacuous (they do not collapse to a single value $e_j$) because $t_j \neq \perfprobshortj$ by Lemma \ref{lemma:ideal_threshold}.

% Thm. \ref{thm:robustness} shows us that confident learning exactly finds label errors and perfectly estimates the joint $\estjoint = \joint$ with per-example error as long as for each example the predicted probability resides within the residual range of the ideal probability and the threshold. 



\endinput





\begin{theorem}[Alternate Per-Example Robustness] \label{thm:robustness2} %Proof \ref{proof:general_robustness}.4 in Supp. Mats. \\
For a dataset $\bm{X} \coloneqq (\bm{x}, \tilde{y})^n \in {(\mathbb{R}^d, [m])}^n$ with no label collisions, and a model $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$ that outputs erroneous predicted probabilities with an error term for every example, for every class, such that $ \forall \bm{x}_k \in \bm{X}, \forall j \in [m], \; \hat{p}(\tilde{y} = j ; \bm{x}, \bm{\theta}) = p(\tilde{y} = j \vert y^* = y_k^* + \epsilon_{\bm{x}, j} \coloneqq \perfprobshortj + \epsilon_{\bm{x}, j}$ where $\epsilon_j = \mathop{\mathbb{E}}_{\bm{x} \in \bm{X}} \epsilon_{\bm{x}, j}$ and
\begin{equation} \label{eqn:piecewise_error}
    \epsilon_{\bm{x}, j} \sim \begin{cases} 
      \mathcal{U}(\epsilon_j + t_j - \perfprobshortj \, , \, \epsilon_j - t_j + \perfprobshortj] & \perfprobshortj \geq t_j \\
      \mathcal{U}[\epsilon_j - t_j + \perfprobshortj \, , \, \epsilon_j + t_j - \perfprobshortj) & \perfprobshortj < t_j
  \end{cases}
\end{equation}
if each diagonal entry of $\nm$ maximizes its row, then $\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} = \bm{X}_{\tilde{y} \smalleq i, y^* \smalleq j}$ and $\bm{C}_{\tilde{y}, y^*} \smalleq n \joint$.
\end{theorem}





% Notes to self
% 1. Confident learning mostly cares about the diagonal of the noise matrix in terms of the ideal probabilities. If p(noisy=k|true=k) >= t\_k, for all k, then everything will get counted correctly. It turns out this is true as long as you use argmax when there are collisions.





% \begin{proof} \label{proof:robustness}

% We consider the non-trivial, real-world setting when a learning model $\bm{\theta}{\scriptstyle:} \bm{x} \smallra \hat{p}(\tilde{y})$ outputs erroneous, non-ideal predicted probabilities with an error term added for every example, across every class, such that $ \forall \bm{x} \in \bm{X}, \forall j \in M, \; \hat{p}_{\bm{x}, j} = p(\tilde{y} = j \vert y^* = y_k^* + \epsilon_{\bm{x}, j}$, where $p(\tilde{y} = j \vert y^* = y_k^*$ are ideal probabilities, and 
% \begin{equation*} 
%     \epsilon_{\bm{x}, j} \sim \begin{cases} 
%       uniform(\epsilon_j + t_j - \hat{p}_{\bm{x}, j} \, , \, \epsilon_j - t_j + \hat{p}_{\bm{x}, j}] & \hat{p}_{\bm{x}, j} \geq t_j \\
%       uniform[\epsilon_j - t_j + \hat{p}_{\bm{x}, j} \, , \, \epsilon_j + t_j - \hat{p}_{\bm{x}, j}) & \hat{p}_{\bm{x}, j} < t_j
%   \end{cases}
% \end{equation*} 

% with $\epsilon_j$ denoting the mean of $\epsilon_{\bm{x}, j}$ per class, i.e. $\epsilon_j = \mathop{\mathbb{E}}_{\bm{x} \in \bm{X}} \epsilon_{\bm{x}, j}$ by construction of Eqn. \ref{eqn:piecewise_error}. 

% When there are no label collisions, the bins created by the confident joint are:
% \begin{equation} \label{eqn_robustness_cj_in_general_proof}
%     \hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j} \coloneqq  \{\bm{x} \in \bm{X}_{\tilde{y} = i} : \hat{p}_{\bm{x}, j}  \ge t_j \}
% \end{equation}
% where 
% \begin{equation*}
%     t_j = \frac{1}{|\bm{}{X}_{\tilde{y}=j}|} \sum_{\bm{x} \in \bm{X}_{\tilde{y}=j}}\hat{p}_{\bm{x}, j}
% \end{equation*}

% Rewriting the threshold $t_j$ for a given $e_j$ and $\epsilon_{\bm{x}, j}$, we have
% \begin{align*}
%     t_j^{\epsilon_j} &= \frac{1}{|\bm{}{X}_{\tilde{y}=j}|} \sum_{\bm{x} \in \bm{X}_{\tilde{y}=j}} \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \\
%      &= t_j + \epsilon_j
% \end{align*}


% We complete the proof by showing that
% $$\hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j \iff \hat{p}_{\bm{x}, j}  \ge t_j$$
% If this statement is true then the subsets created by the confident joint in Eqn. \ref{eqn_robustness_cj_in_general_proof} are unaltered and therefore ${\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}} =  {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}$, where ${\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}}$ denotes the confident joint subsets for $\epsilon_{\bm{x}, j}$ predicted probabilities. 

% Now we complete the proof. From Eqn. \ref{eqn:piecewise_error} (the distribution for $\epsilon_{\bm{x}, j}$) , we have that
% \begin{align*}
%     \hat{p}_{\bm{x}, j} < t_j &\implies \epsilon_{\bm{x}, j} < \epsilon_j + t_j - \hat{p}_{\bm{x}, j} \\
%     \hat{p}_{\bm{x}, j} \ge t_j &\implies \epsilon_{\bm{x}, j} \ge \epsilon_j + t_j - \hat{p}_{\bm{x}, j}
% \end{align*}
% Re-arranging
% \begin{align*}
%     \hat{p}_{\bm{x}, j} < t_j &\implies \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} < t_j + \epsilon_j \\
%     \hat{p}_{\bm{x}, j} \ge t_j &\implies \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j
% \end{align*}
% Using the contrapositive, we have
% \begin{align*}
%     \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j &\implies \hat{p}_{\bm{x}, j}  \ge t_j \\
%     \hat{p}_{\bm{x}, j}  \ge t_j &\implies \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j
% \end{align*}
% Combining, we have
% $$\hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j \iff \hat{p}_{\bm{x}, j}  \ge t_j$$
% Therefore,
% $${\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}} =  {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}$$



% % Rewriting the confident joint to include $\epsilon_{\bm{x}, j}$ and $t_j + \epsilon_j$, we have
% % \begin{align*} 
% %     {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}} &= \{\bm{x} \in \bm{X}_{\tilde{y} = i} :  \hat{p}_{\bm{x}, j} + \epsilon_{\bm{x}, j} \ge t_j + \epsilon_j\}  \\
% %     {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}} &= \{\bm{x} \in \bm{X}_{\tilde{y} = i} : \epsilon_{\bm{x}, j} \ge \epsilon_j + t_j - \hat{p}_{\bm{x}, j}\}  \\
% %     {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}^{\epsilon_{\bm{x}, j}} &=  {\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}  && \triangleright \text{By Equation (\ref{eqn:piecewise_error})}\\
% %     %  &= \lvert \{\bm{x} \in \bm{X}_{\tilde{y} = i} :  \hat{p}_{\bm{x}, j}  \ge t_j \}  \rvert \\
% %     %  &= \cj[i][j]
% % \end{align*}

% % The last step follows from from Eqn. \ref{eqn:piecewise_error}: When $\hat{p}_{\bm{x}, j} \geq t_j$ then $\epsilon_{\bm{x}, j} \ge \epsilon_j + t_j - \hat{p}_{\bm{x}, j}$ and $\hat{p}_{\bm{x}, j} \geq t_j$ then $\epsilon_{\bm{x}, j} \ge \epsilon_j + t_j - \hat{p}_{\bm{x}, j}$


% Because ${\hat{\bm{X}}_{ \tilde{y} \smalleq i,y^* \smalleq j}}$ is unchanged the result of consistent estimation and exact label errors from Corollary \ref{cor:per_class_robustness} holds under no label collisions. While we assume there are infinite examples in $\bm{X}$, the proof applies for finite datasets if you omit discretization error. 

% \end{proof}













==> Confident Learning (JAIR 2021) (Version 6610)/unused_sections/robustness.tex <==
\subsection{Robust Latent Estimation}

In this section, we show how confident learning and the confident joint enable robust estimation of the latent prior. We present Alg. \ref{alg:latent}, which shows the simplicity of the estimation procedure when formulated in terms of the confident joint. Profoundly, Alg. \ref{alg:latent} uses the unnormalized confident joint directly without needing $n\Hat{P}_{s,y}$ because every computation in Alg. \ref{alg:latent} is a relative ratio of unnormalized terms. This approach is reminiscent of the Metropolis–Hastings algorithm for estimating latent distributions, in our case, with label errors. 

Steps 2 and 3 in Alg. \ref{alg:latent} are self-explanatory marginalizations of the confident joint, however, it turns out that latent prior estimation in step 1 plays an important role in robust estimation. The prior in \ref{alg:latent} is estimated as $\hat{p}(y\smalleq k) = C_{y\smalleq k} / C_{s\smalleq k} \cdot p(s\smalleq k)$. We refer to this as the \emph{robust} estimator.  In prior work \citep{northcutt2017rankpruning, Sukhbaatar_fergus_iclr_2015}, $\Hat{p}(y)$ is computed in terms of $p(s)$ as $\hat{p}(y\smalleq k) = \sum_{j \smallin K} P_{y \smalleq k \vert s \smalleq j} \cdot p(s\smalleq j) , \forall k \smallin K$. We refer to this as the \emph{standard} estimator.

% Fig. \ref{fig:many_combined} compares these two methods across the full spectrum of label noise, demonstrating the increased accuracy of the \emph{robust} estimates of the latent prior $p(y)$, noisy channel $\nm$, and inverse noise matrix, $\inv$ for both a noisy three-class Gaussian synthetic dataset (Fig. \ref{fig:gauss3} in Sup. Mats.) and the handwritten digits MNIST dataset \cite{mnist_handwritten_digits_dataset_1998} with added label noise. In all graphs, the average norm of the estimate and the true distribution is plotted. We added label noise by generating 30 uniformly random, $P_{s \vert y}$ valid (meet learnability bounds) matrices for a particular trace value, then flipped the MNIST labels to match the generated noisy channels. The model we used was the PyTorch CNN \cite{mnist_cnn_pytorch_structure} for MNIST and the default scikit-learn implementation of logistic regression with isometric calibration for three-Guassian dataset. 

Fig. \ref{fig:many_combined} compares these two methods across the spectrum of label noise, demonstrating the decreased error (average norm of estimator versus truth) of the \emph{robust} estimator on both synthetic and MNIST datsets. We added label noise by generating 30 uniformly random, $P_{s \vert y}$ valid (meet learnability bounds) matrices for a particular trace value, then flipped the MNIST labels to match the generated noisy channels. The model we used was the PyTorch CNN \cite{mnist_cnn_pytorch_structure} for MNIST and the default scikit-learn implementation of logistic regression with isometric calibration for three-Guassian dataset. 

% The middle and right figures compare our estimates of the noisy channel and inverse noise matrix by (redundantly) computing these conditional distributions in terms of the standard $\Hat{p}(y)$ to understand how the error propagates. 
The vertical lines in Fig. \ref{fig:many_combined} [middle] are error bars and the thick, dashed black line depicts uniformly random performance, i.e. the expected norm of the given noise matrix and a random noise matrix. Importantly, we see a large drop at $\Tr (P_{s \vert y}) < 1$, which agrees with the learnability bound in Thm. \ref{trace_bound}. Observe that for both MNIST and the synthetic Gaussian datasets, the error is small with low label noise, however, in this regime, our robust estimator falls short. To account for this, we introduced a third \emph{converged/consistent} estimator and force mathematical consistency for three iterations. As you can see, these estimators perform best in both low and high noise regimes. %Because the difference is small, for simplicity we only present the robust estimator in Alg. \ref{alg:rp}. 
Finally, notice that the overall norm values are extremely low. In the case of MNIST, the estimated matrices have 100 values, yet the norms are between 1 and 3. %This demonstrates the impressively high accuracy of confident learning for latent estimation. 
For a more concrete example, we provide a side-by-side comparison of the noise matrices estimated by rankpruning versus the actual noise matrices in an experiment on the MNIST dataset in Fig. \ref{fig:mnist_cnn_rho_plots_page_final} in the Supplementary Materials.

The mathematical underpinning of these results relies on the fact that our robust estimator $\hat{p}(y\smalleq k) = C_{y\smalleq k} / C_{s\smalleq k} \cdot p(s\smalleq k)$ has a ratio of estimates and they are for the same class. If we assume that error, $\epsilon$, is added for each class (i.e. error is more similar within the same class than across different classes), then the same epsilon will be in the numerator and denominator of the robust estimator because both depend on class $k$. However, if we consider the standard estimator, $\hat{p}(y\smalleq k) = \sum_{j \smallin K} P_{y \smalleq k \vert s \smalleq j} \cdot p(s\smalleq j) , \forall k \smallin K$, we see the only estimated term is the noise rate which is computed as a ratio of estimates for different classes, and so, the epsilon terms do not have the same cancelling effect.

% Anecdotally, we could have estimated the prior as a marginal $\Hat{p}(y) = \frac{1}{\sum_{k \smallin K} C_{y\smalleq k}}C_{y}$, but this will perform poorly unless the model's predicted probabilities are equally accurate across all latent classes because the confident joint counts examples using thresholds based on averaging the noisy class labels, but this method marginalizes with respect to the latent class labels. Additionally, this method performed worse across all settings, datasets, and models we tested.



% \begin{figure}[ht]
% \begin{subfigure}{0.3\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_train_errors_removed.pdf} 
% \caption{a}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.39\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_test_errors_removed.pdf}
% \caption{b}
% \label{fig:subim2}
% \end{subfigure}
% \begin{subfigure}{0.3\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_test_errors_removed.pdf}
% \caption{b}
% \label{fig:subim2}
% \end{subfigure}
% \caption{MNIST percent reduction in test error from training and test with the complete dataset to training with errors removed from the (a) train set, and (b) test set.}
% \label{fig:image2}
% \end{figure}

% \begin{figure}[ht]

% \begin{subfigure}[ht]{0.3\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_py_calibrated-lr.pdf}}
% % \vskip -.1in
% \caption{a} 
% \label{fig:robust_latent_lr}
% % \vskip -0.3in
% \end{subfigure}

% \begin{subfigure}[ht]{0.4\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_py_mnist_cnn.pdf}}
% % \vskip -.1in
% \caption{b} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{subfigure}

% \begin{subfigure}[ht]{0.3\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=.3\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}}
% % \vskip -.1in
% \caption{c} 
% \label{fig:mnist_test_acc_with_rp}
% % \vskip -0.3in
% \end{subfigure}

% \end{figure}


% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_calibrated_lr.pdf}}
% \vskip -.1in
% \caption{Robust latent estimation on Gaussian $(m=3)$ synthetic data (w/ added label noise) using the default scikit-learn implementation of logistic regression with isometric calibration.} 
% \label{fig:robust_latent_lr}
% % \vskip -0.3in
% \end{figure*}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_mnist_cnn_all3.pdf}}
% \vskip -.1in
% \caption{Depicts reduced robust latent estimation of $p(y)$on MNIST (w/ added label noise) using PyTorch MNIST CNN.} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{figure*}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=.9\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}}
% \vskip -.1in
% \caption{Comparison of MNIST (w/ add label noise) test accuracy (averaged over 30 trials per $\Tr (\nm)$) with and without rankpruning for different noise sparsities. Although the test accuracy is lower for sparser $P_{s \vert y}$, rankpruning boasts increased accuracy gains.} 
% \label{fig:mnist_test_acc_with_rp}
% % \vskip -0.3in
% \end{figure*}


\begin{figure}[htp]

\centering
\includegraphics[width=.3\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}\hfill
\includegraphics[width=.39\textwidth]{img/robust_py_calibrated-lr.pdf}\hfill
\includegraphics[width=.3\textwidth]{img/robust_py_mnist_cnn.pdf}

\caption{MNIST and synthetic experiments with added label noise. \textbf{[left]} Increase in test accuracy with rankpruning on MNIST from extreme (2) to no noise (10) for sparse and dense $P_{s \vert y}$. \textbf{[middle]}$\hat{p}(y)$ estimation error from 100\% noise (trace=0) to 0\% noise (trace=3) on a 3-Gaussian synthetic dataset. \textbf{[right]}  $\hat{p}(y)$ estimation error from 100\% noise (trace=0) to 0\% noise (trace=10) on MNIST. }
\label{fig:many_combined}
\vskip -.1in
\end{figure}

==> Confident Learning (JAIR 2021) (Version 6610)/unused_sections/theory_learning_bounds.tex <==
\section{Necessary Conditions for Learnability}

We prove necessary conditions for learning with noisy labels.


\subsection{Learnability Bounds for Multiclass Learning from Noisy Labels} \label{sec:bounds}


We develop three necessary conditions for the general case of multiclass learning with noisy labels. We call these learnability bounds. A problem is learnable if it is possible that data (training examples and labels) can be used to achieve better than random performance. Unlike the typical information theoretic formulation, in the case of learning with noisy labels, we assume there are no guaranteed labels $y$, thus learning the opposite decision boundary results in 100\% error. So, for example, perfect mutual information could be achieved without meeting the necessary conditions for learnability.

To our knowledge, these are the first bounds on $P_{s , y}$ and also the first strict lower bound on the number of training labels necessary for multiclass noisy learning with noisy labels to be possible. In proving these bounds, the $\Tr (P_{s \vert y})$, $\Tr (P_{y \vert s})$, and $\Tr (P_{s , y})$ reveal themselves as important statistics in confident learning. We use them, or the diagonal terms explicitly, extensively. For all the theorems in this section, we assume there is at least one example belonging to every class, the data $X$ is error-free, and the label noise is class-conditional.

To derive necessary conditions for the general case of multiclass learning with noisy labels, we assume class-conditional uniform noise (flipping) rates. Our focus is necessary conditions for learnability, not error or generalization bounds. We start with a necessary condition for learnability in the binary ($m = 2$) case is {\small $p(s=0 \vert y=1) + p(s=1 \vert y=0) < 1$} \citep{NIPS2013_5073}, or equivalently {\small $p(y=0 \vert s=1) + p(y=1 \vert s=0) < 1$} \citep{ScottBH13}, otherwise more examples would be mislabeled than labeled correctly and we would learn the opposite decision boundary condition. 
% Note this condition makes no assumptions on the data generating distribution or the model and thus allows for what may appear as arbitrarily large mislabeling. As an extreme example, one could have 1,000,000 negative examples, 999,999 of which are mislabeled as positive, and 2 positive examples, both correctly labeled. Then nearly $100\%$ of examples are mislabeled, but a boundary is still learnable, for example, by fitting around the two positive examples. 
Rewriting the condition as {\small $p(s=1 \vert y=0) < p(s=1 \vert y=1)$}, then generally, $\forall k \smallin K, p(s =  k \vert y \neq k) < p(s=k \vert y=k)$ and $p(y = k \vert s \neq k) < p(y=k \vert s=k)$.
% \begin{equation}
% p(s =  k \vert y \neq k) < p(s=k \vert y=k) \text{and} \quad p(y = k \vert s \neq k) < p(y=k \vert s=k)
% \end{equation}

\begin{lemma}[Class Conditional Bound] Proof \ref{proof:class_conditional_bound}.1 in Supplementary Materials % for Multiclass Learning with Noisy Labels]
\label{class_conditional_bound}
$\\ \forall k \smallin K$, $p(s = k) < p(s=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k)$ 
\end{lemma}

% \begin{proof}
% $p(s = k \vert y \neq k) < p(s=k \vert y=k) \leftrightarrow 
% \frac{p(y \neq k \vert s = k) p(s = k)}{p(y \neq k)}  < \frac{p(y=k \vert s = k) p(s = k)}{p(y=k)} \\
% \leftrightarrow p(y \neq k \vert s = k) p(y = k)  < p(y=k \vert s = k) p(y \neq k) \\
% \leftrightarrow p(y = k) - p(y = k \vert s = k) p(y = k)  < p(y=k \vert s = k) - p(y=k \vert s = k) p(y=k) \\
% \leftrightarrow p(y = k) < p(y=k \vert s=k)$ \\
% Symmetrically,
% $p(y = k \vert s \neq k) < p(y=k \vert s=k) 
% \leftrightarrow p(s = k) < p(s=k \vert y=k)$
% \end{proof}


\begin{theorem}[Class Product Bound] Proof \ref{proof:class_product_bound}.2 in Supplementary Materials % for Multiclass Learning with Noisy Labels]
\label{class_product_bound}
$\\ \forall k \smallin K$, $ p(s = k)p(y=k) < p(s=k, y=k)$
\end{theorem}
\vskip -.05in
% \begin{proof}
% \vskip -.1in 
% Multiply the first and second inequalities in Lemma 1 by $p(y=k)$ and $p(s=k)$, respectively.
% \end{proof}
% \vskip -.2in

The class product bound from Thm (\ref{class_product_bound}) expresses a notion of necessary dependence between observed, noisy labels $s$ and actual labels $y$. By contradiction, if $\forall k, p(s = k)p(y=k) = p(s=k, y=k)$, implying $s \independent y$, then learning $x \rightarrow y$ from $X$ and $s$ would be impossible. Because these bounds only depend on the class $k \smallin K$ holds for any set of examples $X$.

\begin{theorem}[Number of Training Examples: $n$ Bound] Proof \ref{proof:n_bound}.3 in Supplementary Materials %for Multiclass Learning with Noisy Labels]
\label{n_bound}
\begin{equation}
% \begin{split} 
% \text{Let } n = &\underbrace{\text{count}(s=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(s=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}    \\   
% + &\underbrace{\text{count}(s\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(s\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
% \end{split}
n \smalleq \underbrace{\text{count}(s=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(s=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}     
+ \underbrace{\text{count}(s\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(s\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
\end{equation} 
\vskip -.05in
then $\forall k \smallin K, n > \frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k)$ and equivalently $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$. 
\end{theorem}

% \begin{proof}
% %\vskip -.1in
% $\forall k, p(s = k)p(y=k) < p(s=k, y=k) \\
% \leftrightarrow \small{\left(p(s = k, y=k) + p(s = k, y \neq k) \right) \cdot \left(p(y = k, s=k) + p(y = k, s \neq k) \right) < p(s=k, y=k) } \\
% \leftrightarrow \left(\frac{C(k) + E_1(k)}{n} \right) \cdot \left(\frac{C(k) + E_2(k)}{n} \right) < \frac{C(k)}{n} \\
% \leftrightarrow C(k) \cdot \left[ C(k) + E_1(k) + E_2(k) \right] + E_1(k) \cdot E_2(k)  < n \cdot C(k) \\
% \leftrightarrow \forall k \smallin K, n > C(k) + E_1(k) + E_2(k) + \frac{E_1(k) \cdot E_2(k)}{C(k)}$ and $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$
% \end{proof}

Thm. (\ref{n_bound}) establishes, to our knowledge, the first lower bound on the number of training examples required for the general case of multiclass learning w.r.t. the number of label errors in each class. %This result is a necessary condition for each class, and therefore it is not sufficient for $k^* = \text{argmax}_k \left(\frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k) + C(k) \right) $. % Although surprisingly simple, to our knowledge this is the first lower bound on the number of examples need for multiclass learning with noisy labels. %If not met, there is not enough "signal" to distinguish the classes, regardless of model complexity. Extending Thm. (\ref{n_bound}) to conditions for error or generalization bounds requires highly restrictive assumptions about predicted probabilities $p(\hat{s}=k \vert x)$, otherwise one cannot disambiguate whether the error in predicted probabilities is due to the label noise or the inability of the learned model to exactly generalized to the complexity of the data distribution. Remaining general in our assumptions, we leave the development of necessary conditions for error and generalization bounds as open questions.
Notice that we can restate Lemma (\ref{class_conditional_bound}) as: 

\begin{theorem}[Trace Bound] Proof \ref{proof:trace_bound}.4 in Supplementary Materials %for Multiclass Learning with Noisy Labels]
\label{trace_bound} 
$\\ \Tr (P_{s \vert y}) > 1$ and $\Tr (P_{y \vert s}) > 1$ are necessary conditions for learnability with class-conditional noise.
\end{theorem}
% \begin{proof}
% %\vskip -.1in
% $
% \forall k \smallin K$, $p(s = k) < p(s=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k) \quad \triangleright \,\, $(Lemma \ref{class_conditional_bound})$\\
% \sum_{k \smallin K} p(s = k) < \sum_{k \smallin K} p(s=k \vert y=k)$ and $\sum_{k \smallin K} p(y = k) < \sum_{k \smallin K} p(y=k \vert s=k)
% \\ \Tr (P_{s \vert y}) > 1$ and $\Tr (P_{y \vert s}) > 1
% $ 
% \end{proof}

Thm. (\ref{trace_bound}) is necessary, but not sufficient for learnability, particularly when Thm. (\ref{class_conditional_bound}) is not satisfied. However, Thm. (\ref{trace_bound}) is of practical importance because it provides a quick way to test if the problem is \emph{not} learnable, i.e. if the trace of the noise matrix is less than or equal to 1.

% \textbfbf{Why do we care?} A growing consensus in the deep learning community suggests that with enough data, learning is possible with arbitrary amounts of uniformly random label noise \citep{krause_unreasonable_effectiveness_of_noisy_data_2016, 7837934_multiclass_learning_with_noise_using_dropout}. A few examples are: (1) ``label noise may be a limited issue if networks are trained on billions of images'' \citep{fair_laurens_van_der_maaten_limits_weak_supervision_2018}, (2) ``it seems the scale of data can overpower noise in the label space'' \citep{gupta_unreasonable_effectiveness_of_data_2017}, and (3) ``successful learning is possible with an arbitrary amount of noise'' \citep{rolnick_shavit_2017}. Theorem (\ref{n_bound}) shows that these assertions are likely misspecified w.r.t class-conditional noise by establishing a lower bound on the number of correctly-labeled training examples required by each class for learning to be possible in the presence of class-conditional label errors.  This is not to discredit the value of these works, particularly in the case of 
% \cite{fair_laurens_van_der_maaten_limits_weak_supervision_2018, gupta_unreasonable_effectiveness_of_data_2017} which are exceptional overviews of weak supervision and big data. Instead, we use these examples to illuminate the fact that our theory of confident learning helps to answer these difficult questions in a principled manner. This is a valuable step forward for the deep learning community, but more broadly, to anyone learning any model with noisy labels, as it strays away from speculation and provides exact, theoretical and necessary bounds on the number of correctly labeled training examples.

\textbf{Why do we care?} A growing consensus in the deep learning community suggests that with enough data, learning is possible with arbitrary amounts of noise \citep{krause_unreasonable_effectiveness_of_noisy_data_2016, 7837934_multiclass_learning_with_noise_using_dropout, fair_laurens_van_der_maaten_limits_weak_supervision_2018, gupta_unreasonable_effectiveness_of_data_2017, rolnick_shavit_2017}.  Theorem (\ref{n_bound}) shows that these assertions may be misspecified w.r.t class-conditional noise by establishing a lower bound on the number of correctly-labeled training examples required by each class for learnability. 




PROOFS FROM APPENDIX:


\section{Theorems and proofs for learnability}

\begin{lemma}[Class Conditional Bound] % for Multiclass Learning with Noisy Labels]
% \label{class_conditional_bound}
$\\ \forall k \in 1..m$, $p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k)$ 
\end{lemma}

\begin{proof} \label{proof:class_conditional_bound}
$p(\tilde{y} = k \vert y \neq k) < p(\tilde{y}=k \vert y=k) \leftrightarrow 
\frac{p(y \neq k \vert s = k) p(\tilde{y} = k)}{p(y \neq k)}  < \frac{p(y=k \vert s = k) p(\tilde{y} = k)}{p(y=k)} \\
\leftrightarrow p(y \neq k \vert s = k) p(y = k)  < p(y=k \vert s = k) p(y \neq k) \\
\leftrightarrow p(y = k) - p(y = k \vert s = k) p(y = k)  < p(y=k \vert s = k) - p(y=k \vert s = k) p(y=k) \\
\leftrightarrow p(y = k) < p(y=k \vert s=k)$ \\
Symmetrically,
$p(y = k \vert s \neq k) < p(y=k \vert s=k) 
\leftrightarrow p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$
\end{proof}


\begin{theorem}[Class Product Bound] % for Multiclass Learning with Noisy Labels]
% \label{class_product_bound}
$\\ \forall k \in 1..m$, $ p(\tilde{y} = k)p(y=k) < p(\tilde{y}=k, y=k)$
\end{theorem}

\begin{proof} \label{proof:class_product_bound}
\vskip -.1in
Multiply the first and second inequalities in Lemma 1 by $p(y=k)$ and $p(\tilde{y}=k)$, respectively.
\end{proof}
\vskip -.2in

\begin{theorem}[Number of Training Examples: $n$ Bound] %for Multiclass Learning with Noisy Labels]
% \label{n_bound}
\begin{equation}
% \begin{split} 
% \text{Let } n = &\underbrace{\text{count}(\tilde{y}=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(\tilde{y}=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}    \\   
% + &\underbrace{\text{count}(\tilde{y}\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(\tilde{y}\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
% \end{split}
n \smalleq \underbrace{\text{count}(\tilde{y}=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(\tilde{y}=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}     
+ \underbrace{\text{count}(\tilde{y}\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(\tilde{y}\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
\end{equation}

% and $k^* = \text{argmax}_k \left(\frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k) + C(k) \right) $, \\

then $\forall k \in 1..m, n > \frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k)$ and equivalently $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$. 
\end{theorem}

\begin{proof} \label{proof:n_bound}
%\vskip -.1in
$\forall k, p(\tilde{y} = k)p(y=k) < p(\tilde{y}=k, y=k) \\
\leftrightarrow \small{\left(p(\tilde{y} = k, y=k) + p(\tilde{y} = k, y \neq k) \right) \cdot \left(p(y = k, s=k) + p(y = k, s \neq k) \right) < p(\tilde{y}=k, y=k) } \\
\leftrightarrow \left(\frac{C(k) + E_1(k)}{n} \right) \cdot \left(\frac{C(k) + E_2(k)}{n} \right) < \frac{C(k)}{n} \\
\leftrightarrow C(k) \cdot \left[ C(k) + E_1(k) + E_2(k) \right] + E_1(k) \cdot E_2(k)  < n \cdot C(k) \\
\leftrightarrow \forall k \in 1..m, n > C(k) + E_1(k) + E_2(k) + \frac{E_1(k) \cdot E_2(k)}{C(k)}$ and $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$
\end{proof}


\begin{theorem}[Trace Bound] %for Multiclass Learning with Noisy Labels]
% \label{trace_bound} 
$\\ \Tr (\nm) > 1$ and $\Tr (\inv) > 1$ are necessary conditions for learnability with class-conditional noise.
\end{theorem}
\begin{proof} \label{proof:trace_bound}
%\vskip -.1in
$
\forall k \in 1..m$, $p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k) \quad \triangleright \,\, $(Lemma \ref{class_conditional_bound})$\\
\sum_{k \in 1..m} p(\tilde{y} = k) < \sum_{k \in 1..m} p(\tilde{y}=k \vert y=k)$ and $\sum_{k \in 1..m} p(y = k) < \sum_{k \in 1..m} p(y=k \vert s=k)
\\ \Tr (\nm) > 1$ and $\Tr (\inv) > 1
$ 
\end{proof}




==> Makefile <==
DEPS := \
	algorithm.sty \
	algorithmic.sty \
	fancyhdr.sty \
	icml2019.bst \
	icml2019.sty \
	paper.bib \
	macros.tex \
	abstract.tex \
	introduction.tex \
	identifying.tex \
	case-study.tex \
	discussion.tex \
	correcting.tex \
	related-work.tex \
	conclusion.tex \
	acknowledgements.tex \
	bibliography.tex \


LATEX  := pdflatex
BIBTEX := bibtex
PANDOC := pandoc

# phony targets

all: paper.pdf abstract.txt

clean:
	rm -rf *.aux *.log *.blg *.bbl *.ent *.out *.dvi *.ps *.pdf *.tar.gz abstract.txt

arxiv: arxiv.tar.gz

.PHONY: all clean arxiv

# main targets

arxiv.tar.gz: paper.pdf # just build the paper because we want to build the .bbl
	tar czvf paper.tar.gz paper.tex paper.bbl $(DEPS)

%.txt: %.tex
	$(PANDOC) $< -o $@ -f latex -t plain --wrap=none

%.pdf: %.tex $(DEPS)
	$(eval SRC_$@ = $(patsubst %.tex, %, $<))
	$(LATEX) $(SRC_$@)
	$(BIBTEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)


==> unused_sections/robustness.tex <==
\subsection{Robust Latent Estimation}

In this section, we show how confident learning and the confident joint enable robust estimation of the latent prior. We present Alg. \ref{alg:latent}, which shows the simplicity of the estimation procedure when formulated in terms of the confident joint. Profoundly, Alg. \ref{alg:latent} uses the unnormalized confident joint directly without needing $n\Hat{P}_{s,y}$ because every computation in Alg. \ref{alg:latent} is a relative ratio of unnormalized terms. This approach is reminiscent of the Metropolis–Hastings algorithm for estimating latent distributions, in our case, with label errors. 

Steps 2 and 3 in Alg. \ref{alg:latent} are self-explanatory marginalizations of the confident joint, however, it turns out that latent prior estimation in step 1 plays an important role in robust estimation. The prior in \ref{alg:latent} is estimated as $\hat{p}(y\smalleq k) = C_{y\smalleq k} / C_{s\smalleq k} \cdot p(s\smalleq k)$. We refer to this as the \emph{robust} estimator.  In prior work \citep{northcutt2017rankpruning, Sukhbaatar_fergus_iclr_2015}, $\Hat{p}(y)$ is computed in terms of $p(s)$ as $\hat{p}(y\smalleq k) = \sum_{j \smallin K} P_{y \smalleq k \vert s \smalleq j} \cdot p(s\smalleq j) , \forall k \smallin K$. We refer to this as the \emph{standard} estimator.

% Fig. \ref{fig:many_combined} compares these two methods across the full spectrum of label noise, demonstrating the increased accuracy of the \emph{robust} estimates of the latent prior $p(y)$, noisy channel $\nm$, and inverse noise matrix, $\inv$ for both a noisy three-class Gaussian synthetic dataset (Fig. \ref{fig:gauss3} in Sup. Mats.) and the handwritten digits MNIST dataset \cite{mnist_handwritten_digits_dataset_1998} with added label noise. In all graphs, the average norm of the estimate and the true distribution is plotted. We added label noise by generating 30 uniformly random, $P_{s \vert y}$ valid (meet learnability bounds) matrices for a particular trace value, then flipped the MNIST labels to match the generated noisy channels. The model we used was the PyTorch CNN \cite{mnist_cnn_pytorch_structure} for MNIST and the default scikit-learn implementation of logistic regression with isometric calibration for three-Guassian dataset. 

Fig. \ref{fig:many_combined} compares these two methods across the spectrum of label noise, demonstrating the decreased error (average norm of estimator versus truth) of the \emph{robust} estimator on both synthetic and MNIST datsets. We added label noise by generating 30 uniformly random, $P_{s \vert y}$ valid (meet learnability bounds) matrices for a particular trace value, then flipped the MNIST labels to match the generated noisy channels. The model we used was the PyTorch CNN \cite{mnist_cnn_pytorch_structure} for MNIST and the default scikit-learn implementation of logistic regression with isometric calibration for three-Guassian dataset. 

% The middle and right figures compare our estimates of the noisy channel and inverse noise matrix by (redundantly) computing these conditional distributions in terms of the standard $\Hat{p}(y)$ to understand how the error propagates. 
The vertical lines in Fig. \ref{fig:many_combined} [middle] are error bars and the thick, dashed black line depicts uniformly random performance, i.e. the expected norm of the given noise matrix and a random noise matrix. Importantly, we see a large drop at $\Tr (P_{s \vert y}) < 1$, which agrees with the learnability bound in Thm. \ref{trace_bound}. Observe that for both MNIST and the synthetic Gaussian datasets, the error is small with low label noise, however, in this regime, our robust estimator falls short. To account for this, we introduced a third \emph{converged/consistent} estimator and force mathematical consistency for three iterations. As you can see, these estimators perform best in both low and high noise regimes. %Because the difference is small, for simplicity we only present the robust estimator in Alg. \ref{alg:rp}. 
Finally, notice that the overall norm values are extremely low. In the case of MNIST, the estimated matrices have 100 values, yet the norms are between 1 and 3. %This demonstrates the impressively high accuracy of confident learning for latent estimation. 
For a more concrete example, we provide a side-by-side comparison of the noise matrices estimated by rankpruning versus the actual noise matrices in an experiment on the MNIST dataset in Fig. \ref{fig:mnist_cnn_rho_plots_page_final} in the Supplementary Materials.

The mathematical underpinning of these results relies on the fact that our robust estimator $\hat{p}(y\smalleq k) = C_{y\smalleq k} / C_{s\smalleq k} \cdot p(s\smalleq k)$ has a ratio of estimates and they are for the same class. If we assume that error, $\epsilon$, is added for each class (i.e. error is more similar within the same class than across different classes), then the same epsilon will be in the numerator and denominator of the robust estimator because both depend on class $k$. However, if we consider the standard estimator, $\hat{p}(y\smalleq k) = \sum_{j \smallin K} P_{y \smalleq k \vert s \smalleq j} \cdot p(s\smalleq j) , \forall k \smallin K$, we see the only estimated term is the noise rate which is computed as a ratio of estimates for different classes, and so, the epsilon terms do not have the same cancelling effect.

% Anecdotally, we could have estimated the prior as a marginal $\Hat{p}(y) = \frac{1}{\sum_{k \smallin K} C_{y\smalleq k}}C_{y}$, but this will perform poorly unless the model's predicted probabilities are equally accurate across all latent classes because the confident joint counts examples using thresholds based on averaging the noisy class labels, but this method marginalizes with respect to the latent class labels. Additionally, this method performed worse across all settings, datasets, and models we tested.



% \begin{figure}[ht]
% \begin{subfigure}{0.3\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_train_errors_removed.pdf} 
% \caption{a}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.39\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_test_errors_removed.pdf}
% \caption{b}
% \label{fig:subim2}
% \end{subfigure}
% \begin{subfigure}{0.3\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{img/mnist_test_error_test_errors_removed.pdf}
% \caption{b}
% \label{fig:subim2}
% \end{subfigure}
% \caption{MNIST percent reduction in test error from training and test with the complete dataset to training with errors removed from the (a) train set, and (b) test set.}
% \label{fig:image2}
% \end{figure}

% \begin{figure}[ht]

% \begin{subfigure}[ht]{0.3\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_py_calibrated-lr.pdf}}
% % \vskip -.1in
% \caption{a} 
% \label{fig:robust_latent_lr}
% % \vskip -0.3in
% \end{subfigure}

% \begin{subfigure}[ht]{0.4\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_py_mnist_cnn.pdf}}
% % \vskip -.1in
% \caption{b} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{subfigure}

% \begin{subfigure}[ht]{0.3\textwidth}
% % \vskip -.1in
% \centerline{\includegraphics[width=.3\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}}
% % \vskip -.1in
% \caption{c} 
% \label{fig:mnist_test_acc_with_rp}
% % \vskip -0.3in
% \end{subfigure}

% \end{figure}


% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_calibrated_lr.pdf}}
% \vskip -.1in
% \caption{Robust latent estimation on Gaussian $(m=3)$ synthetic data (w/ added label noise) using the default scikit-learn implementation of logistic regression with isometric calibration.} 
% \label{fig:robust_latent_lr}
% % \vskip -0.3in
% \end{figure*}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=1\textwidth]{img/robust_mnist_cnn_all3.pdf}}
% \vskip -.1in
% \caption{Depicts reduced robust latent estimation of $p(y)$on MNIST (w/ added label noise) using PyTorch MNIST CNN.} 
% \label{fig:robust_mnist_cnn}
% % \vskip -0.3in
% \end{figure*}

% \begin{figure*}[ht]
% \vskip -.1in
% \centerline{\includegraphics[width=.9\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}}
% \vskip -.1in
% \caption{Comparison of MNIST (w/ add label noise) test accuracy (averaged over 30 trials per $\Tr (\nm)$) with and without rankpruning for different noise sparsities. Although the test accuracy is lower for sparser $P_{s \vert y}$, rankpruning boasts increased accuracy gains.} 
% \label{fig:mnist_test_acc_with_rp}
% % \vskip -0.3in
% \end{figure*}


\begin{figure}[htp]

\centering
\includegraphics[width=.3\textwidth]{img/mnist_with_rankpruning_test_acc.pdf}\hfill
\includegraphics[width=.39\textwidth]{img/robust_py_calibrated-lr.pdf}\hfill
\includegraphics[width=.3\textwidth]{img/robust_py_mnist_cnn.pdf}

\caption{MNIST and synthetic experiments with added label noise. \textbf{[left]} Increase in test accuracy with rankpruning on MNIST from extreme (2) to no noise (10) for sparse and dense $P_{s \vert y}$. \textbf{[middle]}$\hat{p}(y)$ estimation error from 100\% noise (trace=0) to 0\% noise (trace=3) on a 3-Gaussian synthetic dataset. \textbf{[right]}  $\hat{p}(y)$ estimation error from 100\% noise (trace=0) to 0\% noise (trace=10) on MNIST. }
\label{fig:many_combined}
\vskip -.1in
\end{figure}

==> unused_sections/theory_learning_bounds.tex <==
\section{Necessary Conditions for Learnability}

We prove necessary conditions for learning with noisy labels.


\subsection{Learnability Bounds for Multiclass Learning from Noisy Labels} \label{sec:bounds}


We develop three necessary conditions for the general case of multiclass learning with noisy labels. We call these learnability bounds. A problem is learnable if it is possible that data (training examples and labels) can be used to achieve better than random performance. Unlike the typical information theoretic formulation, in the case of learning with noisy labels, we assume there are no guaranteed labels $y$, thus learning the opposite decision boundary results in 100\% error. So, for example, perfect mutual information could be achieved without meeting the necessary conditions for learnability.

To our knowledge, these are the first bounds on $P_{s , y}$ and also the first strict lower bound on the number of training labels necessary for multiclass noisy learning with noisy labels to be possible. In proving these bounds, the $\Tr (P_{s \vert y})$, $\Tr (P_{y \vert s})$, and $\Tr (P_{s , y})$ reveal themselves as important statistics in confident learning. We use them, or the diagonal terms explicitly, extensively. For all the theorems in this section, we assume there is at least one example belonging to every class, the data $X$ is error-free, and the label noise is class-conditional.

To derive necessary conditions for the general case of multiclass learning with noisy labels, we assume class-conditional uniform noise (flipping) rates. Our focus is necessary conditions for learnability, not error or generalization bounds. We start with a necessary condition for learnability in the binary ($m = 2$) case is {\small $p(s=0 \vert y=1) + p(s=1 \vert y=0) < 1$} \citep{NIPS2013_5073}, or equivalently {\small $p(y=0 \vert s=1) + p(y=1 \vert s=0) < 1$} \citep{ScottBH13}, otherwise more examples would be mislabeled than labeled correctly and we would learn the opposite decision boundary condition. 
% Note this condition makes no assumptions on the data generating distribution or the model and thus allows for what may appear as arbitrarily large mislabeling. As an extreme example, one could have 1,000,000 negative examples, 999,999 of which are mislabeled as positive, and 2 positive examples, both correctly labeled. Then nearly $100\%$ of examples are mislabeled, but a boundary is still learnable, for example, by fitting around the two positive examples. 
Rewriting the condition as {\small $p(s=1 \vert y=0) < p(s=1 \vert y=1)$}, then generally, $\forall k \smallin K, p(s =  k \vert y \neq k) < p(s=k \vert y=k)$ and $p(y = k \vert s \neq k) < p(y=k \vert s=k)$.
% \begin{equation}
% p(s =  k \vert y \neq k) < p(s=k \vert y=k) \text{and} \quad p(y = k \vert s \neq k) < p(y=k \vert s=k)
% \end{equation}

\begin{lemma}[Class Conditional Bound] Proof \ref{proof:class_conditional_bound}.1 in Supplementary Materials % for Multiclass Learning with Noisy Labels]
\label{class_conditional_bound}
$\\ \forall k \smallin K$, $p(s = k) < p(s=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k)$ 
\end{lemma}

% \begin{proof}
% $p(s = k \vert y \neq k) < p(s=k \vert y=k) \leftrightarrow 
% \frac{p(y \neq k \vert s = k) p(s = k)}{p(y \neq k)}  < \frac{p(y=k \vert s = k) p(s = k)}{p(y=k)} \\
% \leftrightarrow p(y \neq k \vert s = k) p(y = k)  < p(y=k \vert s = k) p(y \neq k) \\
% \leftrightarrow p(y = k) - p(y = k \vert s = k) p(y = k)  < p(y=k \vert s = k) - p(y=k \vert s = k) p(y=k) \\
% \leftrightarrow p(y = k) < p(y=k \vert s=k)$ \\
% Symmetrically,
% $p(y = k \vert s \neq k) < p(y=k \vert s=k) 
% \leftrightarrow p(s = k) < p(s=k \vert y=k)$
% \end{proof}


\begin{theorem}[Class Product Bound] Proof \ref{proof:class_product_bound}.2 in Supplementary Materials % for Multiclass Learning with Noisy Labels]
\label{class_product_bound}
$\\ \forall k \smallin K$, $ p(s = k)p(y=k) < p(s=k, y=k)$
\end{theorem}
\vskip -.05in
% \begin{proof}
% \vskip -.1in 
% Multiply the first and second inequalities in Lemma 1 by $p(y=k)$ and $p(s=k)$, respectively.
% \end{proof}
% \vskip -.2in

The class product bound from Thm (\ref{class_product_bound}) expresses a notion of necessary dependence between observed, noisy labels $s$ and actual labels $y$. By contradiction, if $\forall k, p(s = k)p(y=k) = p(s=k, y=k)$, implying $s \independent y$, then learning $x \rightarrow y$ from $X$ and $s$ would be impossible. Because these bounds only depend on the class $k \smallin K$ holds for any set of examples $X$.

\begin{theorem}[Number of Training Examples: $n$ Bound] Proof \ref{proof:n_bound}.3 in Supplementary Materials %for Multiclass Learning with Noisy Labels]
\label{n_bound}
\begin{equation}
% \begin{split} 
% \text{Let } n = &\underbrace{\text{count}(s=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(s=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}    \\   
% + &\underbrace{\text{count}(s\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(s\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
% \end{split}
n \smalleq \underbrace{\text{count}(s=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(s=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}     
+ \underbrace{\text{count}(s\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(s\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
\end{equation} 
\vskip -.05in
then $\forall k \smallin K, n > \frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k)$ and equivalently $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$. 
\end{theorem}

% \begin{proof}
% %\vskip -.1in
% $\forall k, p(s = k)p(y=k) < p(s=k, y=k) \\
% \leftrightarrow \small{\left(p(s = k, y=k) + p(s = k, y \neq k) \right) \cdot \left(p(y = k, s=k) + p(y = k, s \neq k) \right) < p(s=k, y=k) } \\
% \leftrightarrow \left(\frac{C(k) + E_1(k)}{n} \right) \cdot \left(\frac{C(k) + E_2(k)}{n} \right) < \frac{C(k)}{n} \\
% \leftrightarrow C(k) \cdot \left[ C(k) + E_1(k) + E_2(k) \right] + E_1(k) \cdot E_2(k)  < n \cdot C(k) \\
% \leftrightarrow \forall k \smallin K, n > C(k) + E_1(k) + E_2(k) + \frac{E_1(k) \cdot E_2(k)}{C(k)}$ and $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$
% \end{proof}

Thm. (\ref{n_bound}) establishes, to our knowledge, the first lower bound on the number of training examples required for the general case of multiclass learning w.r.t. the number of label errors in each class. %This result is a necessary condition for each class, and therefore it is not sufficient for $k^* = \text{argmax}_k \left(\frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k) + C(k) \right) $. % Although surprisingly simple, to our knowledge this is the first lower bound on the number of examples need for multiclass learning with noisy labels. %If not met, there is not enough "signal" to distinguish the classes, regardless of model complexity. Extending Thm. (\ref{n_bound}) to conditions for error or generalization bounds requires highly restrictive assumptions about predicted probabilities $p(\hat{s}=k \vert x)$, otherwise one cannot disambiguate whether the error in predicted probabilities is due to the label noise or the inability of the learned model to exactly generalized to the complexity of the data distribution. Remaining general in our assumptions, we leave the development of necessary conditions for error and generalization bounds as open questions.
Notice that we can restate Lemma (\ref{class_conditional_bound}) as: 

\begin{theorem}[Trace Bound] Proof \ref{proof:trace_bound}.4 in Supplementary Materials %for Multiclass Learning with Noisy Labels]
\label{trace_bound} 
$\\ \Tr (P_{s \vert y}) > 1$ and $\Tr (P_{y \vert s}) > 1$ are necessary conditions for learnability with class-conditional noise.
\end{theorem}
% \begin{proof}
% %\vskip -.1in
% $
% \forall k \smallin K$, $p(s = k) < p(s=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k) \quad \triangleright \,\, $(Lemma \ref{class_conditional_bound})$\\
% \sum_{k \smallin K} p(s = k) < \sum_{k \smallin K} p(s=k \vert y=k)$ and $\sum_{k \smallin K} p(y = k) < \sum_{k \smallin K} p(y=k \vert s=k)
% \\ \Tr (P_{s \vert y}) > 1$ and $\Tr (P_{y \vert s}) > 1
% $ 
% \end{proof}

Thm. (\ref{trace_bound}) is necessary, but not sufficient for learnability, particularly when Thm. (\ref{class_conditional_bound}) is not satisfied. However, Thm. (\ref{trace_bound}) is of practical importance because it provides a quick way to test if the problem is \emph{not} learnable, i.e. if the trace of the noise matrix is less than or equal to 1.

% \textbfbf{Why do we care?} A growing consensus in the deep learning community suggests that with enough data, learning is possible with arbitrary amounts of uniformly random label noise \citep{krause_unreasonable_effectiveness_of_noisy_data_2016, 7837934_multiclass_learning_with_noise_using_dropout}. A few examples are: (1) ``label noise may be a limited issue if networks are trained on billions of images'' \citep{fair_laurens_van_der_maaten_limits_weak_supervision_2018}, (2) ``it seems the scale of data can overpower noise in the label space'' \citep{gupta_unreasonable_effectiveness_of_data_2017}, and (3) ``successful learning is possible with an arbitrary amount of noise'' \citep{rolnick_shavit_2017}. Theorem (\ref{n_bound}) shows that these assertions are likely misspecified w.r.t class-conditional noise by establishing a lower bound on the number of correctly-labeled training examples required by each class for learning to be possible in the presence of class-conditional label errors.  This is not to discredit the value of these works, particularly in the case of 
% \cite{fair_laurens_van_der_maaten_limits_weak_supervision_2018, gupta_unreasonable_effectiveness_of_data_2017} which are exceptional overviews of weak supervision and big data. Instead, we use these examples to illuminate the fact that our theory of confident learning helps to answer these difficult questions in a principled manner. This is a valuable step forward for the deep learning community, but more broadly, to anyone learning any model with noisy labels, as it strays away from speculation and provides exact, theoretical and necessary bounds on the number of correctly labeled training examples.

\textbf{Why do we care?} A growing consensus in the deep learning community suggests that with enough data, learning is possible with arbitrary amounts of noise \citep{krause_unreasonable_effectiveness_of_noisy_data_2016, 7837934_multiclass_learning_with_noise_using_dropout, fair_laurens_van_der_maaten_limits_weak_supervision_2018, gupta_unreasonable_effectiveness_of_data_2017, rolnick_shavit_2017}.  Theorem (\ref{n_bound}) shows that these assertions may be misspecified w.r.t class-conditional noise by establishing a lower bound on the number of correctly-labeled training examples required by each class for learnability. 




PROOFS FROM APPENDIX:


\section{Theorems and proofs for learnability}

\begin{lemma}[Class Conditional Bound] % for Multiclass Learning with Noisy Labels]
% \label{class_conditional_bound}
$\\ \forall k \in 1..m$, $p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k)$ 
\end{lemma}

\begin{proof} \label{proof:class_conditional_bound}
$p(\tilde{y} = k \vert y \neq k) < p(\tilde{y}=k \vert y=k) \leftrightarrow 
\frac{p(y \neq k \vert s = k) p(\tilde{y} = k)}{p(y \neq k)}  < \frac{p(y=k \vert s = k) p(\tilde{y} = k)}{p(y=k)} \\
\leftrightarrow p(y \neq k \vert s = k) p(y = k)  < p(y=k \vert s = k) p(y \neq k) \\
\leftrightarrow p(y = k) - p(y = k \vert s = k) p(y = k)  < p(y=k \vert s = k) - p(y=k \vert s = k) p(y=k) \\
\leftrightarrow p(y = k) < p(y=k \vert s=k)$ \\
Symmetrically,
$p(y = k \vert s \neq k) < p(y=k \vert s=k) 
\leftrightarrow p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$
\end{proof}


\begin{theorem}[Class Product Bound] % for Multiclass Learning with Noisy Labels]
% \label{class_product_bound}
$\\ \forall k \in 1..m$, $ p(\tilde{y} = k)p(y=k) < p(\tilde{y}=k, y=k)$
\end{theorem}

\begin{proof} \label{proof:class_product_bound}
\vskip -.1in
Multiply the first and second inequalities in Lemma 1 by $p(y=k)$ and $p(\tilde{y}=k)$, respectively.
\end{proof}
\vskip -.2in

\begin{theorem}[Number of Training Examples: $n$ Bound] %for Multiclass Learning with Noisy Labels]
% \label{n_bound}
\begin{equation}
% \begin{split} 
% \text{Let } n = &\underbrace{\text{count}(\tilde{y}=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(\tilde{y}=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}    \\   
% + &\underbrace{\text{count}(\tilde{y}\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(\tilde{y}\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
% \end{split}
n \smalleq \underbrace{\text{count}(\tilde{y}=k,y=k)}_{C(k) \text{: Correctly Labeled}} + \underbrace{\text{count}(\tilde{y}=k,y\neq k)}_{E_1(k) \text{: Type 1 Errors}}     
+ \underbrace{\text{count}(\tilde{y}\neq k,y=k)}_{E_2(k) \text{: Type 2 Errors}} + \underbrace{\text{count}(\tilde{y}\neq k,y\neq k)}_{D(k) \text{: Different than class $k$}} 
\end{equation}

% and $k^* = \text{argmax}_k \left(\frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k) + C(k) \right) $, \\

then $\forall k \in 1..m, n > \frac{E_1(k) \cdot E_2(k)}{C(k)} + E_1(k) + E_2(k)$ and equivalently $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$. 
\end{theorem}

\begin{proof} \label{proof:n_bound}
%\vskip -.1in
$\forall k, p(\tilde{y} = k)p(y=k) < p(\tilde{y}=k, y=k) \\
\leftrightarrow \small{\left(p(\tilde{y} = k, y=k) + p(\tilde{y} = k, y \neq k) \right) \cdot \left(p(y = k, s=k) + p(y = k, s \neq k) \right) < p(\tilde{y}=k, y=k) } \\
\leftrightarrow \left(\frac{C(k) + E_1(k)}{n} \right) \cdot \left(\frac{C(k) + E_2(k)}{n} \right) < \frac{C(k)}{n} \\
\leftrightarrow C(k) \cdot \left[ C(k) + E_1(k) + E_2(k) \right] + E_1(k) \cdot E_2(k)  < n \cdot C(k) \\
\leftrightarrow \forall k \in 1..m, n > C(k) + E_1(k) + E_2(k) + \frac{E_1(k) \cdot E_2(k)}{C(k)}$ and $D(k) > \frac{E_1(k) \cdot E_2(k)}{C(k)}$
\end{proof}


\begin{theorem}[Trace Bound] %for Multiclass Learning with Noisy Labels]
% \label{trace_bound} 
$\\ \Tr (\nm) > 1$ and $\Tr (\inv) > 1$ are necessary conditions for learnability with class-conditional noise.
\end{theorem}
\begin{proof} \label{proof:trace_bound}
%\vskip -.1in
$
\forall k \in 1..m$, $p(\tilde{y} = k) < p(\tilde{y}=k \vert y=k)$ and $p(y = k) < p(y=k \vert s=k) \quad \triangleright \,\, $(Lemma \ref{class_conditional_bound})$\\
\sum_{k \in 1..m} p(\tilde{y} = k) < \sum_{k \in 1..m} p(\tilde{y}=k \vert y=k)$ and $\sum_{k \in 1..m} p(y = k) < \sum_{k \in 1..m} p(y=k \vert s=k)
\\ \Tr (\nm) > 1$ and $\Tr (\inv) > 1
$ 
\end{proof}



